Modern and Future Colliders

Since the initial development of charged particle colliders in the middle of the 20th century, these advanced scientific instruments have been at the forefront of scientific discoveries in high energy physics. Collider accelerator technology and beam physics have progressed immensely and modern facilities now operate at energies and luminosities many orders of magnitude greater than the pioneering colliders of the early 1960s. In addition, the field of colliders remains extremely dynamic and continues to develop many innovative approaches. Indeed, several novel concepts are currently being considered for designing and constructing even more powerful future colliders. In this paper, we first review the colliding beam method and the history of colliders, and then present the major achievements of operational machines and the key features of near-term collider projects that are currently under development. We conclude with an analysis of numerous proposals and studies for far-future colliders. The evaluation of their respective potentials reveals tantalizing prospects for further significant breakthroughs in the collider field.

==> crmp-refs.tex <==
%merlin.mbs apsrmp4-1.bst 2010-07-25 4.21a (PWD, AO, DPC) hacked
%Control: key (0)
%Control: author (3) reversed first dotless
%Control: editor formatted (0) differently from author
%Control: production of article title (0) allowed
%Control: page (1) range
%Control: year (0) verbatim
%Control: production of eprint (0) enabled
\begin{thebibliography}{381}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode
  `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{http://dx.doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Abanin}\ and\ \citenamefont
  {Levitov}(2007)}]{AL0704}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abanin}, \bibfnamefont
  {D~A}}, \ and\ \bibinfo {author} {\bibfnamefont {L.~S.}\ \bibnamefont
  {Levitov}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantized transport in graphene p-n junctions in a magnetic
  field},}\ }\href {\doibase 10.1126/science.1144672} {\bibfield  {journal}
  {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo {volume} {317}}~(\bibinfo
  {number} {5838}),\ \bibinfo {pages} {641--643}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Abanin}\ \emph {et~al.}(2006)\citenamefont {Abanin},
  \citenamefont {Lee},\ and\ \citenamefont {Levitov}}]{Abanin06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abanin}, \bibfnamefont
  {Dmitry~A}}, \bibinfo {author} {\bibfnamefont {Patrick~A.}\ \bibnamefont
  {Lee}}, \ and\ \bibinfo {author} {\bibfnamefont {Leonid~S.}\ \bibnamefont
  {Levitov}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Spin-filtered edge states and quantum hall effect in graphene},}\
  }\href {\doibase 10.1103/PhysRevLett.96.176803} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {96}},\
  \bibinfo {pages} {176803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Abanin}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Abanin}, \citenamefont {Lee},\
  and\ \citenamefont {Levitov}}]{ALL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abanin}, \bibfnamefont
  {Dmitry~A}}, \bibinfo {author} {\bibfnamefont {Patrick~A.}\ \bibnamefont
  {Lee}}, \ and\ \bibinfo {author} {\bibfnamefont {Leonid~S.}\ \bibnamefont
  {Levitov}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Charge and spin transport at the quantum hall
  edge of graphene},}\ }\href {\doibase 10.1016/j.ssc.2007.04.024} {\bibfield
  {journal} {\bibinfo  {journal} {Solid State Communications}\ }\textbf
  {\bibinfo {volume} {143}},\ \bibinfo {pages} {77 -- 85}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Abanin}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Abanin}, \citenamefont
  {Novoselov}, \citenamefont {Zeitler}, \citenamefont {Lee}, \citenamefont
  {Geim},\ and\ \citenamefont {Levitov}}]{ANZLGL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abanin}, \bibfnamefont
  {Dmitry~A}}, \bibinfo {author} {\bibfnamefont {Kostya~S.}\ \bibnamefont
  {Novoselov}}, \bibinfo {author} {\bibfnamefont {Uli}\ \bibnamefont
  {Zeitler}}, \bibinfo {author} {\bibfnamefont {Patrick~A.}\ \bibnamefont
  {Lee}}, \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}, \
  and\ \bibinfo {author} {\bibfnamefont {L.~S.}\ \bibnamefont {Levitov}}}
  (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Dissipative quantum hall effect in graphene near the dirac
  point},}\ }\href {\doibase 10.1103/PhysRevLett.98.196806} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {98}},\ \bibinfo {pages} {196806}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Abedpour}\ \emph {et~al.}(2007)\citenamefont
  {Abedpour}, \citenamefont {Neek-Amal}, \citenamefont {Asgari}, \citenamefont
  {Shahbazi}, \citenamefont {Nafari},\ and\ \citenamefont {Tabar}}]{ANASNT07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abedpour},
  \bibfnamefont {N}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Neek-Amal}}, \bibinfo {author} {\bibfnamefont {Reza}\ \bibnamefont
  {Asgari}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Shahbazi}},
  \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Nafari}}, \ and\ \bibinfo
  {author} {\bibfnamefont {M.~Reza~Rahimi}\ \bibnamefont {Tabar}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Roughness of
  undoped graphene and its short-range induced gauge field},}\ }\href {\doibase
  10.1103/PhysRevB.76.195407} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {195407}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Abergel}\ \emph {et~al.}(2007)\citenamefont
  {Abergel}, \citenamefont {Russell},\ and\ \citenamefont {Fal'ko}}]{ARF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abergel}, \bibfnamefont
  {D~S~L}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Russell}}, \
  and\ \bibinfo {author} {\bibfnamefont {Vladimir~I.}\ \bibnamefont {Fal'ko}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Visibility of graphene flakes on a dielectric substrate},}\ }\href {\doibase
  10.1063/1.2768625} {\bibfield  {journal} {\bibinfo  {journal} {Applied
  Physics Letters}\ }\textbf {\bibinfo {volume} {91}}~(\bibinfo {number} {6}),\
  \bibinfo {eid} {063125}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Abrikosov}(1998)}]{Abrikosov98}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Abrikosov},
  \bibfnamefont {A~A}}} (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Quantum magnetoresistance},}\ }\href {\doibase
  10.1103/PhysRevB.58.2788} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {58}},\ \bibinfo {pages}
  {2788--2794}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Adam}\ \emph {et~al.}(2007)\citenamefont {Adam},
  \citenamefont {Hwang}, \citenamefont {Galitski},\ and\ \citenamefont
  {Das~Sarma}}]{AHGS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Adam}, \bibfnamefont
  {Shaffique}}, \bibinfo {author} {\bibfnamefont {E.~H.}\ \bibnamefont
  {Hwang}}, \bibinfo {author} {\bibfnamefont {V.~M.}\ \bibnamefont {Galitski}},
  \ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Das~Sarma}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {A
  self-consistent theory for graphene transport},}\ }\href {\doibase
  10.1073/pnas.0704772104} {\bibfield  {journal} {\bibinfo  {journal}
  {Proceedings of the National Academy of Sciences}\ }\textbf {\bibinfo
  {volume} {104}}~(\bibinfo {number} {47}),\ \bibinfo {pages}
  {18392--18397}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Affoune}\ \emph {et~al.}(2001)\citenamefont
  {Affoune}, \citenamefont {Prasad}, \citenamefont {Sato}, \citenamefont
  {Enoki}, \citenamefont {Kaburagi},\ and\ \citenamefont
  {Hishiyama}}]{Affoune01}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Affoune}, \bibfnamefont
  {AM}}, \bibinfo {author} {\bibfnamefont {B.L.V}\ \bibnamefont {Prasad}},
  \bibinfo {author} {\bibfnamefont {Hirohiko}\ \bibnamefont {Sato}}, \bibinfo
  {author} {\bibfnamefont {Toshiaki}\ \bibnamefont {Enoki}}, \bibinfo {author}
  {\bibfnamefont {Yutaka}\ \bibnamefont {Kaburagi}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Yoshihiro}\ \bibnamefont {Hishiyama}}} (\bibinfo {year}
  {2001}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Experimental
  evidence of a single nano-graphene},}\ }\href {\doibase
  10.1016/S0009-2614(01)01066-1} {\bibfield  {journal} {\bibinfo  {journal}
  {Chemical Physics Letters}\ }\textbf {\bibinfo {volume} {348}}~(\bibinfo
  {number} {1--2}),\ \bibinfo {pages} {17--20}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Akhmerov}\ and\ \citenamefont
  {Beenakker}(2008)}]{AkBe07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Akhmerov},
  \bibfnamefont {A~R}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~W.~J.}\
  \bibnamefont {Beenakker}}} (\bibinfo {year} {2008}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Boundary conditions for dirac fermions on a
  terminated honeycomb lattice},}\ }\href {\doibase 10.1103/PhysRevB.77.085423}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {77}},\ \bibinfo {pages} {085423}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Aleiner}\ and\ \citenamefont {Efetov}(2006)}]{AE06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Aleiner}, \bibfnamefont
  {I~L}}, \ and\ \bibinfo {author} {\bibfnamefont {K.~B.}\ \bibnamefont
  {Efetov}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Effect of disorder on transport in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.97.236801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {236801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Alicea}\ and\ \citenamefont {Fisher}(2006)}]{AF06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Alicea}, \bibfnamefont
  {Jason}}, \ and\ \bibinfo {author} {\bibfnamefont {Matthew P.~A.}\
  \bibnamefont {Fisher}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Graphene integer quantum hall effect in the
  ferromagnetic and paramagnetic regimes},}\ }\href {\doibase
  10.1103/PhysRevB.74.075422} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo {pages}
  {075422}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Alicea}\ and\ \citenamefont {Fisher}(2007)}]{AF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Alicea}, \bibfnamefont
  {Jason}}, \ and\ \bibinfo {author} {\bibfnamefont {Matthew~P.A.}\
  \bibnamefont {Fisher}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Interplay between lattice-scale physics and the
  quantum hall effect in graphene},}\ }\href {\doibase
  10.1016/j.ssc.2007.06.035} {\bibfield  {journal} {\bibinfo  {journal} {Solid
  State Communications}\ }\textbf {\bibinfo {volume} {143}}~(\bibinfo {number}
  {11--12}),\ \bibinfo {pages} {504--509}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Altland}(2006)}]{A06c}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Altland}, \bibfnamefont
  {Alexander}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Low-energy theory of disordered graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.97.236802} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo
  {pages} {236802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(1974{\natexlab{a}})}]{Ando4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {1974}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Theory of quantum transport in a two-dimensional
  electron system under magnetic fields. iii. many-site approximation},}\
  }\href {\doibase 10.1143/JPSJ.37.622} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of the Physical Society of Japan}\ }\textbf {\bibinfo
  {volume} {37}}~(\bibinfo {number} {3}),\ \bibinfo {pages}
  {622--630}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(1974{\natexlab{b}})}]{Ando5}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {1974}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Theory of quantum transport in a two-dimensional
  electron system under magnetic fields. iv. oscillatory conductivity},}\
  }\href {\doibase 10.1143/JPSJ.37.1233} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of the Physical Society of Japan}\ }\textbf {\bibinfo
  {volume} {37}}~(\bibinfo {number} {5}),\ \bibinfo {pages}
  {1233--1237}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(1975)}]{Ando6}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {1975}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Theory of cyclotron resonance lineshape in a two-dimensional
  electron system},}\ }\href {\doibase 10.1143/JPSJ.38.989} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {38}}~(\bibinfo {number} {4}),\ \bibinfo {pages}
  {989--997}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(2000)}]{A00}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {2000}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Spin-orbit interaction in carbon nanotubes},}\ }\href {\doibase
  10.1143/JPSJ.69.1757} {\bibfield  {journal} {\bibinfo  {journal} {Journal of
  the Physical Society of Japan}\ }\textbf {\bibinfo {volume} {69}}~(\bibinfo
  {number} {6}),\ \bibinfo {pages} {1757--1763}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(2006{\natexlab{a}})}]{ando_opt}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Anomaly of optical phonon in monolayer
  graphene},}\ }\href {\doibase 10.1143/JPSJ.75.124701} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of the Physical Society of Japan}\ }\textbf
  {\bibinfo {volume} {75}}~(\bibinfo {number} {12}),\ \bibinfo {pages}
  {124701}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(2006{\natexlab{b}})}]{A06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {2006}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Screening effect and impurity scattering in
  monolayer graphene},}\ }\href {\doibase 10.1143/JPSJ.75.074716} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {75}}~(\bibinfo {number} {7}),\ \bibinfo {pages}
  {074716}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(2007{\natexlab{a}})}]{ando_opt_bi}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Anomaly of optical phonons in bilayer
  graphene},}\ }\href {\doibase 10.1143/JPSJ.76.104711} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of the Physical Society of Japan}\ }\textbf
  {\bibinfo {volume} {76}}~(\bibinfo {number} {10}),\ \bibinfo {pages}
  {104711}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}(2007{\natexlab{b}})}]{A07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Magnetic oscillation of optical phonon in
  graphene},}\ }\href {\doibase 10.1143/JPSJ.76.024712} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of the Physical Society of Japan}\ }\textbf
  {\bibinfo {volume} {76}}~(\bibinfo {number} {2}),\ \bibinfo {pages}
  {024712}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}\ \emph {et~al.}(1998)\citenamefont {Ando},
  \citenamefont {Nakanishi},\ and\ \citenamefont {Saito}}]{ANS98}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}, \bibinfo {author} {\bibfnamefont {Takeshi}\ \bibnamefont
  {Nakanishi}}, \ and\ \bibinfo {author} {\bibfnamefont {Riichiro}\
  \bibnamefont {Saito}}} (\bibinfo {year} {1998}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Berry's phase and absence of back scattering \\
  in carbon nanotubes},}\ }\href {\doibase 10.1143/JPSJ.67.2857} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {67}}~(\bibinfo {number} {8}),\ \bibinfo {pages}
  {2857--2862}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}\ and\ \citenamefont {Uemura}(1974)}]{Ando1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}, \ and\ \bibinfo {author} {\bibfnamefont {Yasutada}\ \bibnamefont
  {Uemura}}} (\bibinfo {year} {1974}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Theory of quantum transport in a two-dimensional electron system
  under magnetic fields. i. characteristics of level broadening and transport
  under strong fields},}\ }\href {\doibase 10.1143/JPSJ.36.959} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of the Physical Society of Japan}\
  }\textbf {\bibinfo {volume} {36}}~(\bibinfo {number} {4}),\ \bibinfo {pages}
  {959--967}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ando}\ \emph {et~al.}(2002)\citenamefont {Ando},
  \citenamefont {Zheng},\ and\ \citenamefont {Suzuura}}]{Ando8}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ando}, \bibfnamefont
  {Tsuneya}}, \bibinfo {author} {\bibfnamefont {Yisong}\ \bibnamefont {Zheng}},
  \ and\ \bibinfo {author} {\bibfnamefont {Hidekatsu}\ \bibnamefont {Suzuura}}}
  (\bibinfo {year} {2002}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Dynamical conductivity and zero-mode anomaly in honeycomb lattices},}\
  }\href {\doibase 10.1143/JPSJ.71.1318} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of the Physical Society of Japan}\ }\textbf {\bibinfo
  {volume} {71}}~(\bibinfo {number} {5}),\ \bibinfo {pages}
  {1318--1324}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Andreoni}(2000)}]{fullerenes}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Andreoni},
  \bibfnamefont {W}}} (\bibinfo {year} {2000}),\ \href@noop {} {\emph {\bibinfo
  {title} {The Physics of Fullerene-Based and Fullerene-related materials}}}\
  (\bibinfo  {publisher} {Springer})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Areshkin}\ \emph {et~al.}(2007)\citenamefont
  {Areshkin}, \citenamefont {Gunlycke},\ and\ \citenamefont {White}}]{AW07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Areshkin},
  \bibfnamefont {Denis~A}}, \bibinfo {author} {\bibfnamefont {Daniel}\
  \bibnamefont {Gunlycke}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Carter~T.}\ \bibnamefont {White}}} (\bibinfo {year} {2007}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Ballistic transport in graphene
  nanostrips in the presence of disorder: Importance of edge effects},}\ }\href
  {\doibase 10.1021/nl062132h} {\bibfield  {journal} {\bibinfo  {journal} {Nano
  Letters}\ }\textbf {\bibinfo {volume} {7}}~(\bibinfo {number} {1}),\ \bibinfo
  {pages} {204--210}},\ \bibinfo {note} {pMID: 17212465}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ashcroft}\ and\ \citenamefont
  {Mermin}(1976)}]{Ashcroft}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ashcroft},
  \bibfnamefont {NW}}, \ and\ \bibinfo {author} {\bibfnamefont {N.D.}\
  \bibnamefont {Mermin}}} (\bibinfo {year} {1976}),\ \href@noop {} {\emph
  {\bibinfo {title} {Solid State Physics}}}\ (\bibinfo  {publisher} {Saunders
  College},\ \bibinfo {address} {Philadelphia, PA})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Baeriswyl}\ \emph {et~al.}(1986)\citenamefont
  {Baeriswyl}, \citenamefont {Campbell},\ and\ \citenamefont
  {Mazumdar}}]{Baeriswyl86}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Baeriswyl},
  \bibfnamefont {Dionys}}, \bibinfo {author} {\bibfnamefont {David~K.}\
  \bibnamefont {Campbell}}, \ and\ \bibinfo {author} {\bibfnamefont {Sumit}\
  \bibnamefont {Mazumdar}}} (\bibinfo {year} {1986}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Correlations and defect energies},}\ }\href
  {\doibase 10.1103/PhysRevLett.56.1509} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {56}},\ \bibinfo
  {pages} {1509--1509}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bak}(1982)}]{Bak82}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bak}, \bibfnamefont
  {P}}} (\bibinfo {year} {1982}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Commensurate phases, incommensurate phases and the devil's
  staircase},}\ }\href {http://stacks.iop.org/0034-4885/45/i=6/a=001}
  {\bibfield  {journal} {\bibinfo  {journal} {Reports on Progress in Physics}\
  }\textbf {\bibinfo {volume} {45}}~(\bibinfo {number} {6}),\ \bibinfo {pages}
  {587}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Balatsky}\ \emph {et~al.}(2006)\citenamefont
  {Balatsky}, \citenamefont {Vekhter},\ and\ \citenamefont {Zhu}}]{BVZ06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Balatsky},
  \bibfnamefont {A~V}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont
  {Vekhter}}, \ and\ \bibinfo {author} {\bibfnamefont {Jian-Xin}\ \bibnamefont
  {Zhu}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Impurity-induced states in conventional and unconventional
  superconductors},}\ }\href {\doibase 10.1103/RevModPhys.78.373} {\bibfield
  {journal} {\bibinfo  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume}
  {78}},\ \bibinfo {pages} {373--433}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bardarson}\ \emph {et~al.}(2007)\citenamefont
  {Bardarson}, \citenamefont {Tworzyd\l{}o}, \citenamefont {Brouwer},\ and\
  \citenamefont {Beenakker}}]{BTBB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bardarson},
  \bibfnamefont {J~H}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Tworzyd\l{}o}}, \bibinfo {author} {\bibfnamefont {P.~W.}\ \bibnamefont
  {Brouwer}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont
  {Beenakker}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {One-parameter scaling at the dirac point in graphene},}\
  }\href {\doibase 10.1103/PhysRevLett.99.106801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\
  \bibinfo {pages} {106801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Barlas}\ \emph {et~al.}(2007)\citenamefont {Barlas},
  \citenamefont {Pereg-Barnea}, \citenamefont {Polini}, \citenamefont
  {Asgari},\ and\ \citenamefont {MacDonald}}]{BPPAM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Barlas}, \bibfnamefont
  {Yafis}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Pereg-Barnea}},
  \bibinfo {author} {\bibfnamefont {Marco}\ \bibnamefont {Polini}}, \bibinfo
  {author} {\bibfnamefont {Reza}\ \bibnamefont {Asgari}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~H.}\ \bibnamefont {MacDonald}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Chirality and
  correlations in graphene},}\ }\href {\doibase 10.1103/PhysRevLett.98.236601}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {98}},\ \bibinfo {pages} {236601}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Barone}\ \emph {et~al.}(2006)\citenamefont {Barone},
  \citenamefont {Hod},\ and\ \citenamefont {Scuseria}}]{BHS06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Barone}, \bibfnamefont
  {Veronica}}, \bibinfo {author} {\bibfnamefont {Oded}\ \bibnamefont {Hod}}, \
  and\ \bibinfo {author} {\bibfnamefont {Gustavo~E.}\ \bibnamefont {Scuseria}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic structure and stability of semiconducting graphene
  nanoribbons},}\ }\href {\doibase 10.1021/nl0617033} {\bibfield  {journal}
  {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo {volume}
  {6}}~(\bibinfo {number} {12}),\ \bibinfo {pages} {2748--2754}},\ \bibinfo
  {note} {pMID: 17163699}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Baym}(1969)}]{Baym}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Baym}, \bibfnamefont
  {G}}} (\bibinfo {year} {1969}),\ \href@noop {} {\emph {\bibinfo {title}
  {Lectures on Quantum Mechanics}}}\ (\bibinfo  {publisher} {Benjamin, New
  York})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bena}\ and\ \citenamefont {Kivelson}(2005)}]{BK05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bena}, \bibfnamefont
  {Cristina}}, \ and\ \bibinfo {author} {\bibfnamefont {Steven~A.}\
  \bibnamefont {Kivelson}}} (\bibinfo {year} {2005}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Quasiparticle scattering and local density of
  states in graphite},}\ }\href {\doibase 10.1103/PhysRevB.72.125432}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {72}},\ \bibinfo {pages} {125432}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Berger}\ \emph {et~al.}(2004)\citenamefont {Berger},
  \citenamefont {Song}, \citenamefont {Li}, \citenamefont {Li}, \citenamefont
  {Ogbazghi}, \citenamefont {Feng}, \citenamefont {Dai}, \citenamefont
  {Marchenkov}, \citenamefont {Conrad}, \citenamefont {First},\ and\
  \citenamefont {de~Heer}}]{Betal04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Berger}, \bibfnamefont
  {Claire}}, \bibinfo {author} {\bibfnamefont {Zhimin}\ \bibnamefont {Song}},
  \bibinfo {author} {\bibfnamefont {Tianbo}\ \bibnamefont {Li}}, \bibinfo
  {author} {\bibfnamefont {Xuebin}\ \bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {Asmerom~Y.}\ \bibnamefont {Ogbazghi}}, \bibinfo {author}
  {\bibfnamefont {Rui}\ \bibnamefont {Feng}}, \bibinfo {author} {\bibfnamefont
  {Zhenting}\ \bibnamefont {Dai}}, \bibinfo {author} {\bibfnamefont
  {Alexei~N.}\ \bibnamefont {Marchenkov}}, \bibinfo {author} {\bibfnamefont
  {Edward~H.}\ \bibnamefont {Conrad}}, \bibinfo {author} {\bibfnamefont
  {Phillip~N.}\ \bibnamefont {First}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Walt~A.}\ \bibnamefont {de~Heer}}} (\bibinfo {year} {2004}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Ultrathin epitaxial graphite: 2d
  electron gas properties and a route toward graphene-based nanoelectronics},}\
  }\href {\doibase 10.1021/jp040650f} {\bibfield  {journal} {\bibinfo
  {journal} {The Journal of Physical Chemistry B}\ }\textbf {\bibinfo {volume}
  {108}}~(\bibinfo {number} {52}),\ \bibinfo {pages}
  {19912--19916}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Berger}\ \emph {et~al.}(2006)\citenamefont {Berger},
  \citenamefont {Song}, \citenamefont {Li}, \citenamefont {Wu}, \citenamefont
  {Brown}, \citenamefont {Naud}, \citenamefont {Mayou}, \citenamefont {Li},
  \citenamefont {Hass}, \citenamefont {Marchenkov}, \citenamefont {Conrad},
  \citenamefont {First},\ and\ \citenamefont {de~Heer}}]{Betal06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Berger}, \bibfnamefont
  {Claire}}, \bibinfo {author} {\bibfnamefont {Zhimin}\ \bibnamefont {Song}},
  \bibinfo {author} {\bibfnamefont {Xuebin}\ \bibnamefont {Li}}, \bibinfo
  {author} {\bibfnamefont {Xiaosong}\ \bibnamefont {Wu}}, \bibinfo {author}
  {\bibfnamefont {Nate}\ \bibnamefont {Brown}}, \bibinfo {author}
  {\bibfnamefont {C{\'e}cile}\ \bibnamefont {Naud}}, \bibinfo {author}
  {\bibfnamefont {Didier}\ \bibnamefont {Mayou}}, \bibinfo {author}
  {\bibfnamefont {Tianbo}\ \bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont
  {Joanna}\ \bibnamefont {Hass}}, \bibinfo {author} {\bibfnamefont {Alexei~N.}\
  \bibnamefont {Marchenkov}}, \bibinfo {author} {\bibfnamefont {Edward~H.}\
  \bibnamefont {Conrad}}, \bibinfo {author} {\bibfnamefont {Phillip~N.}\
  \bibnamefont {First}}, \ and\ \bibinfo {author} {\bibfnamefont {Walt~A.}\
  \bibnamefont {de~Heer}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic confinement and coherence in
  patterned epitaxial graphene},}\ }\href {\doibase 10.1126/science.1125925}
  {\bibfield  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo
  {volume} {312}}~(\bibinfo {number} {5777}),\ \bibinfo {pages}
  {1191--1196}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bergmann}(1984)}]{B84}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bergmann},
  \bibfnamefont {Gerd}}} (\bibinfo {year} {1984}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Weak localization in thin films: a
  time-of-flight experiment with conduction electrons},}\ }\href {\doibase
  10.1016/0370-1573(84)90103-0} {\bibfield  {journal} {\bibinfo  {journal}
  {Physics Reports}\ }\textbf {\bibinfo {volume} {107}}~(\bibinfo {number}
  {1}),\ \bibinfo {pages} {1--58}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bernevig}\ \emph {et~al.}(2007)\citenamefont
  {Bernevig}, \citenamefont {Hughes}, \citenamefont {Raghu},\ and\
  \citenamefont {Arovas}}]{BHRA07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bernevig},
  \bibfnamefont {B~Andrei}}, \bibinfo {author} {\bibfnamefont {Taylor~L.}\
  \bibnamefont {Hughes}}, \bibinfo {author} {\bibfnamefont {Srinivas}\
  \bibnamefont {Raghu}}, \ and\ \bibinfo {author} {\bibfnamefont {Daniel~P.}\
  \bibnamefont {Arovas}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Theory of the three-dimensional quantum hall
  effect in graphite},}\ }\href {\doibase 10.1103/PhysRevLett.99.146804}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {99}},\ \bibinfo {pages} {146804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Berry}\ and\ \citenamefont {Mondragon}(1987)}]{BM87}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Berry}, \bibfnamefont
  {M~V}}, \ and\ \bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont
  {Mondragon}}} (\bibinfo {year} {1987}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Neutrino billiards: Time-reversal symmetry-breaking
  without magnetic fields},}\ }\href {\doibase 10.1098/rspa.1987.0080}
  {\bibfield  {journal} {\bibinfo  {journal} {Proceedings of the Royal Society
  of London. A. Mathematical and Physical Sciences}\ }\textbf {\bibinfo
  {volume} {412}}~(\bibinfo {number} {1842}),\ \bibinfo {pages}
  {53--74}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bhattacharjee}\ and\ \citenamefont
  {Sengupta}(2006)}]{BS06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bhattacharjee},
  \bibfnamefont {Subhro}}, \ and\ \bibinfo {author} {\bibfnamefont
  {K.}~\bibnamefont {Sengupta}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Tunneling conductance of graphene nis
  junctions},}\ }\href {\doibase 10.1103/PhysRevLett.97.217001} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {97}},\ \bibinfo {pages} {217001}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Birrell}\ and\ \citenamefont {Davies}(1982)}]{BD82}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Birrell}, \bibfnamefont
  {ND}}, \ and\ \bibinfo {author} {\bibfnamefont {P.C.W.}\ \bibnamefont
  {Davies}}} (\bibinfo {year} {1982}),\ \href@noop {} {\emph {\bibinfo {title}
  {Quantum Fields in Curved Space}}}\ (\bibinfo  {publisher} {Cambridge Univ.
  Press, Cambridge})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Biswas}\ \emph {et~al.}(2007)\citenamefont {Biswas},
  \citenamefont {Sachdev},\ and\ \citenamefont {Son}}]{BSS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Biswas}, \bibfnamefont
  {Rudro~R}}, \bibinfo {author} {\bibfnamefont {Subir}\ \bibnamefont
  {Sachdev}}, \ and\ \bibinfo {author} {\bibfnamefont {Dam~T.}\ \bibnamefont
  {Son}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Coulomb impurity in graphene},}\ }\href {\doibase
  10.1103/PhysRevB.76.205122} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {205122}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Blake}\ \emph {et~al.}(2007)\citenamefont {Blake},
  \citenamefont {Hill}, \citenamefont {Neto}, \citenamefont {Novoselov},
  \citenamefont {Jiang}, \citenamefont {Yang}, \citenamefont {Booth},\ and\
  \citenamefont {Geim}}]{blake07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Blake}, \bibfnamefont
  {P}}, \bibinfo {author} {\bibfnamefont {E.~W.}\ \bibnamefont {Hill}},
  \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\ \bibnamefont {Neto}},
  \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Jiang}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Yang}}, \bibinfo {author} {\bibfnamefont
  {T.~J.}\ \bibnamefont {Booth}}, \ and\ \bibinfo {author} {\bibfnamefont
  {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Making graphene visible},}\ }\href {\doibase
  10.1063/1.2768624} {\bibfield  {journal} {\bibinfo  {journal} {Applied
  Physics Letters}\ }\textbf {\bibinfo {volume} {91}}~(\bibinfo {number} {6}),\
  \bibinfo {eid} {063124}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bliokh}(2005)}]{B05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bliokh}, \bibfnamefont
  {KYu}}} (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Weak antilocalization of ultrarelativistic fermions},}\ }\href
  {\doibase 10.1016/j.physleta.2005.06.062} {\bibfield  {journal} {\bibinfo
  {journal} {Physics Letters A}\ }\textbf {\bibinfo {volume} {344}},\ \bibinfo
  {pages} {127 -- 130}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bommel}\ \emph {et~al.}(1975)\citenamefont {Bommel},
  \citenamefont {Crombeen},\ and\ \citenamefont {Tooren}}]{VCV75}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bommel}, \bibfnamefont
  {AJ~Van}}, \bibinfo {author} {\bibfnamefont {J.E.}\ \bibnamefont {Crombeen}},
  \ and\ \bibinfo {author} {\bibfnamefont {A.~Van}\ \bibnamefont {Tooren}}}
  (\bibinfo {year} {1975}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Leed and auger electron observations of the sic(0001) surface},}\ }\href
  {\doibase 10.1016/0039-6028(75)90419-7} {\bibfield  {journal} {\bibinfo
  {journal} {Surface Science}\ }\textbf {\bibinfo {volume} {48}}~(\bibinfo
  {number} {2}),\ \bibinfo {pages} {463 -- 472}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bonini}\ \emph {et~al.}(2007)\citenamefont {Bonini},
  \citenamefont {Lazzeri}, \citenamefont {Marzari},\ and\ \citenamefont
  {Mauri}}]{BLMM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bonini}, \bibfnamefont
  {Nicola}}, \bibinfo {author} {\bibfnamefont {Michele}\ \bibnamefont
  {Lazzeri}}, \bibinfo {author} {\bibfnamefont {Nicola}\ \bibnamefont
  {Marzari}}, \ and\ \bibinfo {author} {\bibfnamefont {Francesco}\ \bibnamefont
  {Mauri}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Phonon anharmonicities in graphite and graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.99.176802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {176802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Booth}\ \emph {et~al.}(2008)\citenamefont {Booth},
  \citenamefont {Blake}, \citenamefont {Nair}, \citenamefont {Jiang},
  \citenamefont {Hill}, \citenamefont {Bangert}, \citenamefont {Bleloch},
  \citenamefont {Gass}, \citenamefont {Novoselov}, \citenamefont {Katsnelson},\
  and\ \citenamefont {Geim}}]{BOMESHR07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Booth}, \bibfnamefont
  {Tim~J}}, \bibinfo {author} {\bibfnamefont {Peter}\ \bibnamefont {Blake}},
  \bibinfo {author} {\bibfnamefont {Rahul~R.}\ \bibnamefont {Nair}}, \bibinfo
  {author} {\bibfnamefont {Da}~\bibnamefont {Jiang}}, \bibinfo {author}
  {\bibfnamefont {Ernie~W.}\ \bibnamefont {Hill}}, \bibinfo {author}
  {\bibfnamefont {Ursel}\ \bibnamefont {Bangert}}, \bibinfo {author}
  {\bibfnamefont {Andrew}\ \bibnamefont {Bleloch}}, \bibinfo {author}
  {\bibfnamefont {Mhairi}\ \bibnamefont {Gass}}, \bibinfo {author}
  {\bibfnamefont {Kostya~S.}\ \bibnamefont {Novoselov}}, \bibinfo {author}
  {\bibfnamefont {M.~I.}\ \bibnamefont {Katsnelson}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year} {2008}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Macroscopic graphene
  membranes and their extraordinary stiffness},}\ }\href {\doibase
  10.1021/nl801412y} {\bibfield  {journal} {\bibinfo  {journal} {Nano Letters}\
  }\textbf {\bibinfo {volume} {8}}~(\bibinfo {number} {8}),\ \bibinfo {pages}
  {2442--2446}},\ \bibinfo {note} {pMID: 18593201}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Boyle}\ and\ \citenamefont
  {Nozi\`eres}(1958)}]{BN58}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Boyle}, \bibfnamefont
  {W~S}}, \ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Nozi\`eres}}} (\bibinfo {year} {1958}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Band structure and infrared absorption of graphite},}\
  }\href {\doibase 10.1103/PhysRev.111.782} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {111}},\ \bibinfo {pages}
  {782--785}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Brey}\ and\ \citenamefont
  {Fertig}(2006{\natexlab{a}})}]{Brey206}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Brey}, \bibfnamefont
  {L}}, \ and\ \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont
  {Fertig}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic states of graphene nanoribbons
  studied with the dirac equation},}\ }\href {\doibase
  10.1103/PhysRevB.73.235411} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo {pages}
  {235411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Brey}\ \emph {et~al.}(2007)\citenamefont {Brey},
  \citenamefont {Fertig},\ and\ \citenamefont {Das~Sarma}}]{BFS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Brey}, \bibfnamefont
  {L}}, \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont {Fertig}}, \
  and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Das~Sarma}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Diluted graphene antiferromagnet},}\ }\href {\doibase
  10.1103/PhysRevLett.99.116802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {116802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Brey}\ and\ \citenamefont
  {Fertig}(2006{\natexlab{b}})}]{Brey106}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Brey}, \bibfnamefont
  {Luis}}, \ and\ \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont
  {Fertig}}} (\bibinfo {year} {2006}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Edge states and the quantized hall effect in
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.73.195408} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {73}},\ \bibinfo {pages} {195408}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bunch}\ \emph {et~al.}(2007)\citenamefont {Bunch},
  \citenamefont {van~der Zande}, \citenamefont {Verbridge}, \citenamefont
  {Frank}, \citenamefont {Tanenbaum}, \citenamefont {Parpia}, \citenamefont
  {Craighead},\ and\ \citenamefont {McEuen}}]{bunch07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Bunch}, \bibfnamefont
  {J~Scott}}, \bibinfo {author} {\bibfnamefont {Arend~M.}\ \bibnamefont
  {van~der Zande}}, \bibinfo {author} {\bibfnamefont {Scott~S.}\ \bibnamefont
  {Verbridge}}, \bibinfo {author} {\bibfnamefont {Ian~W.}\ \bibnamefont
  {Frank}}, \bibinfo {author} {\bibfnamefont {David~M.}\ \bibnamefont
  {Tanenbaum}}, \bibinfo {author} {\bibfnamefont {Jeevak~M.}\ \bibnamefont
  {Parpia}}, \bibinfo {author} {\bibfnamefont {Harold~G.}\ \bibnamefont
  {Craighead}}, \ and\ \bibinfo {author} {\bibfnamefont {Paul~L.}\ \bibnamefont
  {McEuen}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electromechanical resonators from graphene sheets},}\ }\href
  {\doibase 10.1126/science.1136836} {\bibfield  {journal} {\bibinfo  {journal}
  {Science}\ }\textbf {\bibinfo {volume} {315}}~(\bibinfo {number} {5811}),\
  \bibinfo {pages} {490--493}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Calandra}\ and\ \citenamefont {Mauri}(2007)}]{CM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Calandra},
  \bibfnamefont {Matteo}}, \ and\ \bibinfo {author} {\bibfnamefont {Francesco}\
  \bibnamefont {Mauri}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Publisher's note: Electronic structure of
  heavily doped graphene: The role of foreign atom states [phys. rev. b 76,
  161406 (2007)]},}\ }\href {\doibase 10.1103/PhysRevB.76.199901} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {199901}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Calizo}\ \emph {et~al.}(2007)\citenamefont {Calizo},
  \citenamefont {Bao}, \citenamefont {Miao}, \citenamefont {Lau},\ and\
  \citenamefont {Balandin}}]{CBMLB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Calizo}, \bibfnamefont
  {Irene}}, \bibinfo {author} {\bibfnamefont {Wenzhong}\ \bibnamefont {Bao}},
  \bibinfo {author} {\bibfnamefont {Feng}\ \bibnamefont {Miao}}, \bibinfo
  {author} {\bibfnamefont {Chun~Ning}\ \bibnamefont {Lau}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Alexander~A.}\ \bibnamefont {Balandin}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {The effect
  of substrates on the raman spectrum of graphene: Graphene- on-sapphire and
  graphene-on-glass},}\ }\href {\doibase 10.1063/1.2805024} {\bibfield
  {journal} {\bibinfo  {journal} {Applied Physics Letters}\ }\textbf {\bibinfo
  {volume} {91}}~(\bibinfo {number} {20}),\ \bibinfo {eid}
  {201904}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Calogeracos}\ and\ \citenamefont
  {Dombey}(1999)}]{calogeracos99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Calogeracos},
  \bibfnamefont {A}}, \ and\ \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Dombey}}} (\bibinfo {year} {1999}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {History and physics of the klein paradox},}\ }\href {\doibase
  10.1080/001075199181387} {\bibfield  {journal} {\bibinfo  {journal}
  {Contemporary Physics}\ }\textbf {\bibinfo {volume} {40}}~(\bibinfo {number}
  {5}),\ \bibinfo {pages} {313--321}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Campagnoli}\ and\ \citenamefont
  {Tosatti}(1989)}]{CT89}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Campagnoli},
  \bibfnamefont {G}}, \ and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Tosatti}}} (\bibinfo {year} {1989}),\ \href@noop {} {\emph {\bibinfo {title}
  {Progress on Electron Properties of Metals}}},\ edited by\ \bibinfo {editor}
  {\bibfnamefont {R.}~\bibnamefont {Girlinda}}\ (\bibinfo  {publisher} {Kluwer
  Academic Publishing})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Casiraghi}\ \emph {et~al.}(2007)\citenamefont
  {Casiraghi}, \citenamefont {Hartschuh}, \citenamefont {Lidorikis},
  \citenamefont {Qian}, \citenamefont {Harutyunyan}, \citenamefont {Gokus},
  \citenamefont {Novoselov},\ and\ \citenamefont {Ferrari}}]{CHLQHGNF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Casiraghi},
  \bibfnamefont {C}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Hartschuh}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {Lidorikis}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Qian}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Harutyunyan}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Gokus}}, \bibinfo {author}
  {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~C.}\ \bibnamefont {Ferrari}}} (\bibinfo {year} {2007}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Rayleigh imaging of graphene
  and graphene layers},}\ }\href {\doibase 10.1021/nl071168m} {\bibfield
  {journal} {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo {volume}
  {7}}~(\bibinfo {number} {9}),\ \bibinfo {pages} {2711--2717}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Cassanello}\ and\ \citenamefont
  {Fradkin}(1996)}]{CF96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cassanello},
  \bibfnamefont {Carlos~R}}, \ and\ \bibinfo {author} {\bibfnamefont {Eduardo}\
  \bibnamefont {Fradkin}}} (\bibinfo {year} {1996}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Kondo effect in flux phases},}\ }\href {\doibase
  10.1103/PhysRevB.53.15079} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {53}},\ \bibinfo {pages}
  {15079--15094}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cassanello}\ and\ \citenamefont
  {Fradkin}(1997)}]{CF97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cassanello},
  \bibfnamefont {Carlos~R}}, \ and\ \bibinfo {author} {\bibfnamefont {Eduardo}\
  \bibnamefont {Fradkin}}} (\bibinfo {year} {1997}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Overscreening of magnetic impurities in
  ${d}_{{x}^{2}-{y}^{2}}$-wave superconductors},}\ }\href {\doibase
  10.1103/PhysRevB.56.11246} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {56}},\ \bibinfo {pages}
  {11246--11261}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Castillo}\ \emph {et~al.}(1997)\citenamefont
  {Castillo}, \citenamefont {de~C.~Chamon}, \citenamefont {Fradkin},
  \citenamefont {Goldbart},\ and\ \citenamefont {Mudry}}]{CCFGM97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Castillo},
  \bibfnamefont {Horacio~E}}, \bibinfo {author} {\bibfnamefont {Claudio}\
  \bibnamefont {de~C.~Chamon}}, \bibinfo {author} {\bibfnamefont {Eduardo}\
  \bibnamefont {Fradkin}}, \bibinfo {author} {\bibfnamefont {Paul~M.}\
  \bibnamefont {Goldbart}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Christopher}\ \bibnamefont {Mudry}}} (\bibinfo {year} {1997}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Exact calculation of multifractal
  exponents of the critical wave function of dirac fermions in a random
  magnetic field},}\ }\href {\doibase 10.1103/PhysRevB.56.10668} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {56}},\ \bibinfo {pages} {10668--10677}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Castro}\ \emph {et~al.}(2008)\citenamefont {Castro},
  \citenamefont {Peres}, \citenamefont {Lopes~dos Santos}, \citenamefont
  {Neto},\ and\ \citenamefont {Guinea}}]{Cetal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Castro}, \bibfnamefont
  {Eduardo~V}}, \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont
  {Peres}}, \bibinfo {author} {\bibfnamefont {J.~M.~B.}\ \bibnamefont
  {Lopes~dos Santos}}, \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\
  \bibnamefont {Neto}}, \ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Guinea}}} (\bibinfo {year} {2008}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Localized states at zigzag edges of bilayer
  graphene},}\ }\href {\doibase 10.1103/PhysRevLett.100.026802} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {100}},\ \bibinfo {pages} {026802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Castro~Neto}\ \emph {et~al.}(2006)\citenamefont
  {Castro~Neto}, \citenamefont {Guinea},\ and\ \citenamefont {Peres}}]{NGP06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Castro~Neto},
  \bibfnamefont {A~H}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont
  {Peres}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Edge and surface states in the quantum hall effect in graphene},}\
  }\href {\doibase 10.1103/PhysRevB.73.205408} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo
  {pages} {205408}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Can\ifmmode~\mbox{\c{c}}\else \c{c}\fi{}ado}\ \emph
  {et~al.}(2004)\citenamefont {Can\ifmmode~\mbox{\c{c}}\else \c{c}\fi{}ado},
  \citenamefont {Pimenta}, \citenamefont {Neves}, \citenamefont
  {Medeiros-Ribeiro}, \citenamefont {Enoki}, \citenamefont {Kobayashi},
  \citenamefont {Takai}, \citenamefont {Fukui}, \citenamefont {Dresselhaus},
  \citenamefont {Saito},\ and\ \citenamefont {Jorio}}]{Cancado04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont
  {Can\ifmmode~\mbox{\c{c}}\else \c{c}\fi{}ado}, \bibfnamefont {L~G}}, \bibinfo
  {author} {\bibfnamefont {M.~A.}\ \bibnamefont {Pimenta}}, \bibinfo {author}
  {\bibfnamefont {B.~R.~A.}\ \bibnamefont {Neves}}, \bibinfo {author}
  {\bibfnamefont {G.}~\bibnamefont {Medeiros-Ribeiro}}, \bibinfo {author}
  {\bibfnamefont {Toshiaki}\ \bibnamefont {Enoki}}, \bibinfo {author}
  {\bibfnamefont {Yousuke}\ \bibnamefont {Kobayashi}}, \bibinfo {author}
  {\bibfnamefont {Kazuyuki}\ \bibnamefont {Takai}}, \bibinfo {author}
  {\bibfnamefont {Ken-ichi}\ \bibnamefont {Fukui}}, \bibinfo {author}
  {\bibfnamefont {M.~S.}\ \bibnamefont {Dresselhaus}}, \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Saito}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Jorio}}} (\bibinfo {year} {2004}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Anisotropy of the raman
  spectra of nanographite ribbons},}\ }\href {\doibase
  10.1103/PhysRevLett.93.047403} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {93}},\ \bibinfo {pages}
  {047403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chakravarty}\ and\ \citenamefont
  {Schmid}(1986)}]{CS86}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Chakravarty},
  \bibfnamefont {Sudip}}, \ and\ \bibinfo {author} {\bibfnamefont {Albert}\
  \bibnamefont {Schmid}}} (\bibinfo {year} {1986}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Weak localization: The quasiclassical theory of
  electrons in a random potential},}\ }\href {\doibase
  10.1016/0370-1573(86)90027-X} {\bibfield  {journal} {\bibinfo  {journal}
  {Physics Reports}\ }\textbf {\bibinfo {volume} {140}}~(\bibinfo {number}
  {4}),\ \bibinfo {pages} {193 -- 236}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chamon}\ \emph {et~al.}(1996)\citenamefont {Chamon},
  \citenamefont {Mudry},\ and\ \citenamefont {Wen}}]{CMW96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Chamon}, \bibfnamefont
  {Claudio de~C}}, \bibinfo {author} {\bibfnamefont {Christopher}\ \bibnamefont
  {Mudry}}, \ and\ \bibinfo {author} {\bibfnamefont {Xiao-Gang}\ \bibnamefont
  {Wen}}} (\bibinfo {year} {1996}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Instability of the disordered critical points of dirac fermions},}\
  }\href {\doibase 10.1103/PhysRevB.53.R7638} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {53}},\ \bibinfo
  {pages} {R7638--R7641}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Charlier}\ \emph {et~al.}(1991)\citenamefont
  {Charlier}, \citenamefont {Michenaud}, \citenamefont {Gonze},\ and\
  \citenamefont {Vigneron}}]{CMGV91}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Charlier},
  \bibfnamefont {J-C}}, \bibinfo {author} {\bibfnamefont {J.-P.}\ \bibnamefont
  {Michenaud}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Gonze}}, \
  and\ \bibinfo {author} {\bibfnamefont {J.-P.}\ \bibnamefont {Vigneron}}}
  (\bibinfo {year} {1991}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Tight-binding model for the electronic properties of simple hexagonal
  graphite},}\ }\href {\doibase 10.1103/PhysRevB.44.13237} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {44}},\ \bibinfo {pages} {13237--13249}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Charlier}\ \emph {et~al.}(2007)\citenamefont
  {Charlier}, \citenamefont {Blase},\ and\ \citenamefont
  {Roche}}]{nanotube_review}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Charlier},
  \bibfnamefont {Jean-Christophe}}, \bibinfo {author} {\bibfnamefont {Xavier}\
  \bibnamefont {Blase}}, \ and\ \bibinfo {author} {\bibfnamefont {Stephan}\
  \bibnamefont {Roche}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic and transport properties of
  nanotubes},}\ }\href {\doibase 10.1103/RevModPhys.79.677} {\bibfield
  {journal} {\bibinfo  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume}
  {79}},\ \bibinfo {pages} {677--732}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cheianov}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Cheianov}, \citenamefont
  {Fal'ko},\ and\ \citenamefont {Altshuler}}]{CFA07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cheianov},
  \bibfnamefont {Vadim~V}}, \bibinfo {author} {\bibfnamefont {Vladimir}\
  \bibnamefont {Fal'ko}}, \ and\ \bibinfo {author} {\bibfnamefont {B.~L.}\
  \bibnamefont {Altshuler}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield
   {title} {\enquote {\bibinfo {title} {The focusing of electron flow and a
  veselago lens in graphene p-n junctions},}\ }\href {\doibase
  10.1126/science.1138020} {\bibfield  {journal} {\bibinfo  {journal}
  {Science}\ }\textbf {\bibinfo {volume} {315}}~(\bibinfo {number} {5816}),\
  \bibinfo {pages} {1252--1255}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cheianov}\ and\ \citenamefont {Fal'ko}(2006)}]{CF06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cheianov},
  \bibfnamefont {Vadim~V}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Vladimir~I.}\ \bibnamefont {Fal'ko}}} (\bibinfo {year} {2006}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Selective transmission of dirac
  electrons and ballistic magnetoresistance of $n\text{-}p$ junctions in
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.74.041403} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {041403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cheianov}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Cheianov}, \citenamefont {Fal'ko},
  \citenamefont {Altshuler},\ and\ \citenamefont {Aleiner}}]{CFAA07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cheianov},
  \bibfnamefont {Vadim~V}}, \bibinfo {author} {\bibfnamefont {Vladimir~I.}\
  \bibnamefont {Fal'ko}}, \bibinfo {author} {\bibfnamefont {Boris~L.}\
  \bibnamefont {Altshuler}}, \ and\ \bibinfo {author} {\bibfnamefont {Igor~L.}\
  \bibnamefont {Aleiner}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Random resistor network model of minimal
  conductivity in graphene},}\ }\href {\doibase 10.1103/PhysRevLett.99.176801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {99}},\ \bibinfo {pages} {176801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chen}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Chen}, \citenamefont {Apalkov},\
  and\ \citenamefont {Chakraborty}}]{CAC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Chen}, \bibfnamefont
  {Hong-Yi}}, \bibinfo {author} {\bibfnamefont {Vadim}\ \bibnamefont
  {Apalkov}}, \ and\ \bibinfo {author} {\bibfnamefont {Tapash}\ \bibnamefont
  {Chakraborty}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Fock-darwin states of dirac electrons in
  graphene-based artificial atoms},}\ }\href {\doibase
  10.1103/PhysRevLett.98.186803} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo {pages}
  {186803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Chen}}\ \emph {et~al.}(2008)\citenamefont {{Chen}},
  \citenamefont {{Jang}}, \citenamefont {{Adam}}, \citenamefont {{Fuhrer}},
  \citenamefont {{Williams}},\ and\ \citenamefont {{Ishigami}}}]{CJFWI07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Chen}}, \bibfnamefont
  {J-H}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {{Jang}}},
  \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {{Adam}}}, \bibinfo
  {author} {\bibfnamefont {M.~S.}\ \bibnamefont {{Fuhrer}}}, \bibinfo {author}
  {\bibfnamefont {E.~D.}\ \bibnamefont {{Williams}}}, \ and\ \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {{Ishigami}}}} (\bibinfo {year} {2008}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {{Charged-impurity scattering
  in graphene}},}\ }\href {\doibase 10.1038/nphys935} {\bibfield  {journal}
  {\bibinfo  {journal} {Nature Physics}\ }\textbf {\bibinfo {volume} {4}},\
  \bibinfo {pages} {377--381}},\ \Eprint {http://arxiv.org/abs/0708.2408}
  {arXiv:0708.2408 [cond-mat.other]} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Chen}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Chen}, \citenamefont {Lin},
  \citenamefont {Rooks},\ and\ \citenamefont {Avouris}}]{CLRA07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Chen}, \bibfnamefont
  {Zhihong}}, \bibinfo {author} {\bibfnamefont {Yu-Ming}\ \bibnamefont {Lin}},
  \bibinfo {author} {\bibfnamefont {Michael~J.}\ \bibnamefont {Rooks}}, \ and\
  \bibinfo {author} {\bibfnamefont {Phaedon}\ \bibnamefont {Avouris}}}
  (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Graphene nano-ribbon electronics},}\ }\href {\doibase
  10.1016/j.physe.2007.06.020} {\bibfield  {journal} {\bibinfo  {journal}
  {Physica E: Low-dimensional Systems and Nanostructures}\ }\textbf {\bibinfo
  {volume} {40}}~(\bibinfo {number} {2}),\ \bibinfo {pages} {228 --
  232}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cho}\ \emph {et~al.}(2007)\citenamefont {Cho},
  \citenamefont {Chen},\ and\ \citenamefont {Fuhrer}}]{CCF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cho}, \bibfnamefont
  {Sungjae}}, \bibinfo {author} {\bibfnamefont {Yung-Fu}\ \bibnamefont {Chen}},
  \ and\ \bibinfo {author} {\bibfnamefont {Michael~S.}\ \bibnamefont {Fuhrer}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Gate-tunable graphene spin valve},}\ }\href {\doibase 10.1063/1.2784934}
  {\bibfield  {journal} {\bibinfo  {journal} {Applied Physics Letters}\
  }\textbf {\bibinfo {volume} {91}}~(\bibinfo {number} {12}),\ \bibinfo {eid}
  {123105}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Coraux}\ \emph {et~al.}(2008)\citenamefont {Coraux},
  \citenamefont {N`Diaye}, \citenamefont {Busse},\ and\ \citenamefont
  {Michely}}]{CNBM08}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Coraux}, \bibfnamefont
  {Johann}}, \bibinfo {author} {\bibfnamefont {Alpha~T.}\ \bibnamefont
  {N`Diaye}}, \bibinfo {author} {\bibfnamefont {Carsten}\ \bibnamefont
  {Busse}}, \ and\ \bibinfo {author} {\bibfnamefont {Thomas}\ \bibnamefont
  {Michely}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Structural coherency of graphene on ir(111)},}\ }\href {\doibase
  10.1021/nl0728874} {\bibfield  {journal} {\bibinfo  {journal} {Nano Letters}\
  }\textbf {\bibinfo {volume} {8}}~(\bibinfo {number} {2}),\ \bibinfo {pages}
  {565--570}},\ \bibinfo {note} {pMID: 18189442}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cortijo}\ and\ \citenamefont
  {Vozmediano}(2007{\natexlab{a}})}]{CV07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cortijo}, \bibfnamefont
  {A}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont
  {Vozmediano}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic properties of curved graphene
  sheets},}\ }\href {http://stacks.iop.org/0295-5075/77/i=4/a=47002} {\bibfield
   {journal} {\bibinfo  {journal} {EPL (Europhysics Letters)}\ }\textbf
  {\bibinfo {volume} {77}}~(\bibinfo {number} {4}),\ \bibinfo {pages}
  {47002}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cortijo}\ and\ \citenamefont
  {Vozmediano}(2007{\natexlab{b}})}]{CV07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cortijo}, \bibfnamefont
  {Alberto}}, \ and\ \bibinfo {author} {\bibfnamefont {Mar{\`\i}a~A.H.}\
  \bibnamefont {Vozmediano}}} (\bibinfo {year} {2007}{\natexlab{b}}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Effects of topological
  defects and local curvature on the electronic properties of planar
  graphene},}\ }\href {\doibase 10.1016/j.nuclphysb.2006.10.031} {\bibfield
  {journal} {\bibinfo  {journal} {Nuclear Physics B}\ }\textbf {\bibinfo
  {volume} {763}}~(\bibinfo {number} {3}),\ \bibinfo {pages}
  {293--308}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cserti}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Cserti}, \citenamefont
  {Csord\'as},\ and\ \citenamefont {D\'avid}}]{CCD07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cserti}, \bibfnamefont
  {J\'ozsef}}, \bibinfo {author} {\bibfnamefont {Andr\'as}\ \bibnamefont
  {Csord\'as}}, \ and\ \bibinfo {author} {\bibfnamefont {Gyula}\ \bibnamefont
  {D\'avid}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Role of the trigonal warping on the minimal
  conductivity of bilayer graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.99.066802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {066802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cserti}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Cserti}, \citenamefont {P\'alyi},\
  and\ \citenamefont {P\'eterfalvi}}]{CPP07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Cserti}, \bibfnamefont
  {J\'ozsef}}, \bibinfo {author} {\bibfnamefont {Andr\'as}\ \bibnamefont
  {P\'alyi}}, \ and\ \bibinfo {author} {\bibfnamefont {Csaba}\ \bibnamefont
  {P\'eterfalvi}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Caustics due to a negative refractive index in
  circular graphene $p\mathrm{\text{-}}n$ junctions},}\ }\href {\doibase
  10.1103/PhysRevLett.99.246801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {246801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Dahal}}\ \emph {et~al.}(2007)\citenamefont
  {{Dahal}}, \citenamefont {{Wehling}}, \citenamefont {{Bedell}}, \citenamefont
  {{Zhu}},\ and\ \citenamefont {{Balatsky}}}]{DWBZB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Dahal}}, \bibfnamefont
  {H~P}}, \bibinfo {author} {\bibfnamefont {T.~O.}\ \bibnamefont {{Wehling}}},
  \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont {{Bedell}}}, \bibinfo
  {author} {\bibfnamefont {J.-X.}\ \bibnamefont {{Zhu}}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~V.}\ \bibnamefont {{Balatsky}}}} (\bibinfo {year}
  {2007}),\ \href@noop {} {\enquote {\bibinfo {title} {{Wigner crystallization
  in a single and bilayer graphene}},}\ }\Eprint
  {http://arxiv.org/abs/0706.1689} {arXiv:0706.1689 [cond-mat.str-el]}
  \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dahal}\ \emph {et~al.}(2006)\citenamefont {Dahal},
  \citenamefont {Joglekar}, \citenamefont {Bedell},\ and\ \citenamefont
  {Balatsky}}]{DJBB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dahal}, \bibfnamefont
  {Hari~P}}, \bibinfo {author} {\bibfnamefont {Yogesh~N.}\ \bibnamefont
  {Joglekar}}, \bibinfo {author} {\bibfnamefont {Kevin~S.}\ \bibnamefont
  {Bedell}}, \ and\ \bibinfo {author} {\bibfnamefont {Alexander~V.}\
  \bibnamefont {Balatsky}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Absence of wigner crystallization in
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.74.233405} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {233405}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Das~Sarma}\ \emph {et~al.}(2007)\citenamefont
  {Das~Sarma}, \citenamefont {Hwang},\ and\ \citenamefont {Tse}}]{SHT07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Das~Sarma},
  \bibfnamefont {S}}, \bibinfo {author} {\bibfnamefont {E.~H.}\ \bibnamefont
  {Hwang}}, \ and\ \bibinfo {author} {\bibfnamefont {Wang-Kong}\ \bibnamefont
  {Tse}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Many-body interaction effects in doped and undoped graphene: Fermi
  liquid versus non-fermi liquid},}\ }\href {\doibase
  10.1103/PhysRevB.75.121406} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {121406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Deacon}\ \emph {et~al.}(2007)\citenamefont {Deacon},
  \citenamefont {Chuang}, \citenamefont {Nicholas}, \citenamefont {Novoselov},\
  and\ \citenamefont {Geim}}]{DCNNG07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Deacon}, \bibfnamefont
  {R~S}}, \bibinfo {author} {\bibfnamefont {K.-C.}\ \bibnamefont {Chuang}},
  \bibinfo {author} {\bibfnamefont {R.~J.}\ \bibnamefont {Nicholas}}, \bibinfo
  {author} {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Cyclotron resonance
  study of the electron and hole velocity in graphene monolayers},}\ }\href
  {\doibase 10.1103/PhysRevB.76.081406} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {081406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dell'Anna}(2006)}]{DAnna06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dell'Anna},
  \bibfnamefont {Luca}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Disordered d-wave superconductors with
  interactions},}\ }\href {\doibase 10.1016/j.nuclphysb.2006.09.024} {\bibfield
   {journal} {\bibinfo  {journal} {Nuclear Physics B}\ }\textbf {\bibinfo
  {volume} {758}}~(\bibinfo {number} {3}),\ \bibinfo {pages} {255 --
  303}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dharma-wardana}(2007)}]{DW0703}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dharma-wardana},
  \bibfnamefont {M~W~C}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic structure and the minimum conductance
  of a graphene layer on sio 2 from density functional methods},}\ }\href
  {http://stacks.iop.org/0953-8984/19/i=38/a=386228} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of Physics: Condensed Matter}\ }\textbf
  {\bibinfo {volume} {19}}~(\bibinfo {number} {38}),\ \bibinfo {pages}
  {386228}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dienwiebel}\ \emph {et~al.}(2004)\citenamefont
  {Dienwiebel}, \citenamefont {Verhoeven}, \citenamefont {Pradeep},
  \citenamefont {Frenken}, \citenamefont {Heimberg},\ and\ \citenamefont
  {Zandbergen}}]{superlub}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dienwiebel},
  \bibfnamefont {Martin}}, \bibinfo {author} {\bibfnamefont {Gertjan~S.}\
  \bibnamefont {Verhoeven}}, \bibinfo {author} {\bibfnamefont {Namboodiri}\
  \bibnamefont {Pradeep}}, \bibinfo {author} {\bibfnamefont {Joost W.~M.}\
  \bibnamefont {Frenken}}, \bibinfo {author} {\bibfnamefont {Jennifer~A.}\
  \bibnamefont {Heimberg}}, \ and\ \bibinfo {author} {\bibfnamefont {Henny~W.}\
  \bibnamefont {Zandbergen}}} (\bibinfo {year} {2004}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Superlubricity of graphite},}\ }\href {\doibase
  10.1103/PhysRevLett.92.126101} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {92}},\ \bibinfo {pages}
  {126101}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dillon}\ \emph {et~al.}(1977)\citenamefont {Dillon},
  \citenamefont {Spain},\ and\ \citenamefont {McClure}}]{DSM77}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dillon}, \bibfnamefont
  {RO}}, \bibinfo {author} {\bibfnamefont {I.L.}\ \bibnamefont {Spain}}, \ and\
  \bibinfo {author} {\bibfnamefont {J.W.}\ \bibnamefont {McClure}}} (\bibinfo
  {year} {1977}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Electronic
  energy band parameters of graphite and their dependence on pressure,
  temperature and acceptor concentration},}\ }\href {\doibase
  10.1016/0022-3697(77)90231-1} {\bibfield  {journal} {\bibinfo  {journal}
  {Journal of Physics and Chemistry of Solids}\ }\textbf {\bibinfo {volume}
  {38}}~(\bibinfo {number} {6}),\ \bibinfo {pages} {635 -- 645}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {DiVincenzo}\ and\ \citenamefont {Mele}(1984)}]{mele}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {DiVincenzo},
  \bibfnamefont {D~P}}, \ and\ \bibinfo {author} {\bibfnamefont {E.~J.}\
  \bibnamefont {Mele}}} (\bibinfo {year} {1984}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Self-consistent effective-mass theory for intralayer
  screening in graphite intercalation compounds},}\ }\href {\doibase
  10.1103/PhysRevB.29.1685} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {29}},\ \bibinfo {pages}
  {1685--1694}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dong}\ \emph {et~al.}(1998)\citenamefont {Dong},
  \citenamefont {Hou},\ and\ \citenamefont {Ma}}]{DHM98}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dong}, \bibfnamefont
  {Shi-Hai}}, \bibinfo {author} {\bibfnamefont {Xi-Wen}\ \bibnamefont {Hou}}, \
  and\ \bibinfo {author} {\bibfnamefont {Zhong-Qi}\ \bibnamefont {Ma}}}
  (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Relativistic levinson theorem in two dimensions},}\ }\href {\doibase
  10.1103/PhysRevA.58.2160} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. A}\ }\textbf {\bibinfo {volume} {58}},\ \bibinfo {pages}
  {2160--2167}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Doretto}\ and\ \citenamefont {Smith}(2007)}]{DMS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Doretto}, \bibfnamefont
  {R~L}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~Morais}\ \bibnamefont
  {Smith}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum hall ferromagnetism in graphene: Su(4) bosonization
  approach},}\ }\href {\doibase 10.1103/PhysRevB.76.195431} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {195431}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dresselhaus}\ and\ \citenamefont
  {Dresselhaus}(1965)}]{DD65}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dresselhaus},
  \bibfnamefont {G}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~S.}\
  \bibnamefont {Dresselhaus}}} (\bibinfo {year} {1965}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Spin-orbit interaction in graphite},}\ }\href
  {\doibase 10.1103/PhysRev.140.A401} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {140}},\ \bibinfo {pages}
  {A401--A412}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dresselhaus}\ and\ \citenamefont
  {Dresselhaus}(2002)}]{gic}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dresselhaus},
  \bibfnamefont {M~S}}, \ and\ \bibinfo {author} {\bibfnamefont
  {G.}~\bibnamefont {Dresselhaus}}} (\bibinfo {year} {2002}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Intercalation compounds of graphite},}\
  }\href {\doibase 10.1080/00018730110113644} {\bibfield  {journal} {\bibinfo
  {journal} {Advances in Physics}\ }\textbf {\bibinfo {volume} {51}}~(\bibinfo
  {number} {1}),\ \bibinfo {pages} {1--186}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dresselhaus}\ \emph {et~al.}(1983)\citenamefont
  {Dresselhaus}, \citenamefont {Dresselhaus}, \citenamefont {Fischer},\ and\
  \citenamefont {Moran}}]{DDFM83}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dresselhaus},
  \bibfnamefont {MS}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Dresselhaus}}, \bibinfo {author} {\bibfnamefont {J.E.}\ \bibnamefont
  {Fischer}}, \ and\ \bibinfo {author} {\bibfnamefont {M.J.}\ \bibnamefont
  {Moran}}} (\bibinfo {year} {1983}),\ \href@noop {} {\emph {\bibinfo {title}
  {Intercalated graphite}}}\ (\bibinfo  {publisher} {North-Holland, New
  York})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dresselhaus}\ and\ \citenamefont
  {Mavroides}(1964)}]{DM64}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Dresselhaus},
  \bibfnamefont {MS}}, \ and\ \bibinfo {author} {\bibfnamefont {J.G.}\
  \bibnamefont {Mavroides}}} (\bibinfo {year} {1964}),\ \href@noop {} {\bibinfo
   {journal} {IBM J. Res. Dev}\ ,\ \bibinfo {pages} {262}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Dugaev}\ \emph {et~al.}(2006)\citenamefont {Dugaev},
  \citenamefont {Litvinov},\ and\ \citenamefont {Barnas}}]{DLB06}%
  \BibitemOpen
\bibfield  {journal} {  }\bibfield  {author} {\bibinfo {author} {\bibnamefont
  {Dugaev}, \bibfnamefont {V~K}}, \bibinfo {author} {\bibfnamefont {V.~I.}\
  \bibnamefont {Litvinov}}, \ and\ \bibinfo {author} {\bibfnamefont
  {J.}~\bibnamefont {Barnas}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Exchange interaction of magnetic impurities in
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.74.224438} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {224438}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Duke}(1968)}]{Duke68}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Duke}, \bibfnamefont
  {C~B}}} (\bibinfo {year} {1968}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum theory of transport in narrow channels},}\ }\href {\doibase
  10.1103/PhysRev.168.816} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {168}},\ \bibinfo {pages}
  {816--831}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Eisenstein}\ \emph {et~al.}(1994)\citenamefont
  {Eisenstein}, \citenamefont {Pfeiffer},\ and\ \citenamefont {West}}]{EPW94}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Eisenstein},
  \bibfnamefont {J~P}}, \bibinfo {author} {\bibfnamefont {L.~N.}\ \bibnamefont
  {Pfeiffer}}, \ and\ \bibinfo {author} {\bibfnamefont {K.~W.}\ \bibnamefont
  {West}}} (\bibinfo {year} {1994}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Compressibility of the two-dimensional electron gas: Measurements of
  the zero-field exchange energy and fractional quantum hall gap},}\ }\href
  {\doibase 10.1103/PhysRevB.50.1760} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {50}},\ \bibinfo
  {pages} {1760--1778}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Eizenberg}\ and\ \citenamefont
  {Blakely}(1979)}]{EB79}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Eizenberg},
  \bibfnamefont {M}}, \ and\ \bibinfo {author} {\bibfnamefont {J.M.}\
  \bibnamefont {Blakely}}} (\bibinfo {year} {1979}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Carbon monolayer phase condensation on
  ni(111)},}\ }\href {\doibase 10.1016/0039-6028(79)90330-3} {\bibfield
  {journal} {\bibinfo  {journal} {Surface Science}\ }\textbf {\bibinfo {volume}
  {82}}~(\bibinfo {number} {1}),\ \bibinfo {pages} {228 -- 236}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Esquinazi}\ \emph {et~al.}(2002)\citenamefont
  {Esquinazi}, \citenamefont {Setzer}, \citenamefont {H\"ohne}, \citenamefont
  {Semmelhack}, \citenamefont {Kopelevich}, \citenamefont {Spemann},
  \citenamefont {Butz}, \citenamefont {Kohlstrunk},\ and\ \citenamefont
  {L\"osche}}]{Eetal02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Esquinazi},
  \bibfnamefont {P}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Setzer}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {H\"ohne}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Semmelhack}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Kopelevich}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Spemann}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Butz}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Kohlstrunk}}, \ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {L\"osche}}} (\bibinfo {year} {2002}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Ferromagnetism in oriented graphite samples},}\ }\href
  {\doibase 10.1103/PhysRevB.66.024429} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {66}},\ \bibinfo
  {pages} {024429}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Esquinazi}\ \emph {et~al.}(2003)\citenamefont
  {Esquinazi}, \citenamefont {Spemann}, \citenamefont {H\"ohne}, \citenamefont
  {Setzer}, \citenamefont {Han},\ and\ \citenamefont {Butz}}]{Eetal03b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Esquinazi},
  \bibfnamefont {P}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Spemann}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {H\"ohne}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Setzer}}, \bibinfo
  {author} {\bibfnamefont {K.-H.}\ \bibnamefont {Han}}, \ and\ \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Butz}}} (\bibinfo {year} {2003}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Induced magnetic ordering by
  proton irradiation in graphite},}\ }\href {\doibase
  10.1103/PhysRevLett.91.227201} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {91}},\ \bibinfo {pages}
  {227201}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Faugeras}\ \emph {et~al.}(2008)\citenamefont
  {Faugeras}, \citenamefont {Nerriere}, \citenamefont {Potemski}, \citenamefont
  {Mahmood}, \citenamefont {Dujardin}, \citenamefont {Berger},\ and\
  \citenamefont {de~Heer}}]{FNPMDBH07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Faugeras},
  \bibfnamefont {C}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Nerriere}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Potemski}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Mahmood}}, \bibinfo
  {author} {\bibfnamefont {E.}~\bibnamefont {Dujardin}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Berger}}, \ and\ \bibinfo {author}
  {\bibfnamefont {W.~A.}\ \bibnamefont {de~Heer}}} (\bibinfo {year} {2008}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Few-layer graphene on sic,
  pyrolitic graphite, and graphene: A raman scattering study},}\ }\href
  {\doibase 10.1063/1.2828975} {\bibfield  {journal} {\bibinfo  {journal}
  {Applied Physics Letters}\ }\textbf {\bibinfo {volume} {92}}~(\bibinfo
  {number} {1}),\ \bibinfo {eid} {011914}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ferrari}\ \emph {et~al.}(2006)\citenamefont
  {Ferrari}, \citenamefont {Meyer}, \citenamefont {Scardaci}, \citenamefont
  {Casiraghi}, \citenamefont {Lazzeri}, \citenamefont {Mauri}, \citenamefont
  {Piscanec}, \citenamefont {Jiang}, \citenamefont {Novoselov}, \citenamefont
  {Roth},\ and\ \citenamefont {Geim}}]{FMSCLMPJNG06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ferrari}, \bibfnamefont
  {A~C}}, \bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Meyer}},
  \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Scardaci}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Casiraghi}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Lazzeri}}, \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Mauri}}, \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Piscanec}}, \bibinfo {author} {\bibfnamefont
  {D.}~\bibnamefont {Jiang}}, \bibinfo {author} {\bibfnamefont {K.~S.}\
  \bibnamefont {Novoselov}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Roth}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont
  {Geim}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Raman spectrum of graphene and graphene layers},}\ }\href {\doibase
  10.1103/PhysRevLett.97.187401} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {187401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fertig}\ and\ \citenamefont {Brey}(2006)}]{FB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fertig}, \bibfnamefont
  {H~A}}, \ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Brey}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Luttinger liquid at the edge of undoped graphene in a strong magnetic
  field},}\ }\href {\doibase 10.1103/PhysRevLett.97.116805} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {97}},\ \bibinfo {pages} {116805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fogler}\ \emph {et~al.}(2008)\citenamefont {Fogler},
  \citenamefont {Novikov}, \citenamefont {Glazman},\ and\ \citenamefont
  {Shklovskii}}]{FGNS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fogler}, \bibfnamefont
  {M~M}}, \bibinfo {author} {\bibfnamefont {D.~S.}\ \bibnamefont {Novikov}},
  \bibinfo {author} {\bibfnamefont {L.~I.}\ \bibnamefont {Glazman}}, \ and\
  \bibinfo {author} {\bibfnamefont {B.~I.}\ \bibnamefont {Shklovskii}}}
  (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Effect of disorder on a graphene $p\text{-}n$ junction},}\ }\href {\doibase
  10.1103/PhysRevB.77.075420} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo {pages}
  {075420}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fogler}\ \emph {et~al.}(2007)\citenamefont {Fogler},
  \citenamefont {Novikov},\ and\ \citenamefont {Shklovskii}}]{FNS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fogler}, \bibfnamefont
  {M~M}}, \bibinfo {author} {\bibfnamefont {D.~S.}\ \bibnamefont {Novikov}}, \
  and\ \bibinfo {author} {\bibfnamefont {B.~I.}\ \bibnamefont {Shklovskii}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Screening of a hypercritical charge in graphene},}\ }\href {\doibase
  10.1103/PhysRevB.76.233402} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {233402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Forbeaux}\ \emph {et~al.}(1998)\citenamefont
  {Forbeaux}, \citenamefont {Themlin},\ and\ \citenamefont {Debever}}]{FTD98}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Forbeaux},
  \bibfnamefont {I}}, \bibinfo {author} {\bibfnamefont {J.-M.}\ \bibnamefont
  {Themlin}}, \ and\ \bibinfo {author} {\bibfnamefont {J.-M.}\ \bibnamefont
  {Debever}}} (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Heteroepitaxial graphite on $6h-\mathrm{SiC}(0001):$\quad{}interface
  formation through conduction-band electronic structure},}\ }\href {\doibase
  10.1103/PhysRevB.58.16396} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {58}},\ \bibinfo {pages}
  {16396--16406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Foster}\ and\ \citenamefont
  {Ludwig}(2006{\natexlab{a}})}]{FA05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Foster}, \bibfnamefont
  {Matthew~S}}, \ and\ \bibinfo {author} {\bibfnamefont {Andreas W.~W.}\
  \bibnamefont {Ludwig}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Interaction effects on two-dimensional
  fermions with random hopping},}\ }\href {\doibase 10.1103/PhysRevB.73.155104}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {73}},\ \bibinfo {pages} {155104}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Foster}\ and\ \citenamefont
  {Ludwig}(2006{\natexlab{b}})}]{FA06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Foster}, \bibfnamefont
  {Matthew~S}}, \ and\ \bibinfo {author} {\bibfnamefont {Andreas W.~W.}\
  \bibnamefont {Ludwig}}} (\bibinfo {year} {2006}{\natexlab{b}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Metal-insulator transition in
  hubbard-like models with random hopping},}\ }\href {\doibase
  10.1103/PhysRevB.74.241102} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo {pages}
  {241102}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fradkin}(1986{\natexlab{a}})}]{F86}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fradkin}, \bibfnamefont
  {Eduardo}}} (\bibinfo {year} {1986}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Critical behavior of disordered degenerate
  semiconductors. i. models, symmetries, and formalism},}\ }\href {\doibase
  10.1103/PhysRevB.33.3257} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {33}},\ \bibinfo {pages}
  {3257--3262}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fradkin}(1986{\natexlab{b}})}]{F86b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fradkin}, \bibfnamefont
  {Eduardo}}} (\bibinfo {year} {1986}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Critical behavior of disordered degenerate
  semiconductors. ii. spectrum and transport properties in mean-field
  theory},}\ }\href {\doibase 10.1103/PhysRevB.33.3263} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {33}},\
  \bibinfo {pages} {3263--3268}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fritz}\ \emph {et~al.}(2006)\citenamefont {Fritz},
  \citenamefont {Florens},\ and\ \citenamefont {Vojta}}]{FFV06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fritz}, \bibfnamefont
  {Lars}}, \bibinfo {author} {\bibfnamefont {Serge}\ \bibnamefont {Florens}}, \
  and\ \bibinfo {author} {\bibfnamefont {Matthias}\ \bibnamefont {Vojta}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Universal crossovers and critical dynamics of quantum phase transitions: A
  renormalization group study of the pseudogap kondo problem},}\ }\href
  {\doibase 10.1103/PhysRevB.74.144410} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo
  {pages} {144410}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fuchs}\ and\ \citenamefont {Lederer}(2007)}]{FL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fuchs}, \bibfnamefont
  {Jean-No\"el}}, \ and\ \bibinfo {author} {\bibfnamefont {Pascal}\
  \bibnamefont {Lederer}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Spontaneous parity breaking of graphene in the
  quantum hall regime},}\ }\href {\doibase 10.1103/PhysRevLett.98.016803}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {98}},\ \bibinfo {pages} {016803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fujita}\ \emph {et~al.}(1996)\citenamefont {Fujita},
  \citenamefont {Wakabayashi}, \citenamefont {Nakada},\ and\ \citenamefont
  {Kusakabe}}]{FWNK96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fujita}, \bibfnamefont
  {Mitsutaka}}, \bibinfo {author} {\bibfnamefont {Katsunori}\ \bibnamefont
  {Wakabayashi}}, \bibinfo {author} {\bibfnamefont {Kyoko}\ \bibnamefont
  {Nakada}}, \ and\ \bibinfo {author} {\bibfnamefont {Koichi}\ \bibnamefont
  {Kusakabe}}} (\bibinfo {year} {1996}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Peculiar localized state at zigzag graphite edge},}\
  }\href {\doibase 10.1143/JPSJ.65.1920} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of the Physical Society of Japan}\ }\textbf {\bibinfo
  {volume} {65}}~(\bibinfo {number} {7}),\ \bibinfo {pages}
  {1920--1923}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fukuyama}(1971)}]{FK1971}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Fukuyama},
  \bibfnamefont {Hidetoshi}}} (\bibinfo {year} {1971}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Theory of orbital magnetism of bloch electrons:
  Coulomb interactions},}\ }\href {\doibase 10.1143/PTP.45.704} {\bibfield
  {journal} {\bibinfo  {journal} {Progress of Theoretical Physics}\ }\textbf
  {\bibinfo {volume} {45}}~(\bibinfo {number} {3}),\ \bibinfo {pages}
  {704--729}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gasparoux}(1967)}]{G67}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gasparoux},
  \bibfnamefont {H}}} (\bibinfo {year} {1967}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Modification des propriÌ©tÌ©s magnÌ©tiques du graphite par
  crÌ©ation de sequences rhomboÌ©driques},}\ }\href {\doibase
  10.1016/0008-6223(67)90021-8} {\bibfield  {journal} {\bibinfo  {journal}
  {Carbon}\ }\textbf {\bibinfo {volume} {5}}~(\bibinfo {number} {5}),\ \bibinfo
  {pages} {441 -- 451}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Geim}\ and\ \citenamefont
  {Novoselov}(2007)}]{geim_review}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Geim}, \bibfnamefont
  {A~K}}, \ and\ \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont
  {Novoselov}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {The rise of graphene},}\ }\href@noop {} {\bibfield
  {journal} {\bibinfo  {journal} {Nature Materials}\ }\textbf {\bibinfo
  {volume} {6}},\ \bibinfo {pages} {183}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Geim}\ and\ \citenamefont
  {MacDonald}(2007)}]{GMac07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Geim}, \bibfnamefont
  {Andrey~K}}, \ and\ \bibinfo {author} {\bibfnamefont {Allan~H.}\ \bibnamefont
  {MacDonald}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Graphene: Exploring carbon flatland},}\ }\href {\doibase
  10.1063/1.2774096} {\bibfield  {journal} {\bibinfo  {journal} {Physics
  Today}\ }\textbf {\bibinfo {volume} {60}}~(\bibinfo {number} {8}),\ \bibinfo
  {pages} {35--41}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ghosal}\ \emph {et~al.}(2007)\citenamefont {Ghosal},
  \citenamefont {Goswami},\ and\ \citenamefont {Chakravarty}}]{G64}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ghosal}, \bibfnamefont
  {Amit}}, \bibinfo {author} {\bibfnamefont {Pallab}\ \bibnamefont {Goswami}},
  \ and\ \bibinfo {author} {\bibfnamefont {Sudip}\ \bibnamefont {Chakravarty}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Diamagnetism of nodal fermions},}\ }\href {\doibase
  10.1103/PhysRevB.75.115123} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {115123}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Giesbers}\ \emph {et~al.}(2007)\citenamefont
  {Giesbers}, \citenamefont {Zeitler}, \citenamefont {Katsnelson},
  \citenamefont {Ponomarenko}, \citenamefont {Mohiuddin},\ and\ \citenamefont
  {Maan}}]{GGC2007}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Giesbers},
  \bibfnamefont {A~J~M}}, \bibinfo {author} {\bibfnamefont {U.}~\bibnamefont
  {Zeitler}}, \bibinfo {author} {\bibfnamefont {M.~I.}\ \bibnamefont
  {Katsnelson}}, \bibinfo {author} {\bibfnamefont {L.~A.}\ \bibnamefont
  {Ponomarenko}}, \bibinfo {author} {\bibfnamefont {T.~M.}\ \bibnamefont
  {Mohiuddin}}, \ and\ \bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont
  {Maan}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum-hall activation gaps in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.99.206803} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {206803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Giovani}\ and\ \citenamefont
  {Vignale}(2005)}]{giovani}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Giovani}, \bibfnamefont
  {GF}}, \ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Vignale}}}
  (\bibinfo {year} {2005}),\ \href@noop {} {\emph {\bibinfo {title} {Quantum
  theory of the electron liquid}}}\ (\bibinfo  {publisher} {Cambridge
  Press})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Giovannetti}\ \emph {et~al.}(2007)\citenamefont
  {Giovannetti}, \citenamefont {Khomyakov}, \citenamefont {Brocks},
  \citenamefont {Kelly},\ and\ \citenamefont {van~den Brink}}]{GKBKB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Giovannetti},
  \bibfnamefont {Gianluca}}, \bibinfo {author} {\bibfnamefont {Petr~A.}\
  \bibnamefont {Khomyakov}}, \bibinfo {author} {\bibfnamefont {Geert}\
  \bibnamefont {Brocks}}, \bibinfo {author} {\bibfnamefont {Paul~J.}\
  \bibnamefont {Kelly}}, \ and\ \bibinfo {author} {\bibfnamefont {Jeroen}\
  \bibnamefont {van~den Brink}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Substrate-induced band gap in graphene on
  hexagonal boron nitride: \textit{Ab initio} density functional
  calculations},}\ }\href {\doibase 10.1103/PhysRevB.76.073103} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {073103}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Goerbig}\ \emph {et~al.}(2007)\citenamefont
  {Goerbig}, \citenamefont {Fuchs}, \citenamefont {Kechedzhi},\ and\
  \citenamefont {Fal'ko}}]{GFKF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Goerbig}, \bibfnamefont
  {M~O}}, \bibinfo {author} {\bibfnamefont {J.-N.}\ \bibnamefont {Fuchs}},
  \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Kechedzhi}}, \ and\
  \bibinfo {author} {\bibfnamefont {Vladimir~I.}\ \bibnamefont {Fal'ko}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Filling-factor-dependent magnetophonon resonance in graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.99.087402} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {087402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gonz\'alez}\ \emph {et~al.}(1996)\citenamefont
  {Gonz\'alez}, \citenamefont {Guinea},\ and\ \citenamefont
  {Vozmediano}}]{GGV96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gonz\'alez},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont
  {Vozmediano}}} (\bibinfo {year} {1996}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Unconventional quasiparticle lifetime in graphite},}\
  }\href {\doibase 10.1103/PhysRevLett.77.3589} {\bibfield  {journal} {\bibinfo
   {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo
  {pages} {3589--3592}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gonz\'alez}\ \emph {et~al.}(1999)\citenamefont
  {Gonz\'alez}, \citenamefont {Guinea},\ and\ \citenamefont
  {Vozmediano}}]{GGV99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gonz\'alez},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont
  {Vozmediano}}} (\bibinfo {year} {1999}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Marginal-fermi-liquid behavior from two-dimensional
  coulomb interaction},}\ }\href {\doibase 10.1103/PhysRevB.59.R2474}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {59}},\ \bibinfo {pages} {R2474--R2477}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gonz\'alez}\ \emph {et~al.}(2001)\citenamefont
  {Gonz\'alez}, \citenamefont {Guinea},\ and\ \citenamefont
  {Vozmediano}}]{GGV01}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gonz\'alez},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont
  {Vozmediano}}} (\bibinfo {year} {2001}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electron-electron interactions in graphene sheets},}\
  }\href {\doibase 10.1103/PhysRevB.63.134421} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {63}},\ \bibinfo
  {pages} {134421}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gonz\'alez}\ \emph {et~al.}(1992)\citenamefont
  {Gonz\'alez}, \citenamefont {Guinea},\ and\ \citenamefont
  {Vozmediano}}]{GMD06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gonz\'alez},
  \bibfnamefont {Jos\'e}}, \bibinfo {author} {\bibfnamefont {Francisco}\
  \bibnamefont {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont
  {M.~Angeles~H.}\ \bibnamefont {Vozmediano}}} (\bibinfo {year} {1992}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Continuum approximation to
  fullerene molecules},}\ }\href {\doibase 10.1103/PhysRevLett.69.172}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {69}},\ \bibinfo {pages} {172--175}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gorbachev}\ \emph {et~al.}(2007)\citenamefont
  {Gorbachev}, \citenamefont {Tikhonenko}, \citenamefont {Mayorov},
  \citenamefont {Horsell},\ and\ \citenamefont {Savchenko}}]{GTMHS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gorbachev},
  \bibfnamefont {R~V}}, \bibinfo {author} {\bibfnamefont {F.~V.}\ \bibnamefont
  {Tikhonenko}}, \bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont
  {Mayorov}}, \bibinfo {author} {\bibfnamefont {D.~W.}\ \bibnamefont
  {Horsell}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont
  {Savchenko}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Weak localization in bilayer graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.98.176805} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo {pages}
  {176805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gorbar}\ \emph {et~al.}(2002)\citenamefont {Gorbar},
  \citenamefont {Gusynin}, \citenamefont {Miransky},\ and\ \citenamefont
  {Shovkovy}}]{Getal02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gorbar}, \bibfnamefont
  {E~V}}, \bibinfo {author} {\bibfnamefont {V.~P.}\ \bibnamefont {Gusynin}},
  \bibinfo {author} {\bibfnamefont {V.~A.}\ \bibnamefont {Miransky}}, \ and\
  \bibinfo {author} {\bibfnamefont {I.~A.}\ \bibnamefont {Shovkovy}}} (\bibinfo
  {year} {2002}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Magnetic
  field driven metal-insulator phase transition in planar systems},}\ }\href
  {\doibase 10.1103/PhysRevB.66.045108} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {66}},\ \bibinfo
  {pages} {045108}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Goswami}\ \emph {et~al.}(2007)\citenamefont
  {Goswami}, \citenamefont {Jia},\ and\ \citenamefont {Chakravarty}}]{GJC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Goswami}, \bibfnamefont
  {Pallab}}, \bibinfo {author} {\bibfnamefont {Xun}\ \bibnamefont {Jia}}, \
  and\ \bibinfo {author} {\bibfnamefont {Sudip}\ \bibnamefont {Chakravarty}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Quantum hall plateau transition in the lowest landau level of disordered
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.76.205408} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {205408}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Graf}\ \emph {et~al.}(2007)\citenamefont {Graf},
  \citenamefont {Molitor}, \citenamefont {Ensslin}, \citenamefont {Stampfer},
  \citenamefont {Jungen}, \citenamefont {Hierold},\ and\ \citenamefont
  {Wirtz}}]{GMESJHW07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Graf}, \bibfnamefont
  {D}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Molitor}}, \bibinfo
  {author} {\bibfnamefont {K.}~\bibnamefont {Ensslin}}, \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Stampfer}}, \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Jungen}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Hierold}}, \ and\ \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Wirtz}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Spatially resolved raman spectroscopy of single-
  and few-layer graphene},}\ }\href {\doibase 10.1021/nl061702a} {\bibfield
  {journal} {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo {volume}
  {7}}~(\bibinfo {number} {2}),\ \bibinfo {pages} {238--242}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Guinea}(2007)}]{G06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Guinea}, \bibfnamefont
  {F}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Charge distribution and screening in layered graphene systems},}\
  }\href {\doibase 10.1103/PhysRevB.75.235433} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo
  {pages} {235433}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Guinea}\ \emph {et~al.}(2006)\citenamefont {Guinea},
  \citenamefont {Castro~Neto},\ and\ \citenamefont {Peres}}]{GNP06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Guinea}, \bibfnamefont
  {F}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont {Castro~Neto}},
  \ and\ \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic states and landau levels in graphene stacks},}\ }\href {\doibase
  10.1103/PhysRevB.73.245426} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo {pages}
  {245426}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Guinea}\ \emph {et~al.}(2008)\citenamefont {Guinea},
  \citenamefont {Katsnelson},\ and\ \citenamefont {Vozmediano}}]{GKV07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Guinea}, \bibfnamefont
  {F}}, \bibinfo {author} {\bibfnamefont {M.~I.}\ \bibnamefont {Katsnelson}}, \
  and\ \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont {Vozmediano}}}
  (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Midgap states and charge inhomogeneities in corrugated graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.77.075422} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo
  {pages} {075422}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gumbs}\ and\ \citenamefont {Fekete}(1997)}]{Gumbs97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gumbs}, \bibfnamefont
  {Godfrey}}, \ and\ \bibinfo {author} {\bibfnamefont {Paula}\ \bibnamefont
  {Fekete}}} (\bibinfo {year} {1997}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Hofstadter butterfly for the hexagonal lattice},}\ }\href {\doibase
  10.1103/PhysRevB.56.3787} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {56}},\ \bibinfo {pages}
  {3787--3791}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gupta}\ \emph {et~al.}(2006)\citenamefont {Gupta},
  \citenamefont {Chen}, \citenamefont {Joshi}, \citenamefont {Tadigadapa},\
  and\ \citenamefont {Eklund}}]{GCJTE06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gupta}, \bibfnamefont
  {A}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Chen}}, \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Joshi}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Tadigadapa}}, \ and\ \bibinfo {author}
  {\bibnamefont {Eklund}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Raman scattering from high-frequency phonons in
  supported n-graphene layer films},}\ }\href {\doibase 10.1021/nl061420a}
  {\bibfield  {journal} {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo
  {volume} {6}}~(\bibinfo {number} {12}),\ \bibinfo {pages} {2667--2673}},\
  \bibinfo {note} {pMID: 17163685}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gusynin}\ \emph {et~al.}(2006)\citenamefont
  {Gusynin}, \citenamefont {Miransky}, \citenamefont {Sharapov},\ and\
  \citenamefont {Shovkovy}}]{GMSS06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gusynin}, \bibfnamefont
  {V~P}}, \bibinfo {author} {\bibfnamefont {V.~A.}\ \bibnamefont {Miransky}},
  \bibinfo {author} {\bibfnamefont {S.~G.}\ \bibnamefont {Sharapov}}, \ and\
  \bibinfo {author} {\bibfnamefont {I.~A.}\ \bibnamefont {Shovkovy}}} (\bibinfo
  {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Excitonic
  gap, phase transition, and quantum hall effect in graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.74.195429} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo
  {pages} {195429}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gusynin}\ and\ \citenamefont
  {Sharapov}(2005)}]{GS05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gusynin}, \bibfnamefont
  {V~P}}, \ and\ \bibinfo {author} {\bibfnamefont {S.~G.}\ \bibnamefont
  {Sharapov}}} (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Unconventional integer quantum hall effect in graphene},}\
  }\href {\doibase 10.1103/PhysRevLett.95.146801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {95}},\
  \bibinfo {pages} {146801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Gusynin}\ \emph {et~al.}(2007)\citenamefont
  {Gusynin}, \citenamefont {Sharapov},\ and\ \citenamefont {Carbotte}}]{GSC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Gusynin}, \bibfnamefont
  {V~P}}, \bibinfo {author} {\bibfnamefont {S~G}\ \bibnamefont {Sharapov}}, \
  and\ \bibinfo {author} {\bibfnamefont {J~P}\ \bibnamefont {Carbotte}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Magneto-optical conductivity in graphene},}\ }\href
  {http://stacks.iop.org/0953-8984/19/i=2/a=026222} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of Physics: Condensed Matter}\ }\textbf
  {\bibinfo {volume} {19}}~(\bibinfo {number} {2}),\ \bibinfo {pages}
  {026222}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Haldane}(1988)}]{H88}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Haldane}, \bibfnamefont
  {F~D~M}}} (\bibinfo {year} {1988}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Model for a quantum hall effect without landau levels:
  Condensed-matter realization of the "parity anomaly"},}\ }\href {\doibase
  10.1103/PhysRevLett.61.2015} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {61}},\ \bibinfo {pages}
  {2015--2018}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Han}\ \emph {et~al.}(2007)\citenamefont {Han},
  \citenamefont {\"Ozyilmaz}, \citenamefont {Zhang},\ and\ \citenamefont
  {Kim}}]{HOZK07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Han}, \bibfnamefont
  {Melinda~Y}}, \bibinfo {author} {\bibfnamefont {Barbaros}\ \bibnamefont
  {\"Ozyilmaz}}, \bibinfo {author} {\bibfnamefont {Yuanbo}\ \bibnamefont
  {Zhang}}, \ and\ \bibinfo {author} {\bibfnamefont {Philip}\ \bibnamefont
  {Kim}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Energy band-gap engineering of graphene nanoribbons},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.206805} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {206805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Harper}(1955)}]{harper}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Harper}, \bibfnamefont
  {P~G}}} (\bibinfo {year} {1955}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Single band motion of conduction electrons in a uniform magnetic
  field},}\ }\href {http://stacks.iop.org/0370-1298/68/i=10/a=304} {\bibfield
  {journal} {\bibinfo  {journal} {Proceedings of the Physical Society. Section
  A}\ }\textbf {\bibinfo {volume} {68}}~(\bibinfo {number} {10}),\ \bibinfo
  {pages} {874}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Harrison}(1980)}]{harrison}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Harrison},
  \bibfnamefont {WA}}} (\bibinfo {year} {1980}),\ \href@noop {} {\emph
  {\bibinfo {title} {Solid State Theory}}}\ (\bibinfo  {publisher}
  {Dover})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hass}\ \emph {et~al.}(2007)\citenamefont {Hass},
  \citenamefont {Feng}, \citenamefont {Mill\'an-Otoya}, \citenamefont {Li},
  \citenamefont {Sprinkle}, \citenamefont {First}, \citenamefont {de~Heer},
  \citenamefont {Conrad},\ and\ \citenamefont {Berger}}]{Hetal07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hass}, \bibfnamefont
  {J}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Feng}}, \bibinfo
  {author} {\bibfnamefont {J.~E.}\ \bibnamefont {Mill\'an-Otoya}}, \bibinfo
  {author} {\bibfnamefont {X.}~\bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {M.}~\bibnamefont {Sprinkle}}, \bibinfo {author}
  {\bibfnamefont {P.~N.}\ \bibnamefont {First}}, \bibinfo {author}
  {\bibfnamefont {W.~A.}\ \bibnamefont {de~Heer}}, \bibinfo {author}
  {\bibfnamefont {E.~H.}\ \bibnamefont {Conrad}}, \ and\ \bibinfo {author}
  {\bibfnamefont {C.}~\bibnamefont {Berger}}} (\bibinfo {year} {2007}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Structural properties of the
  multilayer graphene/$4h\text{-}\mathrm{Si}\mathrm{C}(000\overline{1})$ system
  as determined by surface x-ray diffraction},}\ }\href {\doibase
  10.1103/PhysRevB.75.214109} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {214109}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hass}\ \emph {et~al.}(2008)\citenamefont {Hass},
  \citenamefont {Varchon}, \citenamefont {Mill\'an-Otoya}, \citenamefont
  {Sprinkle}, \citenamefont {Sharma}, \citenamefont {de~Heer}, \citenamefont
  {Berger}, \citenamefont {First}, \citenamefont {Magaud},\ and\ \citenamefont
  {Conrad}}]{HVMSHBFMC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hass}, \bibfnamefont
  {J}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Varchon}}, \bibinfo
  {author} {\bibfnamefont {J.~E.}\ \bibnamefont {Mill\'an-Otoya}}, \bibinfo
  {author} {\bibfnamefont {M.}~\bibnamefont {Sprinkle}}, \bibinfo {author}
  {\bibfnamefont {N.}~\bibnamefont {Sharma}}, \bibinfo {author} {\bibfnamefont
  {W.~A.}\ \bibnamefont {de~Heer}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Berger}}, \bibinfo {author} {\bibfnamefont {P.~N.}\
  \bibnamefont {First}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {Magaud}}, \ and\ \bibinfo {author} {\bibfnamefont {E.~H.}\ \bibnamefont
  {Conrad}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Why multilayer graphene on
  $4h\mathrm{\text{-}}\mathrm{SiC}(000\overline{1})$ behaves like a single
  sheet of graphene},}\ }\href {\doibase 10.1103/PhysRevLett.100.125504}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {100}},\ \bibinfo {pages} {125504}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {de~Heer}\ \emph {et~al.}(2007)\citenamefont
  {de~Heer}, \citenamefont {Berger}, \citenamefont {Wu}, \citenamefont {First},
  \citenamefont {Conrad}, \citenamefont {Li}, \citenamefont {Li}, \citenamefont
  {Sprinkle}, \citenamefont {Hass}, \citenamefont {Sadowski}, \citenamefont
  {Potemski},\ and\ \citenamefont {Martinez}}]{Hetal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {de~Heer}, \bibfnamefont
  {Walt~A}}, \bibinfo {author} {\bibfnamefont {Claire}\ \bibnamefont {Berger}},
  \bibinfo {author} {\bibfnamefont {Xiaosong}\ \bibnamefont {Wu}}, \bibinfo
  {author} {\bibfnamefont {Phillip~N.}\ \bibnamefont {First}}, \bibinfo
  {author} {\bibfnamefont {Edward~H.}\ \bibnamefont {Conrad}}, \bibinfo
  {author} {\bibfnamefont {Xuebin}\ \bibnamefont {Li}}, \bibinfo {author}
  {\bibfnamefont {Tianbo}\ \bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont
  {Michael}\ \bibnamefont {Sprinkle}}, \bibinfo {author} {\bibfnamefont
  {Joanna}\ \bibnamefont {Hass}}, \bibinfo {author} {\bibfnamefont {Marcin~L.}\
  \bibnamefont {Sadowski}}, \bibinfo {author} {\bibfnamefont {Marek}\
  \bibnamefont {Potemski}}, \ and\ \bibinfo {author} {\bibfnamefont {GÌ©rard}\
  \bibnamefont {Martinez}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Epitaxial graphene},}\ }\href {\doibase
  10.1016/j.ssc.2007.04.023} {\bibfield  {journal} {\bibinfo  {journal} {Solid
  State Communications}\ }\textbf {\bibinfo {volume} {143}}~(\bibinfo {number}
  {1--2}),\ \bibinfo {pages} {92--100}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hentschel}\ and\ \citenamefont
  {Guinea}(2007)}]{HG07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hentschel},
  \bibfnamefont {Martina}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Francisco}\ \bibnamefont {Guinea}}} (\bibinfo {year} {2007}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Orthogonality catastrophe and kondo
  effect in graphene},}\ }\href {\doibase 10.1103/PhysRevB.76.115407}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {76}},\ \bibinfo {pages} {115407}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Herbut}(2006)}]{IH06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Herbut}, \bibfnamefont
  {Igor~F}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Interactions and phase transitions on graphene's honeycomb
  lattice},}\ }\href {\doibase 10.1103/PhysRevLett.97.146401} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {97}},\ \bibinfo {pages} {146401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Herbut}(2007)}]{H06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Herbut}, \bibfnamefont
  {Igor~F}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Theory of integer quantum hall effect in graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.75.165411} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo
  {pages} {165411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Heremans}\ \emph {et~al.}(1994)\citenamefont
  {Heremans}, \citenamefont {Olk},\ and\ \citenamefont {Morelli}}]{HOM1994}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Heremans},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {C.~H.}\ \bibnamefont
  {Olk}}, \ and\ \bibinfo {author} {\bibfnamefont {D.~T.}\ \bibnamefont
  {Morelli}}} (\bibinfo {year} {1994}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Magnetic susceptibility of carbon structures},}\ }\href {\doibase
  10.1103/PhysRevB.49.15122} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {49}},\ \bibinfo {pages}
  {15122--15125}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Himpsel}\ \emph {et~al.}(1982)\citenamefont
  {Himpsel}, \citenamefont {Christmann}, \citenamefont {Heimann}, \citenamefont
  {Eastman},\ and\ \citenamefont {Feibelman}}]{HCHEF82}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Himpsel}, \bibfnamefont
  {FJ}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Christmann}},
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Heimann}}, \bibinfo
  {author} {\bibfnamefont {D.E.}\ \bibnamefont {Eastman}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Peter~J.}\ \bibnamefont {Feibelman}}} (\bibinfo
  {year} {1982}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Adsorbate
  band dispersions for c on ru(0001)},}\ }\href {\doibase
  10.1016/0039-6028(82)90379-X} {\bibfield  {journal} {\bibinfo  {journal}
  {Surface Science}\ }\textbf {\bibinfo {volume} {115}}~(\bibinfo {number}
  {3}),\ \bibinfo {pages} {L159 -- L164}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hobson}\ and\ \citenamefont
  {Nierenberg}(1953)}]{HN53}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hobson}, \bibfnamefont
  {J~P}}, \ and\ \bibinfo {author} {\bibfnamefont {W.~A.}\ \bibnamefont
  {Nierenberg}}} (\bibinfo {year} {1953}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {The statistics of a two-dimensional, hexagonal net},}\
  }\href {\doibase 10.1103/PhysRev.89.662} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {89}},\ \bibinfo {pages}
  {662--662}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hod}\ \emph {et~al.}(2007)\citenamefont {Hod},
  \citenamefont {Barone}, \citenamefont {Peralta},\ and\ \citenamefont
  {Scuseria}}]{HBPS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hod}, \bibfnamefont
  {Oded}}, \bibinfo {author} {\bibfnamefont {Ver{\'o}nica}\ \bibnamefont
  {Barone}}, \bibinfo {author} {\bibfnamefont {Juan~E.}\ \bibnamefont
  {Peralta}}, \ and\ \bibinfo {author} {\bibfnamefont {Gustavo~E.}\
  \bibnamefont {Scuseria}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Enhanced half-metallicity in edge-oxidized
  zigzag graphene nanoribbons},}\ }\href {\doibase 10.1021/nl0708922}
  {\bibfield  {journal} {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo
  {volume} {7}}~(\bibinfo {number} {8}),\ \bibinfo {pages}
  {2295--2299}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Horovitz}\ and\ \citenamefont
  {Doussal}(2002)}]{HD02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Horovitz},
  \bibfnamefont {Baruch}}, \ and\ \bibinfo {author} {\bibfnamefont {Pierre~Le}\
  \bibnamefont {Doussal}}} (\bibinfo {year} {2002}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Freezing transitions and the density of states
  of two-dimensional random dirac hamiltonians},}\ }\href {\doibase
  10.1103/PhysRevB.65.125323} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {65}},\ \bibinfo {pages}
  {125323}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hou}\ \emph {et~al.}(2007)\citenamefont {Hou},
  \citenamefont {Chamon},\ and\ \citenamefont {Mudry}}]{HCM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hou}, \bibfnamefont
  {Chang-Yu}}, \bibinfo {author} {\bibfnamefont {Claudio}\ \bibnamefont
  {Chamon}}, \ and\ \bibinfo {author} {\bibfnamefont {Christopher}\
  \bibnamefont {Mudry}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electron fractionalization in two-dimensional
  graphenelike structures},}\ }\href {\doibase 10.1103/PhysRevLett.98.186809}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {98}},\ \bibinfo {pages} {186809}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Huard}\ \emph {et~al.}(2007)\citenamefont {Huard},
  \citenamefont {Sulpizio}, \citenamefont {Stander}, \citenamefont {Todd},
  \citenamefont {Yang},\ and\ \citenamefont {Goldhaber-Gordon}}]{HSSTYG07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Huard}, \bibfnamefont
  {B}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Sulpizio}},
  \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Stander}}, \bibinfo
  {author} {\bibfnamefont {K.}~\bibnamefont {Todd}}, \bibinfo {author}
  {\bibfnamefont {B.}~\bibnamefont {Yang}}, \ and\ \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Goldhaber-Gordon}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Transport
  measurements across a tunable potential barrier in graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.236803} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {236803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Huertas-Hernando}\ \emph {et~al.}(2006)\citenamefont
  {Huertas-Hernando}, \citenamefont {Guinea},\ and\ \citenamefont
  {Brataas}}]{HGB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Huertas-Hernando},
  \bibfnamefont {Daniel}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {Arne}\ \bibnamefont
  {Brataas}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Spin-orbit coupling in curved graphene, fullerenes, nanotubes, and
  nanotube caps},}\ }\href {\doibase 10.1103/PhysRevB.74.155426} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {155426}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hwang}\ and\ \citenamefont
  {Das~Sarma}(2007)}]{HdS06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hwang}, \bibfnamefont
  {E~H}}, \ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Das~Sarma}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Dielectric function, screening, and plasmons in
  two-dimensional graphene},}\ }\href {\doibase 10.1103/PhysRevB.75.205418}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {205418}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hwang}\ \emph {et~al.}(2007)\citenamefont {Hwang},
  \citenamefont {Hu},\ and\ \citenamefont {Das~Sarma}}]{HHS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Hwang}, \bibfnamefont
  {E~H}}, \bibinfo {author} {\bibfnamefont {Ben Yu-Kuang}\ \bibnamefont {Hu}},
  \ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Das~Sarma}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Inelastic carrier lifetime in graphene},}\ }\href {\doibase
  10.1103/PhysRevB.76.115434} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {115434}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ishigami}\ \emph {et~al.}(2007)\citenamefont
  {Ishigami}, \citenamefont {Chen}, \citenamefont {Cullen}, \citenamefont
  {Fuhrer},\ and\ \citenamefont {Williams}}]{Ishal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ishigami},
  \bibfnamefont {Masa}}, \bibinfo {author} {\bibfnamefont {J.~H.}\ \bibnamefont
  {Chen}}, \bibinfo {author} {\bibfnamefont {W.~G.}\ \bibnamefont {Cullen}},
  \bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont {Fuhrer}}, \ and\
  \bibinfo {author} {\bibfnamefont {E.~D.}\ \bibnamefont {Williams}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Atomic
  structure of graphene on sio2},}\ }\href {\doibase 10.1021/nl070613a}
  {\bibfield  {journal} {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo
  {volume} {7}}~(\bibinfo {number} {6}),\ \bibinfo {pages}
  {1643--1648}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Itzykson}\ and\ \citenamefont
  {Zuber}(2006)}]{zuber06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Itzykson},
  \bibfnamefont {C}}, \ and\ \bibinfo {author} {\bibfnamefont {J.-B.}\
  \bibnamefont {Zuber}}} (\bibinfo {year} {2006}),\ \href@noop {} {\emph
  {\bibinfo {title} {Quantum Field Theory}}}\ (\bibinfo  {publisher}
  {Dover})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jackiw}\ and\ \citenamefont {Rebbi}(1976)}]{JR76}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Jackiw}, \bibfnamefont
  {R}}, \ and\ \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Rebbi}}}
  (\bibinfo {year} {1976}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Solitons with fermion number $\frac{1}{2}$},}\ }\href {\doibase
  10.1103/PhysRevD.13.3398} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. D}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages}
  {3398--3409}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jiang}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Jiang}, \citenamefont {Henriksen},
  \citenamefont {Tung}, \citenamefont {Wang}, \citenamefont {Schwartz},
  \citenamefont {Han}, \citenamefont {Kim},\ and\ \citenamefont
  {Stormer}}]{Jetal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Jiang}, \bibfnamefont
  {Z}}, \bibinfo {author} {\bibfnamefont {E.~A.}\ \bibnamefont {Henriksen}},
  \bibinfo {author} {\bibfnamefont {L.~C.}\ \bibnamefont {Tung}}, \bibinfo
  {author} {\bibfnamefont {Y.-J.}\ \bibnamefont {Wang}}, \bibinfo {author}
  {\bibfnamefont {M.~E.}\ \bibnamefont {Schwartz}}, \bibinfo {author}
  {\bibfnamefont {M.~Y.}\ \bibnamefont {Han}}, \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Kim}}, \ and\ \bibinfo {author} {\bibfnamefont {H.~L.}\
  \bibnamefont {Stormer}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Infrared spectroscopy of landau levels
  of graphene},}\ }\href {\doibase 10.1103/PhysRevLett.98.197403} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {98}},\ \bibinfo {pages} {197403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Jiang}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Jiang}, \citenamefont {Zhang},
  \citenamefont {Stormer},\ and\ \citenamefont {Kim}}]{JZSK07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Jiang}, \bibfnamefont
  {Z}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Zhang}}, \bibinfo
  {author} {\bibfnamefont {H.~L.}\ \bibnamefont {Stormer}}, \ and\ \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Kim}}} (\bibinfo {year}
  {2007}{\natexlab{b}}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Quantum hall states near the charge-neutral dirac point in graphene},}\
  }\href {\doibase 10.1103/PhysRevLett.99.106802} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\
  \bibinfo {pages} {106802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kane}\ and\ \citenamefont {Mele}(1997)}]{KM97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kane}, \bibfnamefont
  {C~L}}, \ and\ \bibinfo {author} {\bibfnamefont {E.~J.}\ \bibnamefont
  {Mele}}} (\bibinfo {year} {1997}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Size, shape, and low energy electronic structure of carbon
  nanotubes},}\ }\href {\doibase 10.1103/PhysRevLett.78.1932} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {78}},\ \bibinfo {pages} {1932--1935}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kane}\ and\ \citenamefont {Mele}(2004)}]{KM04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kane}, \bibfnamefont
  {C~L}}, \ and\ \bibinfo {author} {\bibfnamefont {E.~J.}\ \bibnamefont
  {Mele}}} (\bibinfo {year} {2004}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electron interactions and scaling relations for optical excitations
  in carbon nanotubes},}\ }\href {\doibase 10.1103/PhysRevLett.93.197402}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {93}},\ \bibinfo {pages} {197402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kane}\ and\ \citenamefont {Mele}(2005)}]{KM05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kane}, \bibfnamefont
  {C~L}}, \ and\ \bibinfo {author} {\bibfnamefont {E.~J.}\ \bibnamefont
  {Mele}}} (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum spin hall effect in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.95.226801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {95}},\ \bibinfo {pages}
  {226801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Katsnelson}(2006{\natexlab{a}})}]{Kscreening}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {M~I}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Nonlinear screening of charge impurities
  in graphene},}\ }\href {\doibase 10.1103/PhysRevB.74.201401} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {201401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Katsnelson}(2006{\natexlab{b}})}]{K06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {M~I}}} (\bibinfo {year} {2006}{\natexlab{b}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Zitterbewegung, chirality, and minimal
  conductivity in graphene},}\ }\href
  {http://dx.doi.org/10.1140/epjb/e2006-00203-1} {\bibfield  {journal}
  {\bibinfo  {journal} {The European Physical Journal B - Condensed Matter and
  Complex Systems}\ }\textbf {\bibinfo {volume} {51}},\ \bibinfo {pages}
  {157--160}},\ \bibinfo {note} {10.1140/epjb/e2006-00203-1}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Katsnelson}(2007{\natexlab{a}})}]{Kats0703}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {M~I}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Conductance quantization in graphene
  nanoribbons: adiabatic approximation},}\ }\href
  {http://dx.doi.org/10.1140/epjb/e2007-00168-5} {\bibfield  {journal}
  {\bibinfo  {journal} {The European Physical Journal B - Condensed Matter and
  Complex Systems}\ }\textbf {\bibinfo {volume} {57}},\ \bibinfo {pages}
  {225--228}},\ \bibinfo {note} {10.1140/epjb/e2007-00168-5}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Katsnelson}(2007{\natexlab{b}})}]{Kats07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {M~I}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Scattering of charge carriers by point
  defects in bilayer graphene},}\ }\href {\doibase 10.1103/PhysRevB.76.073411}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {76}},\ \bibinfo {pages} {073411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Katsnelson}\ and\ \citenamefont {Geim}(2008)}]{KG07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {MI}}, \ and\ \bibinfo {author} {\bibfnamefont {A.K}\
  \bibnamefont {Geim}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electron scattering on microscopic corrugations in
  graphene},}\ }\href {\doibase 10.1098/rsta.2007.2157} {\bibfield  {journal}
  {\bibinfo  {journal} {Philosophical Transactions of the Royal Society A:
  Mathematical, Physical and Engineering Sciences}\ }\textbf {\bibinfo {volume}
  {366}}~(\bibinfo {number} {1863}),\ \bibinfo {pages} {195--204}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Katsnelson}(2007{\natexlab{c}})}]{KMT}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Katsnelson},
  \bibfnamefont {Mikhail~I}}} (\bibinfo {year} {2007}{\natexlab{c}}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Graphene: carbon in two
  dimensions},}\ }\href {\doibase 10.1016/S1369-7021(06)71788-6} {\bibfield
  {journal} {\bibinfo  {journal} {Materials Today}\ }\textbf {\bibinfo {volume}
  {10}},\ \bibinfo {pages} {20 -- 27}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kechedzhi}\ \emph {et~al.}(2007)\citenamefont
  {Kechedzhi}, \citenamefont {Fal'ko}, \citenamefont {McCann},\ and\
  \citenamefont {Altshuler}}]{KFMA07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kechedzhi},
  \bibfnamefont {K}}, \bibinfo {author} {\bibfnamefont {Vladimir~I.}\
  \bibnamefont {Fal'ko}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont
  {McCann}}, \ and\ \bibinfo {author} {\bibfnamefont {B.~L.}\ \bibnamefont
  {Altshuler}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Influence of trigonal warping on interference effects in
  bilayer graphene},}\ }\href {\doibase 10.1103/PhysRevLett.98.176806}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {98}},\ \bibinfo {pages} {176806}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Khveshchenko}(2001)}]{K01}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Khveshchenko},
  \bibfnamefont {D~V}}} (\bibinfo {year} {2001}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Ghost excitonic insulator transition in layered
  graphite},}\ }\href {\doibase 10.1103/PhysRevLett.87.246802} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {87}},\ \bibinfo {pages} {246802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kim}\ and\ \citenamefont {Neto}(2008)}]{NK07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kim}, \bibfnamefont
  {Eun-Ah}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\
  \bibnamefont {Neto}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Graphene as an electronic membrane},}\ }\href
  {http://stacks.iop.org/0295-5075/84/i=5/a=57007} {\bibfield  {journal}
  {\bibinfo  {journal} {EPL (Europhysics Letters)}\ }\textbf {\bibinfo {volume}
  {84}}~(\bibinfo {number} {5}),\ \bibinfo {pages} {57007}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Kobayashi}\ \emph {et~al.}(2005)\citenamefont
  {Kobayashi}, \citenamefont {Fukui}, \citenamefont {Enoki}, \citenamefont
  {Kusakabe},\ and\ \citenamefont {Kaburagi}}]{Ketal05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kobayashi},
  \bibfnamefont {Yousuke}}, \bibinfo {author} {\bibfnamefont {Ken-ichi}\
  \bibnamefont {Fukui}}, \bibinfo {author} {\bibfnamefont {Toshiaki}\
  \bibnamefont {Enoki}}, \bibinfo {author} {\bibfnamefont {Koichi}\
  \bibnamefont {Kusakabe}}, \ and\ \bibinfo {author} {\bibfnamefont {Yutaka}\
  \bibnamefont {Kaburagi}}} (\bibinfo {year} {2005}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Observation of zigzag and armchair edges of
  graphite using scanning tunneling microscopy and spectroscopy},}\ }\href
  {\doibase 10.1103/PhysRevB.71.193406} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo
  {pages} {193406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kolesnikov}\ and\ \citenamefont
  {Osipov}(2004)}]{KO04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kolesnikov},
  \bibfnamefont {D}}, \ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont
  {Osipov}}} (\bibinfo {year} {2004}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electronic structure of carbon nanohorns near the fermi level},}\
  }\href {http://dx.doi.org/10.1134/1.1787100} {\bibfield  {journal} {\bibinfo
  {journal} {JETP Letters}\ }\textbf {\bibinfo {volume} {79}},\ \bibinfo
  {pages} {532--536}},\ \bibinfo {note} {10.1134/1.1787100}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Kolesnikov}\ and\ \citenamefont
  {Osipov}(2006)}]{KO06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kolesnikov},
  \bibfnamefont {D~V}}, \ and\ \bibinfo {author} {\bibfnamefont {V.~A.}\
  \bibnamefont {Osipov}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {The continuum gauge field-theory model for
  low-energy electronic states of icosahedral fullerenes},}\ }\href
  {http://dx.doi.org/10.1140/epjb/e2006-00087-y} {\bibfield  {journal}
  {\bibinfo  {journal} {The European Physical Journal B - Condensed Matter and
  Complex Systems}\ }\textbf {\bibinfo {volume} {49}},\ \bibinfo {pages}
  {465--470}},\ \bibinfo {note} {10.1140/epjb/e2006-00087-y}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Kolezhuk}\ \emph {et~al.}(2006)\citenamefont
  {Kolezhuk}, \citenamefont {Sachdev}, \citenamefont {Biswas},\ and\
  \citenamefont {Chen}}]{KSBC06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kolezhuk},
  \bibfnamefont {Alexei}}, \bibinfo {author} {\bibfnamefont {Subir}\
  \bibnamefont {Sachdev}}, \bibinfo {author} {\bibfnamefont {Rudro~R.}\
  \bibnamefont {Biswas}}, \ and\ \bibinfo {author} {\bibfnamefont {Peiqiu}\
  \bibnamefont {Chen}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Theory of quantum impurities in spin liquids},}\ }\href
  {\doibase 10.1103/PhysRevB.74.165114} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo
  {pages} {165114}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kopelevich}\ and\ \citenamefont
  {Esquinazi}(2007)}]{KE07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kopelevich},
  \bibfnamefont {Y}}, \ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Esquinazi}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Ferromagnetism and superconductivity in carbon-based
  systems},}\ }\href {http://dx.doi.org/10.1007/s10909-006-9286-5} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of Low Temperature Physics}\ }\textbf
  {\bibinfo {volume} {146}},\ \bibinfo {pages} {629--639}},\ \bibinfo {note}
  {10.1007/s10909-006-9286-5}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kopelevich}\ \emph {et~al.}(2006)\citenamefont
  {Kopelevich}, \citenamefont {Pantoja}, \citenamefont {da~Silva},
  \citenamefont {Mrowka},\ and\ \citenamefont {Esquinazi}}]{KPSME06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kopelevich},
  \bibfnamefont {Y}}, \bibinfo {author} {\bibfnamefont {J.C.~Medina}\
  \bibnamefont {Pantoja}}, \bibinfo {author} {\bibfnamefont {R.R.}\
  \bibnamefont {da~Silva}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Mrowka}}, \ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Esquinazi}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Anomalous hall effect in graphite},}\ }\href {\doibase
  10.1016/j.physleta.2006.02.034} {\bibfield  {journal} {\bibinfo  {journal}
  {Physics Letters A}\ }\textbf {\bibinfo {volume} {355}}~(\bibinfo {number}
  {3}),\ \bibinfo {pages} {233 -- 236}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kopelevich}\ \emph {et~al.}(2003)\citenamefont
  {Kopelevich}, \citenamefont {Torres}, \citenamefont {da~Silva}, \citenamefont
  {Mrowka}, \citenamefont {Kempa},\ and\ \citenamefont {Esquinazi}}]{Ketal03}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kopelevich},
  \bibfnamefont {Y}}, \bibinfo {author} {\bibfnamefont {J.~H.~S.}\ \bibnamefont
  {Torres}}, \bibinfo {author} {\bibfnamefont {R.~R.}\ \bibnamefont
  {da~Silva}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Mrowka}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Kempa}}, \ and\ \bibinfo
  {author} {\bibfnamefont {P.}~\bibnamefont {Esquinazi}}} (\bibinfo {year}
  {2003}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Reentrant metallic
  behavior of graphite in the quantum limit},}\ }\href {\doibase
  10.1103/PhysRevLett.90.156402} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {90}},\ \bibinfo {pages}
  {156402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Koshino}\ and\ \citenamefont {Ando}(2006)}]{KA06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Koshino}, \bibfnamefont
  {Mikito}}, \ and\ \bibinfo {author} {\bibfnamefont {Tsuneya}\ \bibnamefont
  {Ando}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Transport in bilayer graphene: Calculations within a self-consistent
  born approximation},}\ }\href {\doibase 10.1103/PhysRevB.73.245403}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {73}},\ \bibinfo {pages} {245403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Koshino}\ and\ \citenamefont {Ando}(2007)}]{KA0705}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Koshino}, \bibfnamefont
  {Mikito}}, \ and\ \bibinfo {author} {\bibfnamefont {Tsuneya}\ \bibnamefont
  {Ando}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Diamagnetism in disordered graphene},}\ }\href {\doibase
  10.1103/PhysRevB.75.235333} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {235333}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kumazaki}\ and\ \citenamefont
  {Hirashima}(2006)}]{KH06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kumazaki},
  \bibfnamefont {Hideki}}, \ and\ \bibinfo {author} {\bibfnamefont {Dai~S.}\
  \bibnamefont {Hirashima}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Effects of impurities in two-dimensional
  graphite},}\ }\href {\doibase 10.1143/JPSJ.75.053707} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of the Physical Society of Japan}\ }\textbf
  {\bibinfo {volume} {75}}~(\bibinfo {number} {5}),\ \bibinfo {pages}
  {053707}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kumazaki}\ and\ \citenamefont
  {Hirashima}(2007)}]{KH07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kumazaki},
  \bibfnamefont {Hideki}}, \ and\ \bibinfo {author} {\bibfnamefont {Dai~S.}\
  \bibnamefont {Hirashima}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Nonmagnetic-defect-induced magnetism in
  graphene},}\ }\href {\doibase 10.1143/JPSJ.76.064713} {\bibfield  {journal}
  {\bibinfo  {journal} {Journal of the Physical Society of Japan}\ }\textbf
  {\bibinfo {volume} {76}}~(\bibinfo {number} {6}),\ \bibinfo {pages}
  {064713}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kusminskiy}\ \emph {et~al.}(2008)\citenamefont
  {Kusminskiy}, \citenamefont {Nilsson}, \citenamefont {Campbell},\ and\
  \citenamefont {Castro~Neto}}]{KNCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Kusminskiy},
  \bibfnamefont {S~Viola}}, \bibinfo {author} {\bibfnamefont {Johan}\
  \bibnamefont {Nilsson}}, \bibinfo {author} {\bibfnamefont {D.~K.}\
  \bibnamefont {Campbell}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\
  \bibnamefont {Castro~Neto}}} (\bibinfo {year} {2008}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic compressibility of a graphene
  bilayer},}\ }\href {\doibase 10.1103/PhysRevLett.100.106805} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {100}},\ \bibinfo {pages} {106805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lammert}\ and\ \citenamefont {Crespi}(2004)}]{LC04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lammert}, \bibfnamefont
  {Paul~E}}, \ and\ \bibinfo {author} {\bibfnamefont {Vincent~H.}\ \bibnamefont
  {Crespi}}} (\bibinfo {year} {2004}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Graphene cones:$\hskip0.3em${}classification by fictitious flux and
  electronic properties},}\ }\href {\doibase 10.1103/PhysRevB.69.035406}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {69}},\ \bibinfo {pages} {035406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Laughlin}(1981)}]{laughlin}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Laughlin},
  \bibfnamefont {R~B}}} (\bibinfo {year} {1981}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Quantized hall conductivity in two dimensions},}\ }\href
  {\doibase 10.1103/PhysRevB.23.5632} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {23}},\ \bibinfo
  {pages} {5632--5633}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lazzeri}\ and\ \citenamefont {Mauri}(2006)}]{LM06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lazzeri}, \bibfnamefont
  {Michele}}, \ and\ \bibinfo {author} {\bibfnamefont {Francesco}\ \bibnamefont
  {Mauri}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Nonadiabatic kohn anomaly in a doped graphene monolayer},}\ }\href
  {\doibase 10.1103/PhysRevLett.97.266407} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo
  {pages} {266407}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {LeClair}(2000)}]{LC00}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {LeClair}, \bibfnamefont
  {Andr\'e}}} (\bibinfo {year} {2000}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Relevance of disorder for dirac fermions with imaginary vector
  potentials},}\ }\href {\doibase 10.1103/PhysRevLett.84.1292} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {84}},\ \bibinfo {pages} {1292--1295}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lee}(1993)}]{PLee93}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lee}, \bibfnamefont
  {Patrick~A}}} (\bibinfo {year} {1993}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Localized states in a \textit{d} -wave superconductor},}\
  }\href {\doibase 10.1103/PhysRevLett.71.1887} {\bibfield  {journal} {\bibinfo
   {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo
  {pages} {1887--1890}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lee}\ and\ \citenamefont
  {Ramakrishnan}(1985)}]{localization}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lee}, \bibfnamefont
  {Patrick~A}}, \ and\ \bibinfo {author} {\bibfnamefont {T.~V.}\ \bibnamefont
  {Ramakrishnan}}} (\bibinfo {year} {1985}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Disordered electronic systems},}\ }\href {\doibase
  10.1103/RevModPhys.57.287} {\bibfield  {journal} {\bibinfo  {journal} {Rev.
  Mod. Phys.}\ }\textbf {\bibinfo {volume} {57}},\ \bibinfo {pages}
  {287--337}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lee}\ and\ \citenamefont {Lee}(2005)}]{sungsik05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lee}, \bibfnamefont
  {Sung-Sik}}, \ and\ \bibinfo {author} {\bibfnamefont {Patrick~A.}\
  \bibnamefont {Lee}}} (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {U(1) gauge theory of the hubbard model: Spin liquid states
  and possible application to
  $\kappa{}\mathrm{\text{-}}(\mathrm{BEDT}\mathrm{\text{-}}\mathrm{TTF}{)}_{2}{\mathrm{cu}}_{2}(\mathrm{CN}{)}_{3}$},}\
  }\href {\doibase 10.1103/PhysRevLett.95.036403} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {95}},\
  \bibinfo {pages} {036403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Leenaerts}\ \emph {et~al.}(2008)\citenamefont
  {Leenaerts}, \citenamefont {Partoens},\ and\ \citenamefont
  {Peeters}}]{LPP07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Leenaerts},
  \bibfnamefont {O}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Partoens}}, \ and\ \bibinfo {author} {\bibfnamefont {F.~M.}\ \bibnamefont
  {Peeters}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Adsorption of ${\mathrm{h}}_{2}\mathrm{O}$,
  $\mathrm{N}{\mathrm{h}}_{3}$, co, $\mathrm{N}{\mathrm{o}}_{2}$, and no on
  graphene: A first-principles study},}\ }\href {\doibase
  10.1103/PhysRevB.77.125416} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo {pages}
  {125416}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lewenkopf}\ \emph {et~al.}(2008)\citenamefont
  {Lewenkopf}, \citenamefont {Mucciolo},\ and\ \citenamefont
  {Castro~Neto}}]{LMCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lewenkopf},
  \bibfnamefont {C~H}}, \bibinfo {author} {\bibfnamefont {E.~R.}\ \bibnamefont
  {Mucciolo}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Numerical studies of conductivity and fano factor in
  disordered graphene},}\ }\href {\doibase 10.1103/PhysRevB.77.081410}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {77}},\ \bibinfo {pages} {081410}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Li}\ \emph {et~al.}(2006)\citenamefont {Li},
  \citenamefont {Tsai}, \citenamefont {Padilla}, \citenamefont {Dordevic},
  \citenamefont {Burch}, \citenamefont {Wang},\ and\ \citenamefont
  {Basov}}]{Letal06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Li}, \bibfnamefont
  {Z~Q}}, \bibinfo {author} {\bibfnamefont {S.-W.}\ \bibnamefont {Tsai}},
  \bibinfo {author} {\bibfnamefont {W.~J.}\ \bibnamefont {Padilla}}, \bibinfo
  {author} {\bibfnamefont {S.~V.}\ \bibnamefont {Dordevic}}, \bibinfo {author}
  {\bibfnamefont {K.~S.}\ \bibnamefont {Burch}}, \bibinfo {author}
  {\bibfnamefont {Y.~J.}\ \bibnamefont {Wang}}, \ and\ \bibinfo {author}
  {\bibfnamefont {D.~N.}\ \bibnamefont {Basov}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Infrared probe of the
  anomalous magnetotransport of highly oriented pyrolytic graphite in the
  extreme quantum limit},}\ }\href {\doibase 10.1103/PhysRevB.74.195404}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {74}},\ \bibinfo {pages} {195404}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Louis}\ \emph {et~al.}(2007)\citenamefont {Louis},
  \citenamefont {Verg\'es}, \citenamefont {Guinea},\ and\ \citenamefont
  {Chiappe}}]{LVGC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Louis}, \bibfnamefont
  {E}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Verg\'es}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\ \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Chiappe}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Transport regimes
  in surface disordered graphene sheets},}\ }\href {\doibase
  10.1103/PhysRevB.75.085440} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {085440}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ludwig}\ \emph {et~al.}(1994)\citenamefont {Ludwig},
  \citenamefont {Fisher}, \citenamefont {Shankar},\ and\ \citenamefont
  {Grinstein}}]{LFSG94}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ludwig}, \bibfnamefont
  {Andreas W~W}}, \bibinfo {author} {\bibfnamefont {Matthew P.~A.}\
  \bibnamefont {Fisher}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Shankar}}, \ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Grinstein}}} (\bibinfo {year} {1994}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Integer quantum hall transition: An alternative approach
  and exact results},}\ }\href {\doibase 10.1103/PhysRevB.50.7526} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {50}},\ \bibinfo {pages} {7526--7552}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lukose}\ \emph {et~al.}(2007)\citenamefont {Lukose},
  \citenamefont {Shankar},\ and\ \citenamefont {Baskaran}}]{LSB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lukose}, \bibfnamefont
  {Vinu}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Shankar}}, \
  and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Baskaran}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Novel electric field effects on landau levels in graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.116802} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {116802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Luk'yanchuk}\ and\ \citenamefont
  {Kopelevich}(2004)}]{LK04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Luk'yanchuk},
  \bibfnamefont {Igor~A}}, \ and\ \bibinfo {author} {\bibfnamefont {Yakov}\
  \bibnamefont {Kopelevich}}} (\bibinfo {year} {2004}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Phase analysis of quantum oscillations in
  graphite},}\ }\href {\doibase 10.1103/PhysRevLett.93.166402} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {93}},\ \bibinfo {pages} {166402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ma\~nes}\ \emph {et~al.}(2007)\citenamefont
  {Ma\~nes}, \citenamefont {Guinea},\ and\ \citenamefont {Vozmediano}}]{MGV07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ma\~nes}, \bibfnamefont
  {J~L}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\
  \bibinfo {author} {\bibfnamefont {Mar{\'\i}a A.~H.}\ \bibnamefont
  {Vozmediano}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Existence and topological stability of fermi points in
  multilayered graphene},}\ }\href {\doibase 10.1103/PhysRevB.75.155424}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {155424}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Maiti}\ and\ \citenamefont {Sengupta}(2007)}]{M07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Maiti}, \bibfnamefont
  {Moitri}}, \ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont
  {Sengupta}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Josephson effect in graphene
  superconductor/barrier/superconductor junctions: Oscillatory behavior of the
  josephson current},}\ }\href {\doibase 10.1103/PhysRevB.76.054513} {\bibfield
   {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {054513}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Malard}\ \emph {et~al.}(2007)\citenamefont {Malard},
  \citenamefont {Nilsson}, \citenamefont {Elias}, \citenamefont {Brant},
  \citenamefont {Plentz}, \citenamefont {Alves}, \citenamefont {Castro~Neto},\
  and\ \citenamefont {Pimenta}}]{Malard07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Malard}, \bibfnamefont
  {L~M}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Nilsson}},
  \bibinfo {author} {\bibfnamefont {D.~C.}\ \bibnamefont {Elias}}, \bibinfo
  {author} {\bibfnamefont {J.~C.}\ \bibnamefont {Brant}}, \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Plentz}}, \bibinfo {author} {\bibfnamefont
  {E.~S.}\ \bibnamefont {Alves}}, \bibinfo {author} {\bibfnamefont {A.~H.}\
  \bibnamefont {Castro~Neto}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~A.}\
  \bibnamefont {Pimenta}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Probing the electronic structure of bilayer
  graphene by raman scattering},}\ }\href {\doibase 10.1103/PhysRevB.76.201401}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {76}},\ \bibinfo {pages} {201401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mallet}\ \emph {et~al.}(2007)\citenamefont {Mallet},
  \citenamefont {Varchon}, \citenamefont {Naud}, \citenamefont {Magaud},
  \citenamefont {Berger},\ and\ \citenamefont {Veuillen}}]{Metal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mallet}, \bibfnamefont
  {P}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Varchon}}, \bibinfo
  {author} {\bibfnamefont {C.}~\bibnamefont {Naud}}, \bibinfo {author}
  {\bibfnamefont {L.}~\bibnamefont {Magaud}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Berger}}, \ and\ \bibinfo {author} {\bibfnamefont {J.-Y.}\
  \bibnamefont {Veuillen}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electron states of mono- and bilayer graphene on
  sic probed by scanning-tunneling microscopy},}\ }\href {\doibase
  10.1103/PhysRevB.76.041403} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {041403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Maple}(1998)}]{hightc}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Maple}, \bibfnamefont
  {MB}}} (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {High-temperature superconductivity},}\ }\href {\doibase
  10.1016/S0304-8853(97)00999-2} {\bibfield  {journal} {\bibinfo  {journal}
  {Journal of Magnetism and Magnetic Materials}\ }\textbf {\bibinfo {volume}
  {177ÛÒ181, Part 1}}~(\bibinfo {number} {0}),\ \bibinfo {pages} {18 --
  30}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mariani}\ \emph {et~al.}(2007)\citenamefont
  {Mariani}, \citenamefont {Glazman}, \citenamefont {Kamenev},\ and\
  \citenamefont {von Oppen}}]{MGKO07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mariani}, \bibfnamefont
  {Eros}}, \bibinfo {author} {\bibfnamefont {Leonid~I.}\ \bibnamefont
  {Glazman}}, \bibinfo {author} {\bibfnamefont {Alex}\ \bibnamefont {Kamenev}},
  \ and\ \bibinfo {author} {\bibfnamefont {Felix}\ \bibnamefont {von Oppen}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Zero-bias anomaly in the tunneling density of states of graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.76.165402} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {165402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mariani}\ and\ \citenamefont {von
  Oppen}(2008)}]{mVO07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mariani}, \bibfnamefont
  {Eros}}, \ and\ \bibinfo {author} {\bibfnamefont {Felix}\ \bibnamefont {von
  Oppen}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Erratum: Flexural phonons in free-standing graphene [phys. rev.
  lett. 100, 076801 (2008)]},}\ }\href {\doibase
  10.1103/PhysRevLett.100.249901} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo {pages}
  {249901}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Martelo}\ \emph {et~al.}(1997)\citenamefont
  {Martelo}, \citenamefont {Dzierzawa}, \citenamefont {Siffert},\ and\
  \citenamefont {Baeriswyl}}]{martelo97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Martelo}, \bibfnamefont
  {LM}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Dzierzawa}},
  \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Siffert}}, \ and\
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Baeriswyl}}} (\bibinfo
  {year} {1997}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Mott-hubbard
  transition and antiferromagnetism on the honeycomb lattice},}\ }\href
  {http://dx.doi.org/10.1007/s002570050384} {\bibfield  {journal} {\bibinfo
  {journal} {Zeitschrift fÃ¼r Physik B Condensed Matter}\ }\textbf {\bibinfo
  {volume} {103}},\ \bibinfo {pages} {335--338}},\ \bibinfo {note}
  {10.1007/s002570050384}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Martin}}\ and\ \citenamefont
  {{Blanter}}(2009)}]{MB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Martin}},
  \bibfnamefont {I}}, \ and\ \bibinfo {author} {\bibfnamefont {Y.~M.}\
  \bibnamefont {{Blanter}}}} (\bibinfo {year} {2009}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {{Transport in disordered graphene
  nanoribbons}},}\ }\href {\doibase 10.1103/PhysRevB.79.235132} {\bibfield
  {journal} {\bibinfo  {journal} {\prb}\ }\textbf {\bibinfo {volume}
  {79}}~(\bibinfo {number} {23}),\ \bibinfo {eid} {235132}},\ \Eprint
  {http://arxiv.org/abs/0705.0532} {arXiv:0705.0532 [cond-mat.mes-hall]}
  \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Martins}\ \emph {et~al.}(2007)\citenamefont
  {Martins}, \citenamefont {Miwa}, \citenamefont {da~Silva},\ and\
  \citenamefont {Fazzio}}]{MMSF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Martins}, \bibfnamefont
  {T~B}}, \bibinfo {author} {\bibfnamefont {R.~H.}\ \bibnamefont {Miwa}},
  \bibinfo {author} {\bibfnamefont {Ant\^onio J.~R.}\ \bibnamefont {da~Silva}},
  \ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Fazzio}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic and transport properties of boron-doped graphene nanoribbons},}\
  }\href {\doibase 10.1103/PhysRevLett.98.196803} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\
  \bibinfo {pages} {196803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Matsui}\ \emph {et~al.}(2005)\citenamefont {Matsui},
  \citenamefont {Kambara}, \citenamefont {Niimi}, \citenamefont {Tagami},
  \citenamefont {Tsukada},\ and\ \citenamefont {Fukuyama}}]{Metal05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Matsui}, \bibfnamefont
  {T}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Kambara}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Niimi}}, \bibinfo {author}
  {\bibfnamefont {K.}~\bibnamefont {Tagami}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Tsukada}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Hiroshi}\ \bibnamefont {Fukuyama}}} (\bibinfo {year} {2005}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Sts observations of landau levels at
  graphite surfaces},}\ }\href {\doibase 10.1103/PhysRevLett.94.226403}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {94}},\ \bibinfo {pages} {226403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mattausch}\ and\ \citenamefont
  {Pankratov}(2007)}]{MO0704}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mattausch},
  \bibfnamefont {Alexander}}, \ and\ \bibinfo {author} {\bibfnamefont {Oleg}\
  \bibnamefont {Pankratov}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {\textit{Ab~Initio} study of graphene on sic},}\
  }\href {\doibase 10.1103/PhysRevLett.99.076802} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\
  \bibinfo {pages} {076802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McCann}\ \emph {et~al.}(2006)\citenamefont {McCann},
  \citenamefont {Kechedzhi}, \citenamefont {Fal'ko}, \citenamefont {Suzuura},
  \citenamefont {Ando},\ and\ \citenamefont {Altshuler}}]{Metal06b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McCann}, \bibfnamefont
  {E}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Kechedzhi}},
  \bibinfo {author} {\bibfnamefont {Vladimir~I.}\ \bibnamefont {Fal'ko}},
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Suzuura}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Ando}}, \ and\ \bibinfo {author}
  {\bibfnamefont {B.~L.}\ \bibnamefont {Altshuler}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Weak-localization
  magnetoresistance and valley symmetry in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.97.146805} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {146805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McCann}(2006)}]{MC06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McCann}, \bibfnamefont
  {Edward}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Asymmetry gap in the electronic band structure of bilayer
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.74.161403} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {161403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McCann}\ and\ \citenamefont {Fal'ko}(2006)}]{MF06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McCann}, \bibfnamefont
  {Edward}}, \ and\ \bibinfo {author} {\bibfnamefont {Vladimir~I.}\
  \bibnamefont {Fal'ko}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Landau-level degeneracy and quantum hall effect
  in a graphite bilayer},}\ }\href {\doibase 10.1103/PhysRevLett.96.086805}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {96}},\ \bibinfo {pages} {086805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McClure}(1956)}]{M56}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McClure}, \bibfnamefont
  {J~W}}} (\bibinfo {year} {1956}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Diamagnetism of graphite},}\ }\href {\doibase
  10.1103/PhysRev.104.666} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {104}},\ \bibinfo {pages}
  {666--671}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McClure}(1957)}]{M57}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McClure}, \bibfnamefont
  {J~W}}} (\bibinfo {year} {1957}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Band structure of graphite and de haas-van alphen effect},}\ }\href
  {\doibase 10.1103/PhysRev.108.612} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev.}\ }\textbf {\bibinfo {volume} {108}},\ \bibinfo {pages}
  {612--618}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McClure}(1958)}]{M58}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McClure}, \bibfnamefont
  {J~W}}} (\bibinfo {year} {1958}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Analysis of multicarrier galvanomagnetic data for graphite},}\
  }\href {\doibase 10.1103/PhysRev.112.715} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {112}},\ \bibinfo {pages}
  {715--721}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McClure}(1960)}]{M1960}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McClure}, \bibfnamefont
  {J~W}}} (\bibinfo {year} {1960}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Theory of diamagnetism of graphite},}\ }\href {\doibase
  10.1103/PhysRev.119.606} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {119}},\ \bibinfo {pages}
  {606--613}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {McEuen}\ \emph {et~al.}(1999)\citenamefont {McEuen},
  \citenamefont {Bockrath}, \citenamefont {Cobden}, \citenamefont {Yoon},\ and\
  \citenamefont {Louie}}]{Louie99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {McEuen}, \bibfnamefont
  {Paul~L}}, \bibinfo {author} {\bibfnamefont {Marc}\ \bibnamefont {Bockrath}},
  \bibinfo {author} {\bibfnamefont {David~H.}\ \bibnamefont {Cobden}}, \bibinfo
  {author} {\bibfnamefont {Young-Gui}\ \bibnamefont {Yoon}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Steven~G.}\ \bibnamefont {Louie}}} (\bibinfo {year}
  {1999}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Disorder,
  pseudospins, and backscattering in carbon nanotubes},}\ }\href {\doibase
  10.1103/PhysRevLett.83.5098} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {83}},\ \bibinfo {pages}
  {5098--5101}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Meyer}\ \emph {et~al.}(2007)\citenamefont {Meyer},
  \citenamefont {Geim}, \citenamefont {Katsnelson}, \citenamefont {Novoselov},
  \citenamefont {Obergfell}, \citenamefont {Roth}, \citenamefont {Girit},\ and\
  \citenamefont {Zettl}}]{MGKNORGZ07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Meyer}, \bibfnamefont
  {JC}}, \bibinfo {author} {\bibfnamefont {A.K.}\ \bibnamefont {Geim}},
  \bibinfo {author} {\bibfnamefont {M.I.}\ \bibnamefont {Katsnelson}}, \bibinfo
  {author} {\bibfnamefont {K.S.}\ \bibnamefont {Novoselov}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Obergfell}}, \bibinfo {author}
  {\bibfnamefont {S.}~\bibnamefont {Roth}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Girit}}, \ and\ \bibinfo {author} {\bibfnamefont
  {A.}~\bibnamefont {Zettl}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {On the roughness of single- and bi-layer
  graphene membranes},}\ }\href {\doibase 10.1016/j.ssc.2007.02.047} {\bibfield
   {journal} {\bibinfo  {journal} {Solid State Communications}\ }\textbf
  {\bibinfo {volume} {143}},\ \bibinfo {pages} {101 -- 109}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Miao}\ \emph {et~al.}(2007)\citenamefont {Miao},
  \citenamefont {Wijeratne}, \citenamefont {Zhang}, \citenamefont {Coskun},
  \citenamefont {Bao},\ and\ \citenamefont {Lau}}]{MWCZL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Miao}, \bibfnamefont
  {F}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Wijeratne}},
  \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Zhang}}, \bibinfo
  {author} {\bibfnamefont {U.~C.}\ \bibnamefont {Coskun}}, \bibinfo {author}
  {\bibfnamefont {W.}~\bibnamefont {Bao}}, \ and\ \bibinfo {author}
  {\bibfnamefont {C.~N.}\ \bibnamefont {Lau}}} (\bibinfo {year} {2007}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Phase-coherent transport in
  graphene quantum billiards},}\ }\href {\doibase 10.1126/science.1144359}
  {\bibfield  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo
  {volume} {317}}~(\bibinfo {number} {5844}),\ \bibinfo {pages}
  {1530--1533}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Min}\ \emph {et~al.}(2006)\citenamefont {Min},
  \citenamefont {Hill}, \citenamefont {Sinitsyn}, \citenamefont {Sahu},
  \citenamefont {Kleinman},\ and\ \citenamefont {MacDonald}}]{MHSSKM06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Min}, \bibfnamefont
  {Hongki}}, \bibinfo {author} {\bibfnamefont {J.~E.}\ \bibnamefont {Hill}},
  \bibinfo {author} {\bibfnamefont {N.~A.}\ \bibnamefont {Sinitsyn}}, \bibinfo
  {author} {\bibfnamefont {B.~R.}\ \bibnamefont {Sahu}}, \bibinfo {author}
  {\bibfnamefont {Leonard}\ \bibnamefont {Kleinman}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~H.}\ \bibnamefont {MacDonald}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Intrinsic and rashba
  spin-orbit interactions in graphene sheets},}\ }\href {\doibase
  10.1103/PhysRevB.74.165310} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo {pages}
  {165310}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mishchenko}(2007)}]{Mish07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mishchenko},
  \bibfnamefont {E~G}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Effect of electron-electron interactions on the
  conductivity of clean graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.98.216801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo {pages}
  {216801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Morozov}\ \emph {et~al.}(2006)\citenamefont
  {Morozov}, \citenamefont {Novoselov}, \citenamefont {Katsnelson},
  \citenamefont {Schedin}, \citenamefont {Ponomarenko}, \citenamefont {Jiang},\
  and\ \citenamefont {Geim}}]{Metal06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Morozov}, \bibfnamefont
  {S~V}}, \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}},
  \bibinfo {author} {\bibfnamefont {M.~I.}\ \bibnamefont {Katsnelson}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Schedin}}, \bibinfo
  {author} {\bibfnamefont {L.~A.}\ \bibnamefont {Ponomarenko}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Jiang}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Strong suppression of weak
  localization in graphene},}\ }\href {\doibase 10.1103/PhysRevLett.97.016801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {97}},\ \bibinfo {pages} {016801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Morozov}\ \emph {et~al.}(2005)\citenamefont
  {Morozov}, \citenamefont {Novoselov}, \citenamefont {Schedin}, \citenamefont
  {Jiang}, \citenamefont {Firsov},\ and\ \citenamefont {Geim}}]{Metal05c}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Morozov}, \bibfnamefont
  {S~V}}, \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Schedin}}, \bibinfo
  {author} {\bibfnamefont {D.}~\bibnamefont {Jiang}}, \bibinfo {author}
  {\bibfnamefont {A.~A.}\ \bibnamefont {Firsov}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year} {2005}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Two-dimensional electron and
  hole gases at the surface of graphite},}\ }\href {\doibase
  10.1103/PhysRevB.72.201401} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {72}},\ \bibinfo {pages}
  {201401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Morpurgo}\ and\ \citenamefont {Guinea}(2006)}]{MG06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Morpurgo},
  \bibfnamefont {A~F}}, \ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Guinea}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Intervalley scattering, long-range disorder, and
  effective time-reversal symmetry breaking in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.97.196804} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {196804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mrozowski}(1952)}]{M1952}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mrozowski},
  \bibfnamefont {S}}} (\bibinfo {year} {1952}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Semiconductivity and diamagnetism of polycrystalline
  graphite and condensed ring systems},}\ }\href {\doibase
  10.1103/PhysRev.85.609} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {85}},\ \bibinfo {pages}
  {609--620}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nakada}\ \emph {et~al.}(1996)\citenamefont {Nakada},
  \citenamefont {Fujita}, \citenamefont {Dresselhaus},\ and\ \citenamefont
  {Dresselhaus}}]{Nakada96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nakada}, \bibfnamefont
  {Kyoko}}, \bibinfo {author} {\bibfnamefont {Mitsutaka}\ \bibnamefont
  {Fujita}}, \bibinfo {author} {\bibfnamefont {Gene}\ \bibnamefont
  {Dresselhaus}}, \ and\ \bibinfo {author} {\bibfnamefont {Mildred~S.}\
  \bibnamefont {Dresselhaus}}} (\bibinfo {year} {1996}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Edge state in graphene ribbons: Nanometer size
  effect and edge shape dependence},}\ }\href {\doibase
  10.1103/PhysRevB.54.17954} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {54}},\ \bibinfo {pages}
  {17954--17961}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nakamura}(2007)}]{N2007}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nakamura},
  \bibfnamefont {Masaaki}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Orbital magnetism and transport phenomena in
  two-dimensional dirac fermions in a weak magnetic field},}\ }\href {\doibase
  10.1103/PhysRevB.76.113301} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {113301}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Nelson, D.R.}}\ and\ \citenamefont {{Peliti,
  L.}}(1987)}]{NP87}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Nelson, D.R.}},}, \
  and\ \bibinfo {author} {\bibnamefont {{Peliti, L.}}}} (\bibinfo {year}
  {1987}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Fluctuations in
  membranes with crystalline and hexatic order},}\ }\href {\doibase
  10.1051/jphys:019870048070108500} {\bibfield  {journal} {\bibinfo  {journal}
  {J. Phys. France}\ }\textbf {\bibinfo {volume} {48}}~(\bibinfo {number}
  {7}),\ \bibinfo {pages} {1085--1092}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Niimi}\ \emph {et~al.}(2006)\citenamefont {Niimi},
  \citenamefont {Kambara}, \citenamefont {Matsui}, \citenamefont {Yoshioka},\
  and\ \citenamefont {Fukuyama}}]{Netal06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Niimi}, \bibfnamefont
  {Y}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Kambara}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Matsui}}, \bibinfo {author}
  {\bibfnamefont {D.}~\bibnamefont {Yoshioka}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Hiroshi}\ \bibnamefont {Fukuyama}}} (\bibinfo {year}
  {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Real-space imaging
  of alternate localization and extension of quasi-two-dimensional electronic
  states at graphite surfaces in magnetic fields},}\ }\href {\doibase
  10.1103/PhysRevLett.97.236804} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {236804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nilsson}\ and\ \citenamefont
  {Castro~Neto}(2007)}]{NCV06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nilsson}, \bibfnamefont
  {Johan}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Impurities in a biased graphene bilayer},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.126801} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {126801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nilsson}\ \emph {et~al.}(2007)\citenamefont
  {Nilsson}, \citenamefont {Castro~Neto}, \citenamefont {Guinea},\ and\
  \citenamefont {Peres}}]{NCNGP07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nilsson}, \bibfnamefont
  {Johan}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}},
  \ and\ \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Transmission through a biased graphene bilayer barrier},}\ }\href {\doibase
  10.1103/PhysRevB.76.165416} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {165416}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nilsson}\ \emph {et~al.}(2008)\citenamefont
  {Nilsson}, \citenamefont {Castro~Neto}, \citenamefont {Guinea},\ and\
  \citenamefont {Peres}}]{NCNGP06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nilsson}, \bibfnamefont
  {Johan}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}},
  \ and\ \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}}}
  (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic properties of bilayer and multilayer graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.78.045405} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {78}},\ \bibinfo
  {pages} {045405}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nilsson}\ \emph
  {et~al.}(2006{\natexlab{a}})\citenamefont {Nilsson}, \citenamefont
  {Castro~Neto}, \citenamefont {Peres},\ and\ \citenamefont
  {Guinea}}]{NCNPG05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nilsson}, \bibfnamefont
  {Johan}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}, \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont
  {Peres}}, \ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electron-electron interactions and the phase
  diagram of a graphene bilayer},}\ }\href {\doibase
  10.1103/PhysRevB.73.214418} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo {pages}
  {214418}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nilsson}\ \emph
  {et~al.}(2006{\natexlab{b}})\citenamefont {Nilsson}, \citenamefont {Neto},
  \citenamefont {Guinea},\ and\ \citenamefont {Peres}}]{NNGP06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nilsson}, \bibfnamefont
  {Johan}}, \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\ \bibnamefont
  {Neto}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\
  \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}}} (\bibinfo
  {year} {2006}{\natexlab{b}}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic properties of graphene multilayers},}\ }\href {\doibase
  10.1103/PhysRevLett.97.266801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {266801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nomura}\ \emph {et~al.}(2007)\citenamefont {Nomura},
  \citenamefont {Koshino},\ and\ \citenamefont {Ryu}}]{NNPG06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nomura}, \bibfnamefont
  {Kentaro}}, \bibinfo {author} {\bibfnamefont {Mikito}\ \bibnamefont
  {Koshino}}, \ and\ \bibinfo {author} {\bibfnamefont {Shinsei}\ \bibnamefont
  {Ryu}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Topological delocalization of two-dimensional massless dirac
  fermions},}\ }\href {\doibase 10.1103/PhysRevLett.99.146806} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {99}},\ \bibinfo {pages} {146806}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nomura}\ and\ \citenamefont
  {MacDonald}(2007)}]{NMac06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nomura}, \bibfnamefont
  {Kentaro}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {MacDonald}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Quantum transport of massless dirac fermions},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.076602} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {076602}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nomura}\ and\ \citenamefont
  {MacDonald}(2006)}]{NKR07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nomura}, \bibfnamefont
  {Kentaro}}, \ and\ \bibinfo {author} {\bibfnamefont {Allan~H.}\ \bibnamefont
  {MacDonald}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Quantum hall ferromagnetism in graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.96.256602} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {96}},\ \bibinfo
  {pages} {256602}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novikov}(2007{\natexlab{a}})}]{NMac07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novikov}, \bibfnamefont
  {D~S}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Elastic scattering theory and transport in graphene},}\
  }\href {\doibase 10.1103/PhysRevB.76.245435} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {245435}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novikov}(2007{\natexlab{b}})}]{Nov07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novikov}, \bibfnamefont
  {D~S}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Numbers of donors and acceptors from transport
  measurements in graphene},}\ }\href {\doibase 10.1063/1.2779107} {\bibfield
  {journal} {\bibinfo  {journal} {Applied Physics Letters}\ }\textbf {\bibinfo
  {volume} {91}}~(\bibinfo {number} {10}),\ \bibinfo {eid}
  {102102}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novikov}(2007{\natexlab{c}})}]{Novapl07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novikov}, \bibfnamefont
  {D~S}}} (\bibinfo {year} {2007}{\natexlab{c}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Transverse field effect in graphene ribbons},}\ }\href
  {\doibase 10.1103/PhysRevLett.99.056802} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {056802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novoselov}\ \emph {et~al.}(2004)\citenamefont
  {Novoselov}, \citenamefont {Geim}, \citenamefont {Morozov}, \citenamefont
  {Jiang}, \citenamefont {Zhang}, \citenamefont {Dubonos}, \citenamefont
  {Grigorieva},\ and\ \citenamefont {Firsov}}]{Netal04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novoselov},
  \bibfnamefont {K~S}}, \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont
  {Geim}}, \bibinfo {author} {\bibfnamefont {S.~V.}\ \bibnamefont {Morozov}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Jiang}}, \bibinfo
  {author} {\bibfnamefont {Y.}~\bibnamefont {Zhang}}, \bibinfo {author}
  {\bibfnamefont {S.~V.}\ \bibnamefont {Dubonos}}, \bibinfo {author}
  {\bibfnamefont {I.~V.}\ \bibnamefont {Grigorieva}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~A.}\ \bibnamefont {Firsov}}} (\bibinfo {year} {2004}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Electric field effect in
  atomically thin carbon films},}\ }\href {\doibase 10.1126/science.1102896}
  {\bibfield  {journal} {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo
  {volume} {306}}~(\bibinfo {number} {5696}),\ \bibinfo {pages}
  {666--669}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novoselov}\ \emph {et~al.}(2005)\citenamefont
  {Novoselov}, \citenamefont {Jiang}, \citenamefont {Schedin}, \citenamefont
  {Booth}, \citenamefont {Khotkevich}, \citenamefont {Morozov},\ and\
  \citenamefont {Geim}}]{Netal05b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novoselov},
  \bibfnamefont {K~S}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Jiang}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Schedin}},
  \bibinfo {author} {\bibfnamefont {T.~J.}\ \bibnamefont {Booth}}, \bibinfo
  {author} {\bibfnamefont {V.~V.}\ \bibnamefont {Khotkevich}}, \bibinfo
  {author} {\bibfnamefont {S.~V.}\ \bibnamefont {Morozov}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}} (\bibinfo {year}
  {2005}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Two-dimensional
  atomic crystals},}\ }\href {\doibase 10.1073/pnas.0502848102} {\bibfield
  {journal} {\bibinfo  {journal} {Proceedings of the National Academy of
  Sciences of the United States of America}\ }\textbf {\bibinfo {volume}
  {102}}~(\bibinfo {number} {30}),\ \bibinfo {pages}
  {10451--10453}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Novoselov}\ \emph {et~al.}(2007)\citenamefont
  {Novoselov}, \citenamefont {Jiang}, \citenamefont {Zhang}, \citenamefont
  {Morozov}, \citenamefont {Stormer}, \citenamefont {Zeitler}, \citenamefont
  {Maan}, \citenamefont {Boebinger}, \citenamefont {Kim},\ and\ \citenamefont
  {Geim}}]{Netal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Novoselov},
  \bibfnamefont {K~S}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont
  {Jiang}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Zhang}},
  \bibinfo {author} {\bibfnamefont {S.~V.}\ \bibnamefont {Morozov}}, \bibinfo
  {author} {\bibfnamefont {H.~L.}\ \bibnamefont {Stormer}}, \bibinfo {author}
  {\bibfnamefont {U.}~\bibnamefont {Zeitler}}, \bibinfo {author} {\bibfnamefont
  {J.~C.}\ \bibnamefont {Maan}}, \bibinfo {author} {\bibfnamefont {G.~S.}\
  \bibnamefont {Boebinger}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Kim}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont
  {Geim}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Room-temperature quantum hall effect in graphene},}\ }\href
  {\doibase 10.1126/science.1137201} {\bibfield  {journal} {\bibinfo  {journal}
  {Science}\ }\textbf {\bibinfo {volume} {315}}~(\bibinfo {number} {5817}),\
  \bibinfo {pages} {1379}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Nozi\`eres}(1958)}]{N58}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Nozi\`eres},
  \bibfnamefont {Philippe}}} (\bibinfo {year} {1958}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Cyclotron resonance in graphite},}\ }\href
  {\doibase 10.1103/PhysRev.109.1510} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {109}},\ \bibinfo {pages}
  {1510--1521}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ohta}(1971{\natexlab{a}})}]{Ohta1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ohta}, \bibfnamefont
  {Kuniichi}}} (\bibinfo {year} {1971}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Broadening of landau levels in two-dimensional
  electron gas. ii. transverse magnetoconductance},}\ }\href {\doibase
  10.1143/JPSJ.31.1627} {\bibfield  {journal} {\bibinfo  {journal} {Journal of
  the Physical Society of Japan}\ }\textbf {\bibinfo {volume} {31}}~(\bibinfo
  {number} {6}),\ \bibinfo {pages} {1627--1638}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ohta}(1971{\natexlab{b}})}]{OSNNSS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ohta}, \bibfnamefont
  {Kuniichi}}} (\bibinfo {year} {1971}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Broadening of landau levels in two-dimensional
  electron gas: Its effect on surface capacitance},}\ }\href {\doibase
  10.1143/JJAP.10.850} {\bibfield  {journal} {\bibinfo  {journal} {Japanese
  Journal of Applied Physics}\ }\textbf {\bibinfo {volume} {10}}~(\bibinfo
  {number} {7}),\ \bibinfo {pages} {850--863}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ohta}\ \emph {et~al.}(2007)\citenamefont {Ohta},
  \citenamefont {Bostwick}, \citenamefont {McChesney}, \citenamefont {Seyller},
  \citenamefont {Horn},\ and\ \citenamefont {Rotenberg}}]{Ohta2}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ohta}, \bibfnamefont
  {Taisuke}}, \bibinfo {author} {\bibfnamefont {Aaron}\ \bibnamefont
  {Bostwick}}, \bibinfo {author} {\bibfnamefont {J.~L.}\ \bibnamefont
  {McChesney}}, \bibinfo {author} {\bibfnamefont {Thomas}\ \bibnamefont
  {Seyller}}, \bibinfo {author} {\bibfnamefont {Karsten}\ \bibnamefont {Horn}},
  \ and\ \bibinfo {author} {\bibfnamefont {Eli}\ \bibnamefont {Rotenberg}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Interlayer interaction and electronic screening in multilayer graphene
  investigated with angle-resolved photoemission spectroscopy},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.206802} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {206802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ohta}\ \emph {et~al.}(2006)\citenamefont {Ohta},
  \citenamefont {Bostwick}, \citenamefont {Seyller}, \citenamefont {Horn},\
  and\ \citenamefont {Rotenberg}}]{Oetal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ohta}, \bibfnamefont
  {Taisuke}}, \bibinfo {author} {\bibfnamefont {Aaron}\ \bibnamefont
  {Bostwick}}, \bibinfo {author} {\bibfnamefont {Thomas}\ \bibnamefont
  {Seyller}}, \bibinfo {author} {\bibfnamefont {Karsten}\ \bibnamefont {Horn}},
  \ and\ \bibinfo {author} {\bibfnamefont {Eli}\ \bibnamefont {Rotenberg}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Controlling the electronic structure of bilayer graphene},}\ }\href
  {\doibase 10.1126/science.1130681} {\bibfield  {journal} {\bibinfo  {journal}
  {Science}\ }\textbf {\bibinfo {volume} {313}}~(\bibinfo {number} {5789}),\
  \bibinfo {pages} {951--954}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Oshima}\ and\ \citenamefont
  {Nagashima}(1997)}]{ON97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Oshima}, \bibfnamefont
  {Chuhei}}, \ and\ \bibinfo {author} {\bibfnamefont {Ayato}\ \bibnamefont
  {Nagashima}}} (\bibinfo {year} {1997}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Ultra-thin epitaxial films of graphite and hexagonal boron
  nitride on solid surfaces},}\ }\href
  {http://stacks.iop.org/0953-8984/9/i=1/a=004} {\bibfield  {journal} {\bibinfo
   {journal} {Journal of Physics: Condensed Matter}\ }\textbf {\bibinfo
  {volume} {9}}~(\bibinfo {number} {1}),\ \bibinfo {pages} {1}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Osipov}\ \emph {et~al.}(2003)\citenamefont {Osipov},
  \citenamefont {Kochetov},\ and\ \citenamefont {Pudlak}}]{OKP03}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Osipov}, \bibfnamefont
  {V}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Kochetov}}, \ and\
  \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Pudlak}}} (\bibinfo
  {year} {2003}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Electronic
  structure of carbon nanoparticles},}\ }\href
  {http://dx.doi.org/10.1134/1.1545393} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of Experimental and Theoretical Physics}\ }\textbf
  {\bibinfo {volume} {96}},\ \bibinfo {pages} {140--149}},\ \bibinfo {note}
  {10.1134/1.1545393}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ossipov}\ \emph {et~al.}(2007)\citenamefont
  {Ossipov}, \citenamefont {Titov},\ and\ \citenamefont {Beenakker}}]{OTB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ossipov}, \bibfnamefont
  {A}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Titov}}, \ and\
  \bibinfo {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont {Beenakker}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Reentrance effect in a graphene $n\text{-}p\text{-}n$ junction coupled to a
  superconductor},}\ }\href {\doibase 10.1103/PhysRevB.75.241401} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {75}},\ \bibinfo {pages} {241401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ostrovsky}\ \emph {et~al.}(2006)\citenamefont
  {Ostrovsky}, \citenamefont {Gornyi},\ and\ \citenamefont {Mirlin}}]{OGM06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ostrovsky},
  \bibfnamefont {P~M}}, \bibinfo {author} {\bibfnamefont {I.~V.}\ \bibnamefont
  {Gornyi}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~D.}\ \bibnamefont
  {Mirlin}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electron transport in disordered graphene},}\ }\href {\doibase
  10.1103/PhysRevB.74.235443} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo {pages}
  {235443}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ostrovsky}\ \emph {et~al.}(2007)\citenamefont
  {Ostrovsky}, \citenamefont {Gornyi},\ and\ \citenamefont {Mirlin}}]{OGM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ostrovsky},
  \bibfnamefont {P~M}}, \bibinfo {author} {\bibfnamefont {I.~V.}\ \bibnamefont
  {Gornyi}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~D.}\ \bibnamefont
  {Mirlin}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum criticality and minimal conductivity in graphene with
  long-range disorder},}\ }\href {\doibase 10.1103/PhysRevLett.98.256801}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {98}},\ \bibinfo {pages} {256801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {\"Ozyilmaz}\ \emph {et~al.}(2007)\citenamefont
  {\"Ozyilmaz}, \citenamefont {Jarillo-Herrero}, \citenamefont {Efetov},
  \citenamefont {Abanin}, \citenamefont {Levitov},\ and\ \citenamefont
  {Kim}}]{OJEALK07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {\"Ozyilmaz},
  \bibfnamefont {Barbaros}}, \bibinfo {author} {\bibfnamefont {Pablo}\
  \bibnamefont {Jarillo-Herrero}}, \bibinfo {author} {\bibfnamefont {Dmitri}\
  \bibnamefont {Efetov}}, \bibinfo {author} {\bibfnamefont {Dmitry~A.}\
  \bibnamefont {Abanin}}, \bibinfo {author} {\bibfnamefont {Leonid~S.}\
  \bibnamefont {Levitov}}, \ and\ \bibinfo {author} {\bibfnamefont {Philip}\
  \bibnamefont {Kim}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electronic transport and quantum hall effect in bipolar
  graphene $p\mathrm{\text{-}}n\mathrm{\text{-}}p$ junctions},}\ }\href
  {\doibase 10.1103/PhysRevLett.99.166804} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {166804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Paiva}\ \emph {et~al.}(2005)\citenamefont {Paiva},
  \citenamefont {Scalettar}, \citenamefont {Zheng}, \citenamefont {Singh},\
  and\ \citenamefont {Oitmaa}}]{paiva05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Paiva}, \bibfnamefont
  {Thereza}}, \bibinfo {author} {\bibfnamefont {R.~T.}\ \bibnamefont
  {Scalettar}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Zheng}},
  \bibinfo {author} {\bibfnamefont {R.~R.~P.}\ \bibnamefont {Singh}}, \ and\
  \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Oitmaa}}} (\bibinfo
  {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Ground-state
  and finite-temperature signatures of quantum phase transitions in the
  half-filled hubbard model on a honeycomb lattice},}\ }\href {\doibase
  10.1103/PhysRevB.72.085123} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {72}},\ \bibinfo {pages}
  {085123}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {V\'azquez~de Parga}\ \emph
  {et~al.}(2008)\citenamefont {V\'azquez~de Parga}, \citenamefont {Calleja},
  \citenamefont {Borca}, \citenamefont {Passeggi}, \citenamefont {Hinarejos},
  \citenamefont {Guinea},\ and\ \citenamefont {Miranda}}]{Vetal07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {V\'azquez~de Parga},
  \bibfnamefont {A~L}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Calleja}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Borca}},
  \bibinfo {author} {\bibfnamefont {M.~C.~G.}\ \bibnamefont {Passeggi}},
  \bibinfo {author} {\bibfnamefont {J.~J.}\ \bibnamefont {Hinarejos}}, \bibinfo
  {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\ \bibinfo {author}
  {\bibfnamefont {R.}~\bibnamefont {Miranda}}} (\bibinfo {year} {2008}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Periodically rippled
  graphene: Growth and spatially resolved electronic structure},}\ }\href
  {\doibase 10.1103/PhysRevLett.100.056807} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo
  {pages} {056807}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Parr}\ \emph {et~al.}(1950)\citenamefont {Parr},
  \citenamefont {Craig},\ and\ \citenamefont {Ross}}]{Parr50}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Parr}, \bibfnamefont
  {Robert~G}}, \bibinfo {author} {\bibfnamefont {David~P.}\ \bibnamefont
  {Craig}}, \ and\ \bibinfo {author} {\bibfnamefont {Ian~G.}\ \bibnamefont
  {Ross}}} (\bibinfo {year} {1950}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Molecular orbital calculations of the lower excited electronic
  levels of benzene, configuration interaction included},}\ }\href {\doibase
  10.1063/1.1747540} {\bibfield  {journal} {\bibinfo  {journal} {The Journal of
  Chemical Physics}\ }\textbf {\bibinfo {volume} {18}}~(\bibinfo {number}
  {12}),\ \bibinfo {pages} {1561--1563}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Partoens}\ and\ \citenamefont {Peeters}(2006)}]{P72}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Partoens},
  \bibfnamefont {B}}, \ and\ \bibinfo {author} {\bibfnamefont {F.~M.}\
  \bibnamefont {Peeters}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {From graphene to graphite: Electronic structure
  around the $k$ point},}\ }\href {\doibase 10.1103/PhysRevB.74.075404}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {74}},\ \bibinfo {pages} {075404}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peliti}\ and\ \citenamefont {Leibler}(1985)}]{PL85}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peliti}, \bibfnamefont
  {L}}, \ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Leibler}}}
  (\bibinfo {year} {1985}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Effects of thermal fluctuations on systems with small surface tension},}\
  }\href {\doibase 10.1103/PhysRevLett.54.1690} {\bibfield  {journal} {\bibinfo
   {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {54}},\ \bibinfo
  {pages} {1690--1693}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pereira}\ \emph {et~al.}(2006)\citenamefont
  {Pereira}, \citenamefont {Guinea}, \citenamefont {Lopes~dos Santos},
  \citenamefont {Peres},\ and\ \citenamefont {Castro~Neto}}]{Petal06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Pereira}, \bibfnamefont
  {Vitor~M}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}},
  \bibinfo {author} {\bibfnamefont {J.~M.~B.}\ \bibnamefont {Lopes~dos
  Santos}}, \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}},
  \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont {Castro~Neto}}}
  (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Disorder induced localized states in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.96.036801} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {96}},\ \bibinfo {pages}
  {036801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pereira}\ \emph {et~al.}(2007)\citenamefont
  {Pereira}, \citenamefont {Nilsson},\ and\ \citenamefont
  {Castro~Neto}}]{PNCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Pereira}, \bibfnamefont
  {Vitor~M}}, \bibinfo {author} {\bibfnamefont {Johan}\ \bibnamefont
  {Nilsson}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Coulomb impurity problem in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.99.166802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {166802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pereira}\ \emph {et~al.}(2008)\citenamefont
  {Pereira}, \citenamefont {Lopes~dos Santos},\ and\ \citenamefont
  {Castro~Neto}}]{PLSCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Pereira}, \bibfnamefont
  {Vitor~M}}, \bibinfo {author} {\bibfnamefont {J.~M.~B.}\ \bibnamefont
  {Lopes~dos Santos}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\
  \bibnamefont {Castro~Neto}}} (\bibinfo {year} {2008}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Modeling disorder in graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.77.115109} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo
  {pages} {115109}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph {et~al.}(2004)\citenamefont {Peres},
  \citenamefont {Ara\'ujo},\ and\ \citenamefont {Bozi}}]{PAD04}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {M.~A.~N.}\ \bibnamefont
  {Ara\'ujo}}, \ and\ \bibinfo {author} {\bibfnamefont {Daniel}\ \bibnamefont
  {Bozi}}} (\bibinfo {year} {2004}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Phase diagram and magnetic collective excitations of the hubbard
  model for graphene sheets and layers},}\ }\href {\doibase
  10.1103/PhysRevB.70.195122} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {70}},\ \bibinfo {pages}
  {195122}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2006{\natexlab{a}})\citenamefont {Peres}, \citenamefont
  {Castro~Neto},\ and\ \citenamefont {Guinea}}]{nuno_cond}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}, \ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}} (\bibinfo {year} {2006}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Conductance quantization in mesoscopic
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.73.195411} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {73}},\ \bibinfo {pages} {195411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2006{\natexlab{b}})\citenamefont {Peres}, \citenamefont
  {Castro~Neto},\ and\ \citenamefont {Guinea}}]{nuno_confinement}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}, \ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}} (\bibinfo {year} {2006}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Dirac fermion confinement in graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.73.241403} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo
  {pages} {241403}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph {et~al.}(2005)\citenamefont {Peres},
  \citenamefont {Guinea},\ and\ \citenamefont {Castro~Neto}}]{PGN05b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \
  and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont {Castro~Neto}}}
  (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Coulomb interactions and ferromagnetism in pure and doped graphene},}\
  }\href {\doibase 10.1103/PhysRevB.72.174406} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {72}},\ \bibinfo
  {pages} {174406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2006{\natexlab{c}})\citenamefont {Peres}, \citenamefont {Guinea},\
  and\ \citenamefont {Castro~Neto}}]{PGC06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \
  and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont {Castro~Neto}}}
  (\bibinfo {year} {2006}{\natexlab{c}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electronic properties of disordered two-dimensional
  carbon},}\ }\href {\doibase 10.1103/PhysRevB.73.125411} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {73}},\
  \bibinfo {pages} {125411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Peres}, \citenamefont
  {Klironomos}, \citenamefont {Tsai}, \citenamefont {Santos}, \citenamefont
  {dos Santos},\ and\ \citenamefont {Neto}}]{nit_bor}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {F.~D.}\ \bibnamefont
  {Klironomos}}, \bibinfo {author} {\bibfnamefont {S.-W.}\ \bibnamefont
  {Tsai}}, \bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont {Santos}},
  \bibinfo {author} {\bibfnamefont {J.~M. B.~Lopes}\ \bibnamefont {dos
  Santos}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\
  \bibnamefont {Neto}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Electron waves in chemically substituted
  graphene},}\ }\href {http://stacks.iop.org/0295-5075/80/i=6/a=67007}
  {\bibfield  {journal} {\bibinfo  {journal} {EPL (Europhysics Letters)}\
  }\textbf {\bibinfo {volume} {80}}~(\bibinfo {number} {6}),\ \bibinfo {pages}
  {67007}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Peres}, \citenamefont {Lopes~dos
  Santos},\ and\ \citenamefont {Stauber}}]{PLS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {N~M~R}}, \bibinfo {author} {\bibfnamefont {J.~M.~B.}\ \bibnamefont
  {Lopes~dos Santos}}, \ and\ \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Stauber}}} (\bibinfo {year} {2007}{\natexlab{b}}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Phenomenological study of the
  electronic transport coefficients of graphene},}\ }\href {\doibase
  10.1103/PhysRevB.76.073412} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {073412}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Peres}\ \emph
  {et~al.}(2006{\natexlab{d}})\citenamefont {Peres}, \citenamefont {Guinea},\
  and\ \citenamefont {Neto}}]{PGN06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Peres}, \bibfnamefont
  {NMR}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\
  \bibinfo {author} {\bibfnamefont {A.H.~Castro}\ \bibnamefont {Neto}}}
  (\bibinfo {year} {2006}{\natexlab{d}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electronic properties of two-dimensional carbon},}\ }\href
  {\doibase 10.1016/j.aop.2006.04.006} {\bibfield  {journal} {\bibinfo
  {journal} {Annals of Physics}\ }\textbf {\bibinfo {volume} {321}}~(\bibinfo
  {number} {7}),\ \bibinfo {pages} {1559 -- 1567}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Phillips}(2006)}]{mottness}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Phillips},
  \bibfnamefont {Philip}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Mottness},}\ }\href {\doibase
  10.1016/j.aop.2006.04.003} {\bibfield  {journal} {\bibinfo  {journal} {Annals
  of Physics}\ }\textbf {\bibinfo {volume} {321}}~(\bibinfo {number} {7}),\
  \bibinfo {pages} {1634 -- 1650}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Polini}\ \emph {et~al.}(2007)\citenamefont {Polini},
  \citenamefont {Asgari}, \citenamefont {Barlas}, \citenamefont
  {Pereg-Barnea},\ and\ \citenamefont {MacDonald}}]{PABPM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Polini}, \bibfnamefont
  {Marco}}, \bibinfo {author} {\bibfnamefont {Reza}\ \bibnamefont {Asgari}},
  \bibinfo {author} {\bibfnamefont {Yafis}\ \bibnamefont {Barlas}}, \bibinfo
  {author} {\bibfnamefont {T.}~\bibnamefont {Pereg-Barnea}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.H.}\ \bibnamefont {MacDonald}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Graphene: A
  pseudochiral fermi liquid},}\ }\href {\doibase 10.1016/j.ssc.2007.04.035}
  {\bibfield  {journal} {\bibinfo  {journal} {Solid State Communications}\
  }\textbf {\bibinfo {volume} {143}}~(\bibinfo {number} {1--2}),\ \bibinfo
  {pages} {58--62}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Polkovnikov}(2002)}]{anatoli02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Polkovnikov},
  \bibfnamefont {Anatoli}}} (\bibinfo {year} {2002}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Kondo effect in $d$-wave superconductors},}\
  }\href {\doibase 10.1103/PhysRevB.65.064503} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {65}},\ \bibinfo
  {pages} {064503}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Polkovnikov}\ \emph {et~al.}(2001)\citenamefont
  {Polkovnikov}, \citenamefont {Sachdev},\ and\ \citenamefont {Vojta}}]{PSV01}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Polkovnikov},
  \bibfnamefont {Anatoli}}, \bibinfo {author} {\bibfnamefont {Subir}\
  \bibnamefont {Sachdev}}, \ and\ \bibinfo {author} {\bibfnamefont {Matthias}\
  \bibnamefont {Vojta}}} (\bibinfo {year} {2001}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Impurity in a $\mathit{d}$-wave superconductor:
  Kondo effect and stm spectra},}\ }\href {\doibase 10.1103/PhysRevLett.86.296}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {86}},\ \bibinfo {pages} {296--299}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Rammal, R.}}(1985)}]{rammal85}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Rammal, R.}},}}
  (\bibinfo {year} {1985}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Landau level spectrum of bloch electrons in a honeycomb lattice},}\ }\href
  {\doibase 10.1051/jphys:019850046080134500} {\bibfield  {journal} {\bibinfo
  {journal} {J. Phys. France}\ }\textbf {\bibinfo {volume} {46}}~(\bibinfo
  {number} {8}),\ \bibinfo {pages} {1345--1354}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Recher}\ \emph {et~al.}(2007)\citenamefont {Recher},
  \citenamefont {Trauzettel}, \citenamefont {Rycerz}, \citenamefont {Blanter},
  \citenamefont {Beenakker},\ and\ \citenamefont {Morpurgo}}]{RTBBM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Recher}, \bibfnamefont
  {P}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Trauzettel}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Rycerz}}, \bibinfo
  {author} {\bibfnamefont {Ya.~M.}\ \bibnamefont {Blanter}}, \bibinfo {author}
  {\bibfnamefont {C.~W.~J.}\ \bibnamefont {Beenakker}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~F.}\ \bibnamefont {Morpurgo}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Aharonov-bohm
  effect and broken valley degeneracy in graphene rings},}\ }\href {\doibase
  10.1103/PhysRevB.76.235404} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {235404}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Reich}\ \emph {et~al.}(2002)\citenamefont {Reich},
  \citenamefont {Maultzsch}, \citenamefont {Thomsen},\ and\ \citenamefont
  {Ordej\'on}}]{Retal02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Reich}, \bibfnamefont
  {S}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Maultzsch}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Thomsen}}, \ and\
  \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Ordej\'on}}} (\bibinfo
  {year} {2002}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Tight-binding description of graphene},}\ }\href {\doibase
  10.1103/PhysRevB.66.035412} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {66}},\ \bibinfo {pages}
  {035412}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Robinson}\ and\ \citenamefont
  {Schomerus}(2007)}]{RS06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Robinson},
  \bibfnamefont {John~P}}, \ and\ \bibinfo {author} {\bibfnamefont {Henning}\
  \bibnamefont {Schomerus}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic transport in
  normal-conductor/graphene/normal-conductor junctions and conditions for
  insulating behavior at a finite charge-carrier density},}\ }\href {\doibase
  10.1103/PhysRevB.76.115430} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {115430}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mu\~noz Rojas}\ \emph {et~al.}(2006)\citenamefont
  {Mu\~noz Rojas}, \citenamefont {Jacob}, \citenamefont {Fern\'andez-Rossier},\
  and\ \citenamefont {Palacios}}]{MJFP06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Mu\~noz Rojas},
  \bibfnamefont {F}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont
  {Jacob}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Fern\'andez-Rossier}}, \ and\ \bibinfo {author} {\bibfnamefont {J.~J.}\
  \bibnamefont {Palacios}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Coherent transport in graphene
  nanoconstrictions},}\ }\href {\doibase 10.1103/PhysRevB.74.195417} {\bibfield
   {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {74}},\ \bibinfo {pages} {195417}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rollings}\ \emph {et~al.}(2006)\citenamefont
  {Rollings}, \citenamefont {Gweon}, \citenamefont {Zhou}, \citenamefont {Mun},
  \citenamefont {McChesney}, \citenamefont {Hussain}, \citenamefont {Fedorov},
  \citenamefont {First}, \citenamefont {de~Heer},\ and\ \citenamefont
  {Lanzara}}]{Retal05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Rollings},
  \bibfnamefont {E}}, \bibinfo {author} {\bibfnamefont {G.-H.}\ \bibnamefont
  {Gweon}}, \bibinfo {author} {\bibfnamefont {S.Y.}\ \bibnamefont {Zhou}},
  \bibinfo {author} {\bibfnamefont {B.S.}\ \bibnamefont {Mun}}, \bibinfo
  {author} {\bibfnamefont {J.L.}\ \bibnamefont {McChesney}}, \bibinfo {author}
  {\bibfnamefont {B.S.}\ \bibnamefont {Hussain}}, \bibinfo {author}
  {\bibfnamefont {A.V.}\ \bibnamefont {Fedorov}}, \bibinfo {author}
  {\bibfnamefont {P.N.}\ \bibnamefont {First}}, \bibinfo {author}
  {\bibfnamefont {W.A.}\ \bibnamefont {de~Heer}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.}~\bibnamefont {Lanzara}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Synthesis and
  characterization of atomically thin graphite films on a silicon carbide
  substrate},}\ }\href {\doibase 10.1016/j.jpcs.2006.05.010} {\bibfield
  {journal} {\bibinfo  {journal} {Journal of Physics and Chemistry of Solids}\
  }\textbf {\bibinfo {volume} {67}}~(\bibinfo {number} {9--10}),\ \bibinfo
  {pages} {2172--2177}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rong}\ and\ \citenamefont {Kuiper}(1993)}]{Rong93}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Rong}, \bibfnamefont
  {Zhao~Y}}, \ and\ \bibinfo {author} {\bibfnamefont {Pieter}\ \bibnamefont
  {Kuiper}}} (\bibinfo {year} {1993}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electronic effects in scanning tunneling microscopy: Moir\'e pattern
  on a graphite surface},}\ }\href {\doibase 10.1103/PhysRevB.48.17427}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {48}},\ \bibinfo {pages} {17427--17431}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rosenstein}\ \emph {et~al.}(1989)\citenamefont
  {Rosenstein}, \citenamefont {Warr},\ and\ \citenamefont {Park}}]{RWP89}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Rosenstein},
  \bibfnamefont {Baruch}}, \bibinfo {author} {\bibfnamefont {Brian~J.}\
  \bibnamefont {Warr}}, \ and\ \bibinfo {author} {\bibfnamefont {Seon~H.}\
  \bibnamefont {Park}}} (\bibinfo {year} {1989}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Four-fermion theory is renormalizable in 2+1
  dimensions},}\ }\href {\doibase 10.1103/PhysRevLett.62.1433} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {62}},\ \bibinfo {pages} {1433--1436}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rosenstein}\ \emph {et~al.}(1991)\citenamefont
  {Rosenstein}, \citenamefont {Warr},\ and\ \citenamefont {Park}}]{RWP91}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Rosenstein},
  \bibfnamefont {Baruch}}, \bibinfo {author} {\bibfnamefont {Brian~J.}\
  \bibnamefont {Warr}}, \ and\ \bibinfo {author} {\bibfnamefont {Seon~H.}\
  \bibnamefont {Park}}} (\bibinfo {year} {1991}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Dynamical symmetry breaking in four-fermion interaction
  models},}\ }\href {\doibase 10.1016/0370-1573(91)90129-A} {\bibfield
  {journal} {\bibinfo  {journal} {Physics Reports}\ }\textbf {\bibinfo {volume}
  {205}}~(\bibinfo {number} {2}),\ \bibinfo {pages} {59 -- 108}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {{Russo}}\ \emph {et~al.}(2008)\citenamefont
  {{Russo}}, \citenamefont {{Oostinga}}, \citenamefont {{Wehenkel}},
  \citenamefont {{Heersche}}, \citenamefont {{Sobhani}}, \citenamefont
  {{Vandersypen}},\ and\ \citenamefont {{Morpurgo}}}]{ROWHSVM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Russo}}, \bibfnamefont
  {S}}, \bibinfo {author} {\bibfnamefont {J.~B.}\ \bibnamefont {{Oostinga}}},
  \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {{Wehenkel}}}, \bibinfo
  {author} {\bibfnamefont {H.~B.}\ \bibnamefont {{Heersche}}}, \bibinfo
  {author} {\bibfnamefont {S.~S.}\ \bibnamefont {{Sobhani}}}, \bibinfo {author}
  {\bibfnamefont {L.~M.~K.}\ \bibnamefont {{Vandersypen}}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~F.}\ \bibnamefont {{Morpurgo}}}} (\bibinfo {year}
  {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title} {{Observation of
  Aharonov-Bohm conductance oscillations in a graphene ring}},}\ }\href
  {\doibase 10.1103/PhysRevB.77.085413} {\bibfield  {journal} {\bibinfo
  {journal} {\prb}\ }\textbf {\bibinfo {volume} {77}}~(\bibinfo {number} {8}),\
  \bibinfo {eid} {085413}},\ \Eprint {http://arxiv.org/abs/0711.1508}
  {arXiv:0711.1508 [cond-mat.mes-hall]} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Rydberg}\ \emph {et~al.}(2003)\citenamefont
  {Rydberg}, \citenamefont {Dion}, \citenamefont {Jacobson}, \citenamefont
  {Schr\"oder}, \citenamefont {Hyldgaard}, \citenamefont {Simak}, \citenamefont
  {Langreth},\ and\ \citenamefont {Lundqvist}}]{langreth}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Rydberg}, \bibfnamefont
  {H}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Dion}}, \bibinfo
  {author} {\bibfnamefont {N.}~\bibnamefont {Jacobson}}, \bibinfo {author}
  {\bibfnamefont {E.}~\bibnamefont {Schr\"oder}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Hyldgaard}}, \bibinfo {author}
  {\bibfnamefont {S.~I.}\ \bibnamefont {Simak}}, \bibinfo {author}
  {\bibfnamefont {D.~C.}\ \bibnamefont {Langreth}}, \ and\ \bibinfo {author}
  {\bibfnamefont {B.~I.}\ \bibnamefont {Lundqvist}}} (\bibinfo {year} {2003}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Van der waals density
  functional for layered structures},}\ }\href {\doibase
  10.1103/PhysRevLett.91.126402} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {91}},\ \bibinfo {pages}
  {126402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ryu}\ \emph {et~al.}(2007)\citenamefont {Ryu},
  \citenamefont {Mudry}, \citenamefont {Obuse},\ and\ \citenamefont
  {Furusaki}}]{RMOF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ryu}, \bibfnamefont
  {Shinsei}}, \bibinfo {author} {\bibfnamefont {Christopher}\ \bibnamefont
  {Mudry}}, \bibinfo {author} {\bibfnamefont {Hideaki}\ \bibnamefont {Obuse}},
  \ and\ \bibinfo {author} {\bibfnamefont {Akira}\ \bibnamefont {Furusaki}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {${\mathbb{z}}_{2}$ topological term, the global anomaly, and the
  two-dimensional symplectic symmetry class of anderson localization},}\ }\href
  {\doibase 10.1103/PhysRevLett.99.116601} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {116601}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sadowski}\ \emph {et~al.}(2006)\citenamefont
  {Sadowski}, \citenamefont {Martinez}, \citenamefont {Potemski}, \citenamefont
  {Berger},\ and\ \citenamefont {de~Heer}}]{SMPBH06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sadowski},
  \bibfnamefont {M~L}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Martinez}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Potemski}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Berger}}, \ and\ \bibinfo
  {author} {\bibfnamefont {W.~A.}\ \bibnamefont {de~Heer}}} (\bibinfo {year}
  {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Landau level
  spectroscopy of ultrathin graphite layers},}\ }\href {\doibase
  10.1103/PhysRevLett.97.266405} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {266405}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Safran}(1984)}]{S1984}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Safran}, \bibfnamefont
  {S~A}}} (\bibinfo {year} {1984}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Stage dependence of magnetic susceptibility of intercalated
  graphite},}\ }\href {\doibase 10.1103/PhysRevB.30.421} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {30}},\
  \bibinfo {pages} {421--423}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Safran}\ and\ \citenamefont
  {DiSalvo}(1979)}]{SD1979}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Safran}, \bibfnamefont
  {S~A}}, \ and\ \bibinfo {author} {\bibfnamefont {F.~J.}\ \bibnamefont
  {DiSalvo}}} (\bibinfo {year} {1979}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Theory of magnetic susceptibility of graphite intercalation
  compounds},}\ }\href {\doibase 10.1103/PhysRevB.20.4889} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {20}},\ \bibinfo {pages} {4889--4895}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {{Saha}}\ \emph {et~al.}(2007)\citenamefont {{Saha}},
  \citenamefont {{Waghmare}}, \citenamefont {{Krishnamurthy}},\ and\
  \citenamefont {{Sood}}}]{SWKS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {{Saha}}, \bibfnamefont
  {S~K}}, \bibinfo {author} {\bibfnamefont {U.~V.}\ \bibnamefont {{Waghmare}}},
  \bibinfo {author} {\bibfnamefont {H.~R.}\ \bibnamefont {{Krishnamurthy}}}, \
  and\ \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont {{Sood}}}}
  (\bibinfo {year} {2007}),\ \href@noop {} {\enquote {\bibinfo {title}
  {Frequency shift of optical phonons in doped graphene layers},}\ }\Eprint
  {http://arxiv.org/abs/cond-mat/0702627} {arXiv:cond-mat/0702627} \BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Saito}\ \emph
  {et~al.}(1992{\natexlab{a}})\citenamefont {Saito}, \citenamefont {Fujita},
  \citenamefont {Dresselhaus},\ and\ \citenamefont {Dresselhaus}}]{SFDD092b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Saito}, \bibfnamefont
  {R}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Fujita}}, \bibinfo
  {author} {\bibfnamefont {G.}~\bibnamefont {Dresselhaus}}, \ and\ \bibinfo
  {author} {\bibfnamefont {M.~S}\ \bibnamefont {Dresselhaus}}} (\bibinfo {year}
  {1992}{\natexlab{a}}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Electronic structure of chiral graphene tubules},}\ }\href {\doibase
  10.1063/1.107080} {\bibfield  {journal} {\bibinfo  {journal} {Applied Physics
  Letters}\ }\textbf {\bibinfo {volume} {60}}~(\bibinfo {number} {18}),\
  \bibinfo {pages} {2204--2206}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Saito}\ \emph
  {et~al.}(1992{\natexlab{b}})\citenamefont {Saito}, \citenamefont {Fujita},
  \citenamefont {Dresselhaus},\ and\ \citenamefont {Dresselhaus}}]{SFDD092a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Saito}, \bibfnamefont
  {Riichiro}}, \bibinfo {author} {\bibfnamefont {Mitsutaka}\ \bibnamefont
  {Fujita}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Dresselhaus}},
  \ and\ \bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont {Dresselhaus}}}
  (\bibinfo {year} {1992}{\natexlab{b}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Electronic structure of graphene tubules based on
  ${\mathrm{c}}_{60}$},}\ }\href {\doibase 10.1103/PhysRevB.46.1804} {\bibfield
   {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {46}},\ \bibinfo {pages} {1804--1811}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {San-Jose}\ \emph {et~al.}(2007)\citenamefont
  {San-Jose}, \citenamefont {Prada},\ and\ \citenamefont {Golubev}}]{SPG07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {San-Jose},
  \bibfnamefont {Pablo}}, \bibinfo {author} {\bibfnamefont {Elsa}\ \bibnamefont
  {Prada}}, \ and\ \bibinfo {author} {\bibfnamefont {Dmitry~S.}\ \bibnamefont
  {Golubev}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Universal scaling of current fluctuations in disordered graphene},}\
  }\href {\doibase 10.1103/PhysRevB.76.195445} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {195445}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lopes~dos Santos}\ \emph {et~al.}(2007)\citenamefont
  {Lopes~dos Santos}, \citenamefont {Peres},\ and\ \citenamefont
  {Castro~Neto}}]{LSPCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Lopes~dos Santos},
  \bibfnamefont {J~M~B}}, \bibinfo {author} {\bibfnamefont {N.~M.~R.}\
  \bibnamefont {Peres}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\
  \bibnamefont {Castro~Neto}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Graphene bilayer with a twist: Electronic
  structure},}\ }\href {\doibase 10.1103/PhysRevLett.99.256802} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {99}},\ \bibinfo {pages} {256802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Saremi}(2007)}]{S07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Saremi}, \bibfnamefont
  {Saeed}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Rkky in half-filled bipartite lattices: Graphene as an example},}\
  }\href {\doibase 10.1103/PhysRevB.76.184430} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {184430}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schakel}(1991)}]{Sch91}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Schakel}, \bibfnamefont
  {Adriaan M~J}}} (\bibinfo {year} {1991}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Relativistic quantum hall effect},}\ }\href {\doibase
  10.1103/PhysRevD.43.1428} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. D}\ }\textbf {\bibinfo {volume} {43}},\ \bibinfo {pages}
  {1428--1431}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schomerus}(2007)}]{S06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Schomerus},
  \bibfnamefont {Henning}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Effective contact model for transport through
  weakly-doped graphene},}\ }\href {\doibase 10.1103/PhysRevB.76.045433}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {76}},\ \bibinfo {pages} {045433}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Schroeder}\ \emph {et~al.}(1968)\citenamefont
  {Schroeder}, \citenamefont {Dresselhaus},\ and\ \citenamefont
  {Javan}}]{SDJ68}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Schroeder},
  \bibfnamefont {P~R}}, \bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont
  {Dresselhaus}}, \ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont
  {Javan}}} (\bibinfo {year} {1968}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Location of electron and hole carriers in graphite from laser
  magnetoreflection data},}\ }\href {\doibase 10.1103/PhysRevLett.20.1292}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {20}},\ \bibinfo {pages} {1292--1295}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Semenoff}(1984)}]{semenoff84}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Semenoff},
  \bibfnamefont {Gordon~W}}} (\bibinfo {year} {1984}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Condensed-matter simulation of a
  three-dimensional anomaly},}\ }\href {\doibase 10.1103/PhysRevLett.53.2449}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {53}},\ \bibinfo {pages} {2449--2452}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sengupta}\ and\ \citenamefont
  {Baskaran}(2008)}]{SB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sengupta},
  \bibfnamefont {K}}, \ and\ \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont
  {Baskaran}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Tuning kondo physics in graphene with gate voltage},}\
  }\href {\doibase 10.1103/PhysRevB.77.045417} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo
  {pages} {045417}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Seo\'anez}\ \emph {et~al.}(2007)\citenamefont
  {Seo\'anez}, \citenamefont {Guinea},\ and\ \citenamefont
  {Castro~Neto}}]{SGCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Seo\'anez},
  \bibfnamefont {C}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont
  {Guinea}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Dissipation in graphene and nanotube resonators},}\ }\href
  {\doibase 10.1103/PhysRevB.76.125427} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {125427}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shankar}(1994)}]{S94}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shankar}, \bibfnamefont
  {R}}} (\bibinfo {year} {1994}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Renormalization-group approach to interacting fermions},}\ }\href
  {\doibase 10.1103/RevModPhys.66.129} {\bibfield  {journal} {\bibinfo
  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {66}},\ \bibinfo
  {pages} {129--192}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sharma}\ \emph {et~al.}(1974)\citenamefont {Sharma},
  \citenamefont {Johnson},\ and\ \citenamefont {McClure}}]{SJM1974}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sharma}, \bibfnamefont
  {M~P}}, \bibinfo {author} {\bibfnamefont {L.~G.}\ \bibnamefont {Johnson}}, \
  and\ \bibinfo {author} {\bibfnamefont {J.~W.}\ \bibnamefont {McClure}}}
  (\bibinfo {year} {1974}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Diamagnetism of graphite},}\ }\href {\doibase 10.1103/PhysRevB.9.2467}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {9}},\ \bibinfo {pages} {2467--2475}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shelton}\ \emph {et~al.}(1974)\citenamefont
  {Shelton}, \citenamefont {Patil},\ and\ \citenamefont {Blakely}}]{SPB74}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shelton}, \bibfnamefont
  {JC}}, \bibinfo {author} {\bibfnamefont {H.R.}\ \bibnamefont {Patil}}, \ and\
  \bibinfo {author} {\bibfnamefont {J.M.}\ \bibnamefont {Blakely}}} (\bibinfo
  {year} {1974}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Equilibrium
  segregation of carbon to a nickel (111) surface: A surface phase
  transition},}\ }\href {\doibase 10.1016/0039-6028(74)90272-6} {\bibfield
  {journal} {\bibinfo  {journal} {Surface Science}\ }\textbf {\bibinfo {volume}
  {43}}~(\bibinfo {number} {2}),\ \bibinfo {pages} {493 -- 520}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Sheng}\ \emph {et~al.}(2006)\citenamefont {Sheng},
  \citenamefont {Sheng},\ and\ \citenamefont {Weng}}]{SSW06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sheng}, \bibfnamefont
  {D~N}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Sheng}}, \ and\
  \bibinfo {author} {\bibfnamefont {Z.~Y.}\ \bibnamefont {Weng}}} (\bibinfo
  {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Quantum hall
  effect in graphene: Disorder effect and phase diagram},}\ }\href {\doibase
  10.1103/PhysRevB.73.233406} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo {pages}
  {233406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shklovskii}(2007)}]{Shk07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shklovskii},
  \bibfnamefont {B~I}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Simple model of coulomb disorder and screening in
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.76.233411} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {76}},\ \bibinfo {pages} {233411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shon}\ and\ \citenamefont {Ando}(1998)}]{Ando7}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shon}, \bibfnamefont
  {Nguyen~Hong}}, \ and\ \bibinfo {author} {\bibfnamefont {Tsuneya}\
  \bibnamefont {Ando}}} (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Quantum transport in two-dimensional graphite system},}\
  }\href {\doibase 10.1143/JPSJ.67.2421} {\bibfield  {journal} {\bibinfo
  {journal} {Journal of the Physical Society of Japan}\ }\textbf {\bibinfo
  {volume} {67}}~(\bibinfo {number} {7}),\ \bibinfo {pages}
  {2421--2429}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shung}(1986{\natexlab{a}})}]{S86}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shung}, \bibfnamefont
  {Kenneth W~K}}} (\bibinfo {year} {1986}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Dielectric function and plasmon structure of
  stage-1 intercalated graphite},}\ }\href {\doibase 10.1103/PhysRevB.34.979}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {34}},\ \bibinfo {pages} {979--993}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shung}(1986{\natexlab{b}})}]{S86b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shung}, \bibfnamefont
  {Kenneth W~K}}} (\bibinfo {year} {1986}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Lifetime effects in low-stage intercalated
  graphite systems},}\ }\href {\doibase 10.1103/PhysRevB.34.1264} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {34}},\ \bibinfo {pages} {1264--1272}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Shytov}\ \emph {et~al.}(2007)\citenamefont {Shytov},
  \citenamefont {Katsnelson},\ and\ \citenamefont {Levitov}}]{SKL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Shytov}, \bibfnamefont
  {A~V}}, \bibinfo {author} {\bibfnamefont {M.~I.}\ \bibnamefont {Katsnelson}},
  \ and\ \bibinfo {author} {\bibfnamefont {L.~S.}\ \bibnamefont {Levitov}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Vacuum polarization and screening of supercritical impurities in
  graphene},}\ }\href {\doibase 10.1103/PhysRevLett.99.236801} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {99}},\ \bibinfo {pages} {236801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Silvestrov}\ and\ \citenamefont
  {Efetov}(2007)}]{SE07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Silvestrov},
  \bibfnamefont {P~G}}, \ and\ \bibinfo {author} {\bibfnamefont {K.~B.}\
  \bibnamefont {Efetov}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Quantum dots in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.98.016802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo {pages}
  {016802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sinitsyna}\ and\ \citenamefont
  {Yaminsky}(2006)}]{SY06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sinitsyna},
  \bibfnamefont {O~V}}, \ and\ \bibinfo {author} {\bibfnamefont {Igor~V}\
  \bibnamefont {Yaminsky}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Atomic resolution probe microscopy of the
  graphite surface},}\ }\href {http://stacks.iop.org/0036-021X/75/i=1/a=R02}
  {\bibfield  {journal} {\bibinfo  {journal} {Russian Chemical Reviews}\
  }\textbf {\bibinfo {volume} {75}}~(\bibinfo {number} {1}),\ \bibinfo {pages}
  {23}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Skrypnyk}\ and\ \citenamefont {Loktev}(2006)}]{SL06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Skrypnyk},
  \bibfnamefont {Yu~V}}, \ and\ \bibinfo {author} {\bibfnamefont {V.~M.}\
  \bibnamefont {Loktev}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Impurity effects in a two-dimensional system
  with the dirac spectrum},}\ }\href {\doibase 10.1103/PhysRevB.73.241402}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {73}},\ \bibinfo {pages} {241402}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Skrypnyk}\ and\ \citenamefont {Loktev}(2007)}]{SL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Skrypnyk},
  \bibfnamefont {Yuriy~V}}, \ and\ \bibinfo {author} {\bibfnamefont {Vadim~M.}\
  \bibnamefont {Loktev}}} (\bibinfo {year} {2007}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Local spectrum rearrangement in impure
  graphene},}\ }\href {\doibase 10.1103/PhysRevB.75.245401} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {75}},\ \bibinfo {pages} {245401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Slonczewski}\ and\ \citenamefont
  {Weiss}(1958)}]{SW58}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Slonczewski},
  \bibfnamefont {J~C}}, \ and\ \bibinfo {author} {\bibfnamefont {P.~R.}\
  \bibnamefont {Weiss}}} (\bibinfo {year} {1958}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Band structure of graphite},}\ }\href {\doibase
  10.1103/PhysRev.109.272} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {109}},\ \bibinfo {pages}
  {272--279}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Snyman}\ and\ \citenamefont
  {Beenakker}(2007)}]{SB07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Snyman}, \bibfnamefont
  {I}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont
  {Beenakker}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Ballistic transmission through a graphene bilayer},}\
  }\href {\doibase 10.1103/PhysRevB.75.045322} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo
  {pages} {045322}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sols}\ \emph {et~al.}(2007)\citenamefont {Sols},
  \citenamefont {Guinea},\ and\ \citenamefont {Neto}}]{SGN07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sols}, \bibfnamefont
  {F}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\
  \bibinfo {author} {\bibfnamefont {A.~H.~Castro}\ \bibnamefont {Neto}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Coulomb blockade in graphene nanoribbons},}\ }\href {\doibase
  10.1103/PhysRevLett.99.166803} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo {pages}
  {166803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Son}(2007)}]{DTS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Son}, \bibfnamefont
  {D~T}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum critical point in graphene approached in the limit of
  infinitely strong coulomb interaction},}\ }\href {\doibase
  10.1103/PhysRevB.75.235423} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {235423}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Son}\ \emph {et~al.}(2006)\citenamefont {Son},
  \citenamefont {Cohen},\ and\ \citenamefont {Louie}}]{SCL06b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Son}, \bibfnamefont
  {Young-Woo}}, \bibinfo {author} {\bibfnamefont {Marvin~L.}\ \bibnamefont
  {Cohen}}, \ and\ \bibinfo {author} {\bibfnamefont {Steven~G.}\ \bibnamefont
  {Louie}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Energy gaps in graphene nanoribbons},}\ }\href {\doibase
  10.1103/PhysRevLett.97.216803} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo {pages}
  {216803}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sorella}\ and\ \citenamefont
  {Tosatti}(1992)}]{sorella92}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sorella}, \bibfnamefont
  {S}}, \ and\ \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Tosatti}}}
  (\bibinfo {year} {1992}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Semi-metal-insulator transition of the hubbard model in the honeycomb
  lattice},}\ }\href {http://stacks.iop.org/0295-5075/19/i=8/a=007} {\bibfield
  {journal} {\bibinfo  {journal} {EPL (Europhysics Letters)}\ }\textbf
  {\bibinfo {volume} {19}}~(\bibinfo {number} {8}),\ \bibinfo {pages}
  {699}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Soule}\ \emph {et~al.}(1964)\citenamefont {Soule},
  \citenamefont {McClure},\ and\ \citenamefont {Smith}}]{SMS64}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Soule}, \bibfnamefont
  {D~E}}, \bibinfo {author} {\bibfnamefont {J.~W.}\ \bibnamefont {McClure}}, \
  and\ \bibinfo {author} {\bibfnamefont {L.~B.}\ \bibnamefont {Smith}}}
  (\bibinfo {year} {1964}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Study of the shubnikov-de haas effect. determination of the fermi surfaces
  in graphite},}\ }\href {\doibase 10.1103/PhysRev.134.A453} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume}
  {134}},\ \bibinfo {pages} {A453--A470}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Spataru}\ \emph {et~al.}(2001)\citenamefont
  {Spataru}, \citenamefont {Cazalilla}, \citenamefont {Rubio}, \citenamefont
  {Benedict}, \citenamefont {Echenique},\ and\ \citenamefont
  {Louie}}]{SCABEL01}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Spataru}, \bibfnamefont
  {Catalin~D}}, \bibinfo {author} {\bibfnamefont {Miguel~A.}\ \bibnamefont
  {Cazalilla}}, \bibinfo {author} {\bibfnamefont {Angel}\ \bibnamefont
  {Rubio}}, \bibinfo {author} {\bibfnamefont {Lorin~X.}\ \bibnamefont
  {Benedict}}, \bibinfo {author} {\bibfnamefont {Pedro~M.}\ \bibnamefont
  {Echenique}}, \ and\ \bibinfo {author} {\bibfnamefont {Steven~G.}\
  \bibnamefont {Louie}}} (\bibinfo {year} {2001}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Anomalous quasiparticle lifetime in graphite:
  Band structure effects},}\ }\href {\doibase 10.1103/PhysRevLett.87.246405}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {87}},\ \bibinfo {pages} {246405}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Spry}\ and\ \citenamefont {Scherer}(1960)}]{SS60}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Spry}, \bibfnamefont
  {W~J}}, \ and\ \bibinfo {author} {\bibfnamefont {P.~M.}\ \bibnamefont
  {Scherer}}} (\bibinfo {year} {1960}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {de haas-van alphen effect in graphite between 3 and 85 kilogauss},}\
  }\href {\doibase 10.1103/PhysRev.120.826} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {120}},\ \bibinfo {pages}
  {826--829}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stauber}\ \emph {et~al.}(2005)\citenamefont
  {Stauber}, \citenamefont {Guinea},\ and\ \citenamefont {Vozmediano}}]{SGV05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Stauber}, \bibfnamefont
  {T}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\
  \bibinfo {author} {\bibfnamefont {M.~A.~H.}\ \bibnamefont {Vozmediano}}}
  (\bibinfo {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Disorder and interaction effects in two-dimensional graphene sheets},}\
  }\href {\doibase 10.1103/PhysRevB.71.041406} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo
  {pages} {041406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stauber}\ \emph {et~al.}(2007)\citenamefont
  {Stauber}, \citenamefont {Peres}, \citenamefont {Guinea},\ and\ \citenamefont
  {Castro~Neto}}]{SPGN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Stauber}, \bibfnamefont
  {T}}, \bibinfo {author} {\bibfnamefont {N.~M.~R.}\ \bibnamefont {Peres}},
  \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Guinea}}, \ and\ \bibinfo
  {author} {\bibfnamefont {A.~H.}\ \bibnamefont {Castro~Neto}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Fermi liquid
  theory of a fermi ring},}\ }\href {\doibase 10.1103/PhysRevB.75.115425}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {115425}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stephan}\ \emph {et~al.}(1994)\citenamefont
  {Stephan}, \citenamefont {Ajayan}, \citenamefont {Colliex}, \citenamefont
  {Redlich}, \citenamefont {Lambert}, \citenamefont {Bernier},\ and\
  \citenamefont {Lefin}}]{nano_boron}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Stephan}, \bibfnamefont
  {O}}, \bibinfo {author} {\bibfnamefont {P.~M.}\ \bibnamefont {Ajayan}},
  \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Colliex}}, \bibinfo
  {author} {\bibfnamefont {Ph.}\ \bibnamefont {Redlich}}, \bibinfo {author}
  {\bibfnamefont {J.~M.}\ \bibnamefont {Lambert}}, \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Bernier}}, \ and\ \bibinfo {author}
  {\bibfnamefont {P.}~\bibnamefont {Lefin}}} (\bibinfo {year} {1994}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Doping graphitic and carbon
  nanotube structures with boron and nitrogen},}\ }\href {\doibase
  10.1126/science.266.5191.1683} {\bibfield  {journal} {\bibinfo  {journal}
  {Science}\ }\textbf {\bibinfo {volume} {266}}~(\bibinfo {number} {5191}),\
  \bibinfo {pages} {1683--1685}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stolyarova}\ \emph {et~al.}(2007)\citenamefont
  {Stolyarova}, \citenamefont {Rim}, \citenamefont {Ryu}, \citenamefont
  {Maultzsch}, \citenamefont {Kim}, \citenamefont {Brus}, \citenamefont
  {Heinz}, \citenamefont {Hybertsen},\ and\ \citenamefont
  {Flynn}}]{SRRMKBHHF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Stolyarova},
  \bibfnamefont {Elena}}, \bibinfo {author} {\bibfnamefont {Kwang~Taeg}\
  \bibnamefont {Rim}}, \bibinfo {author} {\bibfnamefont {Sunmin}\ \bibnamefont
  {Ryu}}, \bibinfo {author} {\bibfnamefont {Janina}\ \bibnamefont {Maultzsch}},
  \bibinfo {author} {\bibfnamefont {Philip}\ \bibnamefont {Kim}}, \bibinfo
  {author} {\bibfnamefont {Louis~E.}\ \bibnamefont {Brus}}, \bibinfo {author}
  {\bibfnamefont {Tony~F.}\ \bibnamefont {Heinz}}, \bibinfo {author}
  {\bibfnamefont {Mark~S.}\ \bibnamefont {Hybertsen}}, \ and\ \bibinfo {author}
  {\bibfnamefont {George~W.}\ \bibnamefont {Flynn}}} (\bibinfo {year} {2007}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {High-resolution scanning
  tunneling microscopy imaging of mesoscopic graphene sheets on an insulating
  surface},}\ }\href {\doibase 10.1073/pnas.0703337104} {\bibfield  {journal}
  {\bibinfo  {journal} {Proceedings of the National Academy of Sciences}\
  }\textbf {\bibinfo {volume} {104}}~(\bibinfo {number} {22}),\ \bibinfo
  {pages} {9209--9212}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Su}\ \emph {et~al.}(1979)\citenamefont {Su},
  \citenamefont {Schrieffer},\ and\ \citenamefont {Heeger}}]{SSH79_PRL}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Su}, \bibfnamefont
  {W~P}}, \bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont {Schrieffer}},
  \ and\ \bibinfo {author} {\bibfnamefont {A.~J.}\ \bibnamefont {Heeger}}}
  (\bibinfo {year} {1979}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Solitons in polyacetylene},}\ }\href {\doibase 10.1103/PhysRevLett.42.1698}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {42}},\ \bibinfo {pages} {1698--1701}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Su}\ \emph {et~al.}(1980)\citenamefont {Su},
  \citenamefont {Schrieffer},\ and\ \citenamefont {Heeger}}]{SSH79_PRB}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Su}, \bibfnamefont
  {W~P}}, \bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont {Schrieffer}},
  \ and\ \bibinfo {author} {\bibfnamefont {A.~J.}\ \bibnamefont {Heeger}}}
  (\bibinfo {year} {1980}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Soliton excitations in polyacetylene},}\ }\href {\doibase
  10.1103/PhysRevB.22.2099} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {22}},\ \bibinfo {pages}
  {2099--2111}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sugawara}\ \emph {et~al.}(2007)\citenamefont
  {Sugawara}, \citenamefont {Sato}, \citenamefont {Souma}, \citenamefont
  {Takahashi},\ and\ \citenamefont {Suematsu}}]{SSSTS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Sugawara},
  \bibfnamefont {K}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont
  {Sato}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Souma}},
  \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Takahashi}}, \ and\
  \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Suematsu}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Anomalous
  quasiparticle lifetime and strong electron-phonon coupling in graphite},}\
  }\href {\doibase 10.1103/PhysRevLett.98.036801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\
  \bibinfo {pages} {036801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Suzuura}\ and\ \citenamefont
  {Ando}(2002{\natexlab{a}})}]{SA02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Suzuura}, \bibfnamefont
  {Hidekatsu}}, \ and\ \bibinfo {author} {\bibfnamefont {Tsuneya}\ \bibnamefont
  {Ando}}} (\bibinfo {year} {2002}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Crossover from symplectic to orthogonal class in
  a two-dimensional honeycomb lattice},}\ }\href {\doibase
  10.1103/PhysRevLett.89.266603} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {89}},\ \bibinfo {pages}
  {266603}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Suzuura}\ and\ \citenamefont
  {Ando}(2002{\natexlab{b}})}]{SA02b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Suzuura}, \bibfnamefont
  {Hidekatsu}}, \ and\ \bibinfo {author} {\bibfnamefont {Tsuneya}\ \bibnamefont
  {Ando}}} (\bibinfo {year} {2002}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Phonons and electron-phonon scattering in carbon
  nanotubes},}\ }\href {\doibase 10.1103/PhysRevB.65.235412} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume}
  {65}},\ \bibinfo {pages} {235412}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Swain}\ and\ \citenamefont
  {Andelman}(1999)}]{swain99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Swain}, \bibfnamefont
  {Peter~S}}, \ and\ \bibinfo {author} {\bibfnamefont {David}\ \bibnamefont
  {Andelman}}} (\bibinfo {year} {1999}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {The influence of substrate structure on membrane
  adhesion},}\ }\href {\doibase 10.1021/la990503m} {\bibfield  {journal}
  {\bibinfo  {journal} {Langmuir}\ }\textbf {\bibinfo {volume} {15}}~(\bibinfo
  {number} {26}),\ \bibinfo {pages} {8902--8914}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tersoff}(1992)}]{tersoff92}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tersoff}, \bibfnamefont
  {J}}} (\bibinfo {year} {1992}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Energies of fullerenes},}\ }\href {\doibase
  10.1103/PhysRevB.46.15546} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {46}},\ \bibinfo {pages}
  {15546--15549}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tikhonenko}\ \emph {et~al.}(2008)\citenamefont
  {Tikhonenko}, \citenamefont {Horsell}, \citenamefont {Gorbachev},\ and\
  \citenamefont {Savchenko}}]{THGS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tikhonenko},
  \bibfnamefont {F~V}}, \bibinfo {author} {\bibfnamefont {D.~W.}\ \bibnamefont
  {Horsell}}, \bibinfo {author} {\bibfnamefont {R.~V.}\ \bibnamefont
  {Gorbachev}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~K.}\ \bibnamefont
  {Savchenko}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Weak localization in graphene flakes},}\ }\href {\doibase
  10.1103/PhysRevLett.100.056802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo {pages}
  {056802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Titov}(2007)}]{T07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Titov}, \bibfnamefont
  {M}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Impurity-assisted tunneling in graphene},}\ }\href
  {http://stacks.iop.org/0295-5075/79/i=1/a=17004} {\bibfield  {journal}
  {\bibinfo  {journal} {EPL (Europhysics Letters)}\ }\textbf {\bibinfo {volume}
  {79}}~(\bibinfo {number} {1}),\ \bibinfo {pages} {17004}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Titov}\ and\ \citenamefont {Beenakker}(2006)}]{TB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Titov}, \bibfnamefont
  {M}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont
  {Beenakker}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Josephson effect in ballistic graphene},}\ }\href
  {\doibase 10.1103/PhysRevB.74.041401} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {74}},\ \bibinfo
  {pages} {041401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tom\'anek}\ \emph {et~al.}(1987)\citenamefont
  {Tom\'anek}, \citenamefont {Louie}, \citenamefont {Mamin}, \citenamefont
  {Abraham}, \citenamefont {Thomson}, \citenamefont {Ganz},\ and\ \citenamefont
  {Clarke}}]{Tetal87}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tom\'anek},
  \bibfnamefont {David}}, \bibinfo {author} {\bibfnamefont {Steven~G.}\
  \bibnamefont {Louie}}, \bibinfo {author} {\bibfnamefont {H.~Jonathon}\
  \bibnamefont {Mamin}}, \bibinfo {author} {\bibfnamefont {David~W.}\
  \bibnamefont {Abraham}}, \bibinfo {author} {\bibfnamefont {Ruth~Ellen}\
  \bibnamefont {Thomson}}, \bibinfo {author} {\bibfnamefont {Eric}\
  \bibnamefont {Ganz}}, \ and\ \bibinfo {author} {\bibfnamefont {John}\
  \bibnamefont {Clarke}}} (\bibinfo {year} {1987}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Theory and observation of highly asymmetric
  atomic structure in scanning-tunneling-microscopy images of graphite},}\
  }\href {\doibase 10.1103/PhysRevB.35.7790} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {35}},\ \bibinfo
  {pages} {7790--7793}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Trushin}\ and\ \citenamefont
  {Schliemann}(2007)}]{TS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Trushin}, \bibfnamefont
  {Maxim}}, \ and\ \bibinfo {author} {\bibfnamefont {John}\ \bibnamefont
  {Schliemann}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Minimum electrical and thermal conductivity of graphene: A
  quasiclassical approach},}\ }\href {\doibase 10.1103/PhysRevLett.99.216602}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {99}},\ \bibinfo {pages} {216602}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tu}\ and\ \citenamefont {Ou-Yang}(2002)}]{tu02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tu}, \bibfnamefont
  {Zhan-chun}}, \ and\ \bibinfo {author} {\bibfnamefont {Zhong-can}\
  \bibnamefont {Ou-Yang}}} (\bibinfo {year} {2002}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Single-walled and multiwalled carbon nanotubes
  viewed as elastic tubes with the effective young's moduli dependent on layer
  number},}\ }\href {\doibase 10.1103/PhysRevB.65.233407} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {65}},\
  \bibinfo {pages} {233407}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tworzyd\l{}o}\ \emph {et~al.}(2007)\citenamefont
  {Tworzyd\l{}o}, \citenamefont {Snyman}, \citenamefont {Akhmerov},\ and\
  \citenamefont {Beenakker}}]{TSAB07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tworzyd\l{}o},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont
  {Snyman}}, \bibinfo {author} {\bibfnamefont {A.~R.}\ \bibnamefont
  {Akhmerov}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont
  {Beenakker}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Valley-isospin dependence of the quantum hall effect in a
  graphene $p\text{-}n$ junction},}\ }\href {\doibase
  10.1103/PhysRevB.76.035411} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo {pages}
  {035411}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Tworzyd\l{}o}\ \emph {et~al.}(2006)\citenamefont
  {Tworzyd\l{}o}, \citenamefont {Trauzettel}, \citenamefont {Titov},
  \citenamefont {Rycerz},\ and\ \citenamefont {Beenakker}}]{TTTRB06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Tworzyd\l{}o},
  \bibfnamefont {J}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Trauzettel}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Titov}},
  \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Rycerz}}, \ and\ \bibinfo
  {author} {\bibfnamefont {C.~W.~J.}\ \bibnamefont {Beenakker}}} (\bibinfo
  {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Sub-poissonian shot noise in graphene},}\ }\href {\doibase
  10.1103/PhysRevLett.96.246802} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {96}},\ \bibinfo {pages}
  {246802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Uchoa}\ and\ \citenamefont
  {Castro~Neto}(2007)}]{UCN07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Uchoa}, \bibfnamefont
  {Bruno}}, \ and\ \bibinfo {author} {\bibfnamefont {A.~H.}\ \bibnamefont
  {Castro~Neto}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Superconducting states of pure and doped graphene},}\
  }\href {\doibase 10.1103/PhysRevLett.98.146801} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\
  \bibinfo {pages} {146801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vafek}(2006)}]{V06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Vafek}, \bibfnamefont
  {Oskar}}} (\bibinfo {year} {2006}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Thermoplasma polariton within scaling theory of single-layer
  graphene},}\ }\href {\doibase 10.1103/PhysRevLett.97.266406} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {97}},\ \bibinfo {pages} {266406}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vafek}(2007)}]{V07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Vafek}, \bibfnamefont
  {Oskar}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Anomalous thermodynamics of coulomb-interacting massless dirac
  fermions in two spatial dimensions},}\ }\href {\doibase
  10.1103/PhysRevLett.98.216401} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo {pages}
  {216401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Varchon}\ \emph {et~al.}(2007)\citenamefont
  {Varchon}, \citenamefont {Feng}, \citenamefont {Hass}, \citenamefont {Li},
  \citenamefont {Nguyen}, \citenamefont {Naud}, \citenamefont {Mallet},
  \citenamefont {Veuillen}, \citenamefont {Berger}, \citenamefont {Conrad},\
  and\ \citenamefont {Magaud}}]{Vetal07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Varchon}, \bibfnamefont
  {F}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Feng}}, \bibinfo
  {author} {\bibfnamefont {J.}~\bibnamefont {Hass}}, \bibinfo {author}
  {\bibfnamefont {X.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont
  {B.~Ngoc}\ \bibnamefont {Nguyen}}, \bibinfo {author} {\bibfnamefont
  {C.}~\bibnamefont {Naud}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont
  {Mallet}}, \bibinfo {author} {\bibfnamefont {J.-Y.}\ \bibnamefont
  {Veuillen}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Berger}},
  \bibinfo {author} {\bibfnamefont {E.~H.}\ \bibnamefont {Conrad}}, \ and\
  \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Magaud}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Electronic
  structure of epitaxial graphene layers on sic: Effect of the substrate},}\
  }\href {\doibase 10.1103/PhysRevLett.99.126805} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\
  \bibinfo {pages} {126805}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Visscher}\ and\ \citenamefont
  {Falicov}(1971)}]{VF71}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Visscher},
  \bibfnamefont {P~B}}, \ and\ \bibinfo {author} {\bibfnamefont {L.~M.}\
  \bibnamefont {Falicov}}} (\bibinfo {year} {1971}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Dielectric screening in a layered electron
  gas},}\ }\href {\doibase 10.1103/PhysRevB.3.2541} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {3}},\
  \bibinfo {pages} {2541--2547}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vozmediano}\ \emph {et~al.}(2002)\citenamefont
  {Vozmediano}, \citenamefont {L\'opez-Sancho},\ and\ \citenamefont
  {Guinea}}]{VLG02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Vozmediano},
  \bibfnamefont {M~A~H}}, \bibinfo {author} {\bibfnamefont {M.~P.}\
  \bibnamefont {L\'opez-Sancho}}, \ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Guinea}}} (\bibinfo {year} {2002}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Confinement of electrons in layered metals},}\
  }\href {\doibase 10.1103/PhysRevLett.89.166401} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {89}},\
  \bibinfo {pages} {166401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Vozmediano}\ \emph {et~al.}(2005)\citenamefont
  {Vozmediano}, \citenamefont {L\'opez-Sancho}, \citenamefont {Stauber},\ and\
  \citenamefont {Guinea}}]{VLSG05}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Vozmediano},
  \bibfnamefont {M~A~H}}, \bibinfo {author} {\bibfnamefont {M.~P.}\
  \bibnamefont {L\'opez-Sancho}}, \bibinfo {author} {\bibfnamefont
  {T.}~\bibnamefont {Stauber}}, \ and\ \bibinfo {author} {\bibfnamefont
  {F.}~\bibnamefont {Guinea}}} (\bibinfo {year} {2005}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Local defects and ferromagnetism in graphene
  layers},}\ }\href {\doibase 10.1103/PhysRevB.72.155121} {\bibfield  {journal}
  {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {72}},\
  \bibinfo {pages} {155121}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wakabayashi}\ \emph {et~al.}(1999)\citenamefont
  {Wakabayashi}, \citenamefont {Fujita}, \citenamefont {Ajiki},\ and\
  \citenamefont {Sigrist}}]{WFA+99}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wakabayashi},
  \bibfnamefont {Katsunori}}, \bibinfo {author} {\bibfnamefont {Mitsutaka}\
  \bibnamefont {Fujita}}, \bibinfo {author} {\bibfnamefont {Hiroshi}\
  \bibnamefont {Ajiki}}, \ and\ \bibinfo {author} {\bibfnamefont {Manfred}\
  \bibnamefont {Sigrist}}} (\bibinfo {year} {1999}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Electronic and magnetic properties of
  nanographite ribbons},}\ }\href {\doibase 10.1103/PhysRevB.59.8271}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {59}},\ \bibinfo {pages} {8271--8282}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wakabayashi}\ and\ \citenamefont
  {Sigrist}(2000)}]{WS00}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wakabayashi},
  \bibfnamefont {Katsunori}}, \ and\ \bibinfo {author} {\bibfnamefont
  {Manfred}\ \bibnamefont {Sigrist}}} (\bibinfo {year} {2000}),\ \bibfield
  {title} {\enquote {\bibinfo {title} {Zero-conductance resonances due to flux
  states in nanographite ribbon junctions},}\ }\href {\doibase
  10.1103/PhysRevLett.84.3390} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {84}},\ \bibinfo {pages}
  {3390--3393}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wallace}(1947)}]{W47}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wallace}, \bibfnamefont
  {P~R}}} (\bibinfo {year} {1947}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {The band theory of graphite},}\ }\href {\doibase
  10.1103/PhysRev.71.622} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev.}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo {pages}
  {622--634}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ \emph {et~al.}(2008)\citenamefont {Wang},
  \citenamefont {Sheng}, \citenamefont {Sheng},\ and\ \citenamefont
  {Haldane}}]{WSSH07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wang}, \bibfnamefont
  {Hao}}, \bibinfo {author} {\bibfnamefont {D.~N.}\ \bibnamefont {Sheng}},
  \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Sheng}}, \ and\ \bibinfo
  {author} {\bibfnamefont {F.~D.~M.}\ \bibnamefont {Haldane}}} (\bibinfo {year}
  {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Broken-symmetry
  states of dirac fermions in graphene with a partially filled high landau
  level},}\ }\href {\doibase 10.1103/PhysRevLett.100.116802} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {100}},\ \bibinfo {pages} {116802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ and\ \citenamefont
  {Chakraborty}(2007{\natexlab{a}})}]{WC07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wang}, \bibfnamefont
  {Xue-Feng}}, \ and\ \bibinfo {author} {\bibfnamefont {Tapash}\ \bibnamefont
  {Chakraborty}}} (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Collective excitations of dirac electrons in a
  graphene layer with spin-orbit interactions},}\ }\href {\doibase
  10.1103/PhysRevB.75.033408} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {033408}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wang}\ and\ \citenamefont
  {Chakraborty}(2007{\natexlab{b}})}]{WC07b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wang}, \bibfnamefont
  {Xue-Feng}}, \ and\ \bibinfo {author} {\bibfnamefont {Tapash}\ \bibnamefont
  {Chakraborty}}} (\bibinfo {year} {2007}{\natexlab{b}}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Coulomb screening and collective excitations in
  a graphene bilayer},}\ }\href {\doibase 10.1103/PhysRevB.75.041404}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {041404}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wehling}\ \emph {et~al.}(2008)\citenamefont
  {Wehling}, \citenamefont {Novoselov}, \citenamefont {Morozov}, \citenamefont
  {Vdovin}, \citenamefont {Katsnelson}, \citenamefont {Geim},\ and\
  \citenamefont {Lichtenstein}}]{WNMVKGL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wehling}, \bibfnamefont
  {T~O}}, \bibinfo {author} {\bibfnamefont {K.~S.}\ \bibnamefont {Novoselov}},
  \bibinfo {author} {\bibfnamefont {S.~V.}\ \bibnamefont {Morozov}}, \bibinfo
  {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Vdovin}}, \bibinfo {author}
  {\bibfnamefont {M.~I.}\ \bibnamefont {Katsnelson}}, \bibinfo {author}
  {\bibfnamefont {A.~K.}\ \bibnamefont {Geim}}, \ and\ \bibinfo {author}
  {\bibfnamefont {A.~I.}\ \bibnamefont {Lichtenstein}}} (\bibinfo {year}
  {2008}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Molecular doping of
  graphene},}\ }\href {\doibase 10.1021/nl072364w} {\bibfield  {journal}
  {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo {volume}
  {8}}~(\bibinfo {number} {1}),\ \bibinfo {pages} {173--177}},\ \bibinfo {note}
  {pMID: 18085811}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Williams}\ \emph {et~al.}(2007)\citenamefont
  {Williams}, \citenamefont {DiCarlo},\ and\ \citenamefont {Marcus}}]{WDM07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Williams},
  \bibfnamefont {J~R}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont
  {DiCarlo}}, \ and\ \bibinfo {author} {\bibfnamefont {C.~M.}\ \bibnamefont
  {Marcus}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Quantum hall effect in a gate-controlled p-n junction of
  graphene},}\ }\href {\doibase 10.1126/science.1144657} {\bibfield  {journal}
  {\bibinfo  {journal} {Science}\ }\textbf {\bibinfo {volume} {317}}~(\bibinfo
  {number} {5838}),\ \bibinfo {pages} {638--641}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Williamson}\ \emph {et~al.}(1965)\citenamefont
  {Williamson}, \citenamefont {Foner},\ and\ \citenamefont
  {Dresselhaus}}]{WFD65}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Williamson},
  \bibfnamefont {S~J}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont
  {Foner}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont
  {Dresselhaus}}} (\bibinfo {year} {1965}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {de haas-van alphen effect in pyrolytic and single-crystal
  graphite},}\ }\href {\doibase 10.1103/PhysRev.140.A1429} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume}
  {140}},\ \bibinfo {pages} {A1429--A1447}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wirtz}\ and\ \citenamefont {Rubio}(2004)}]{rubio}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wirtz}, \bibfnamefont
  {Ludger}}, \ and\ \bibinfo {author} {\bibfnamefont {Angel}\ \bibnamefont
  {Rubio}}} (\bibinfo {year} {2004}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {The phonon dispersion of graphite revisited},}\ }\href {\doibase
  10.1016/j.ssc.2004.04.042} {\bibfield  {journal} {\bibinfo  {journal} {Solid
  State Communications}\ }\textbf {\bibinfo {volume} {131}},\ \bibinfo {pages}
  {141 -- 152}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wunsch}\ \emph {et~al.}(2006)\citenamefont {Wunsch},
  \citenamefont {Stauber}, \citenamefont {Sols},\ and\ \citenamefont
  {Guinea}}]{WSSG06}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Wunsch}, \bibfnamefont
  {B}}, \bibinfo {author} {\bibfnamefont {T}~\bibnamefont {Stauber}}, \bibinfo
  {author} {\bibfnamefont {F}~\bibnamefont {Sols}}, \ and\ \bibinfo {author}
  {\bibfnamefont {F}~\bibnamefont {Guinea}}} (\bibinfo {year} {2006}),\
  \bibfield  {title} {\enquote {\bibinfo {title} {Dynamical polarization of
  graphene at finite doping},}\ }\href
  {http://stacks.iop.org/1367-2630/8/i=12/a=318} {\bibfield  {journal}
  {\bibinfo  {journal} {New Journal of Physics}\ }\textbf {\bibinfo {volume}
  {8}}~(\bibinfo {number} {12}),\ \bibinfo {pages} {318}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Xin}\ \emph {et~al.}(2000)\citenamefont {Xin},
  \citenamefont {Jianjun},\ and\ \citenamefont {Zhong-can}}]{zhou00}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Xin}, \bibfnamefont
  {Zhou}}, \bibinfo {author} {\bibfnamefont {Zhou}\ \bibnamefont {Jianjun}}, \
  and\ \bibinfo {author} {\bibfnamefont {Ou-Yang}\ \bibnamefont {Zhong-can}}}
  (\bibinfo {year} {2000}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Strain energy and young's modulus of single-wall carbon nanotubes calculated
  from electronic energy-band theory},}\ }\href {\doibase
  10.1103/PhysRevB.62.13692} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {62}},\ \bibinfo {pages}
  {13692--13696}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Xu}\ \emph {et~al.}(1996)\citenamefont {Xu},
  \citenamefont {Cao}, \citenamefont {Miller}, \citenamefont {Mantell},
  \citenamefont {Miller},\ and\ \citenamefont {Gao}}]{Xetal96}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Xu}, \bibfnamefont
  {S}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Cao}}, \bibinfo
  {author} {\bibfnamefont {C.~C.}\ \bibnamefont {Miller}}, \bibinfo {author}
  {\bibfnamefont {D.~A.}\ \bibnamefont {Mantell}}, \bibinfo {author}
  {\bibfnamefont {R.~J.~D.}\ \bibnamefont {Miller}}, \ and\ \bibinfo {author}
  {\bibfnamefont {Y.}~\bibnamefont {Gao}}} (\bibinfo {year} {1996}),\ \bibfield
   {title} {\enquote {\bibinfo {title} {Energy dependence of electron lifetime
  in graphite observed with femtosecond photoemission spectroscopy},}\ }\href
  {\doibase 10.1103/PhysRevLett.76.483} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {76}},\ \bibinfo
  {pages} {483--486}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yan}\ \emph {et~al.}(2007)\citenamefont {Yan},
  \citenamefont {Zhang}, \citenamefont {Kim},\ and\ \citenamefont
  {Pinczuk}}]{YZKP07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Yan}, \bibfnamefont
  {Jun}}, \bibinfo {author} {\bibfnamefont {Yuanbo}\ \bibnamefont {Zhang}},
  \bibinfo {author} {\bibfnamefont {Philip}\ \bibnamefont {Kim}}, \ and\
  \bibinfo {author} {\bibfnamefont {Aron}\ \bibnamefont {Pinczuk}}} (\bibinfo
  {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Electric
  field effect tuning of electron-phonon coupling in graphene},}\ }\href
  {\doibase 10.1103/PhysRevLett.98.166802} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {166802}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yang}\ \emph
  {et~al.}(2007{\natexlab{a}})\citenamefont {Yang}, \citenamefont {Cohen},\
  and\ \citenamefont {Louie}}]{YCL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Yang}, \bibfnamefont
  {Li}}, \bibinfo {author} {\bibfnamefont {Marvin~L.}\ \bibnamefont {Cohen}}, \
  and\ \bibinfo {author} {\bibfnamefont {Steven~G.}\ \bibnamefont {Louie}}}
  (\bibinfo {year} {2007}{\natexlab{a}}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Excitonic effects in the optical spectra of graphene
  nanoribbons},}\ }\href {\doibase 10.1021/nl0716404} {\bibfield  {journal}
  {\bibinfo  {journal} {Nano Letters}\ }\textbf {\bibinfo {volume}
  {7}}~(\bibinfo {number} {10}),\ \bibinfo {pages} {3112--3115}}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Yang}\ \emph
  {et~al.}(2007{\natexlab{b}})\citenamefont {Yang}, \citenamefont {Park},
  \citenamefont {Son}, \citenamefont {Cohen},\ and\ \citenamefont
  {Louie}}]{YPSCL07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Yang}, \bibfnamefont
  {Li}}, \bibinfo {author} {\bibfnamefont {Cheol-Hwan}\ \bibnamefont {Park}},
  \bibinfo {author} {\bibfnamefont {Young-Woo}\ \bibnamefont {Son}}, \bibinfo
  {author} {\bibfnamefont {Marvin~L.}\ \bibnamefont {Cohen}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Steven~G.}\ \bibnamefont {Louie}}} (\bibinfo {year}
  {2007}{\natexlab{b}}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Quasiparticle energies and band gaps in graphene nanoribbons},}\ }\href
  {\doibase 10.1103/PhysRevLett.99.186801} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {99}},\ \bibinfo
  {pages} {186801}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yang}\ and\ \citenamefont {Nayak}(2002)}]{Yang02}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Yang}, \bibfnamefont
  {Xiao}}, \ and\ \bibinfo {author} {\bibfnamefont {Chetan}\ \bibnamefont
  {Nayak}}} (\bibinfo {year} {2002}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electrical and thermal transport by nodal quasiparticles in the
  \textit{d} -density-wave state},}\ }\href {\doibase
  10.1103/PhysRevB.65.064523} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {65}},\ \bibinfo {pages}
  {064523}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Yao}\ \emph {et~al.}(2007)\citenamefont {Yao},
  \citenamefont {Ye}, \citenamefont {Qi}, \citenamefont {Zhang},\ and\
  \citenamefont {Fang}}]{YYQZF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Yao}, \bibfnamefont
  {Yugui}}, \bibinfo {author} {\bibfnamefont {Fei}\ \bibnamefont {Ye}},
  \bibinfo {author} {\bibfnamefont {Xiao-Liang}\ \bibnamefont {Qi}}, \bibinfo
  {author} {\bibfnamefont {Shou-Cheng}\ \bibnamefont {Zhang}}, \ and\ \bibinfo
  {author} {\bibfnamefont {Zhong}\ \bibnamefont {Fang}}} (\bibinfo {year}
  {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Spin-orbit gap of
  graphene: First-principles calculations},}\ }\href {\doibase
  10.1103/PhysRevB.75.041401} {\bibfield  {journal} {\bibinfo  {journal} {Phys.
  Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages}
  {041401}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zarea}\ and\ \citenamefont {Sandler}(2007)}]{ZS07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zarea}, \bibfnamefont
  {Mahdi}}, \ and\ \bibinfo {author} {\bibfnamefont {Nancy}\ \bibnamefont
  {Sandler}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Electron-electron and spin-orbit interactions in armchair graphene
  ribbons},}\ }\href {\doibase 10.1103/PhysRevLett.99.256804} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {99}},\ \bibinfo {pages} {256804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}\ and\ \citenamefont
  {Joglekar}(2007)}]{ZJ0703}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhang}, \bibfnamefont
  {C-H}}, \ and\ \bibinfo {author} {\bibfnamefont {Yogesh~N.}\ \bibnamefont
  {Joglekar}}} (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Wigner crystal and bubble phases in graphene in the
  quantum hall regime},}\ }\href {\doibase 10.1103/PhysRevB.75.245414}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo
  {volume} {75}},\ \bibinfo {pages} {245414}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}\ and\ \citenamefont {Fogler}(2008)}]{ZF07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhang}, \bibfnamefont
  {L~M}}, \ and\ \bibinfo {author} {\bibfnamefont {M.~M.}\ \bibnamefont
  {Fogler}}} (\bibinfo {year} {2008}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Nonlinear screening and ballistic transport in a graphene
  $p\mathrm{\text{-}}n$ junction},}\ }\href {\doibase
  10.1103/PhysRevLett.100.116804} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo {pages}
  {116804}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}\ \emph {et~al.}(2006)\citenamefont {Zhang},
  \citenamefont {Jiang}, \citenamefont {Small}, \citenamefont {Purewal},
  \citenamefont {Tan}, \citenamefont {Fazlollahi}, \citenamefont {Chudow},
  \citenamefont {Jaszczak}, \citenamefont {Stormer},\ and\ \citenamefont
  {Kim}}]{Zetal06b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhang}, \bibfnamefont
  {Y}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Jiang}}, \bibinfo
  {author} {\bibfnamefont {J.~P.}\ \bibnamefont {Small}}, \bibinfo {author}
  {\bibfnamefont {M.~S.}\ \bibnamefont {Purewal}}, \bibinfo {author}
  {\bibfnamefont {Y.-W.}\ \bibnamefont {Tan}}, \bibinfo {author} {\bibfnamefont
  {M.}~\bibnamefont {Fazlollahi}}, \bibinfo {author} {\bibfnamefont {J.~D.}\
  \bibnamefont {Chudow}}, \bibinfo {author} {\bibfnamefont {J.~A.}\
  \bibnamefont {Jaszczak}}, \bibinfo {author} {\bibfnamefont {H.~L.}\
  \bibnamefont {Stormer}}, \ and\ \bibinfo {author} {\bibfnamefont
  {P.}~\bibnamefont {Kim}}} (\bibinfo {year} {2006}),\ \bibfield  {title}
  {\enquote {\bibinfo {title} {Landau-level splitting in graphene in high
  magnetic fields},}\ }\href {\doibase 10.1103/PhysRevLett.96.136806}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {96}},\ \bibinfo {pages} {136806}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhang}\ \emph {et~al.}(2005)\citenamefont {Zhang},
  \citenamefont {Tan}, \citenamefont {Stormer},\ and\ \citenamefont
  {Kim}}]{Zetal05b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhang}, \bibfnamefont
  {Yuanbo}}, \bibinfo {author} {\bibfnamefont {Yan-Wen}\ \bibnamefont {Tan}},
  \bibinfo {author} {\bibfnamefont {Horst~L.}\ \bibnamefont {Stormer}}, \ and\
  \bibinfo {author} {\bibfnamefont {Philip}\ \bibnamefont {Kim}}} (\bibinfo
  {year} {2005}),\ \bibfield  {title} {\enquote {\bibinfo {title} {Experimental
  observation of quantum hall effect and berry's phase in graphene},}\ }\href
  {doi:10.1038/nature04235} {\bibfield  {journal} {\bibinfo  {journal}
  {NATURE}\ }\textbf {\bibinfo {volume} {438}},\ \bibinfo {pages}
  {201}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhong-can}\ \emph {et~al.}(1997)\citenamefont
  {Zhong-can}, \citenamefont {Su},\ and\ \citenamefont {Wang}}]{zhou97}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhong-can},
  \bibfnamefont {Ou-Yang}}, \bibinfo {author} {\bibfnamefont {Zhao-Bin}\
  \bibnamefont {Su}}, \ and\ \bibinfo {author} {\bibfnamefont {Chui-Lin}\
  \bibnamefont {Wang}}} (\bibinfo {year} {1997}),\ \bibfield  {title} {\enquote
  {\bibinfo {title} {Coil formation in multishell carbon nanotubes: Competition
  between curvature elasticity and interlayer adhesion},}\ }\href {\doibase
  10.1103/PhysRevLett.78.4055} {\bibfield  {journal} {\bibinfo  {journal}
  {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {78}},\ \bibinfo {pages}
  {4055--4058}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhu}\ and\ \citenamefont {Cai}(2007)}]{GAW07}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Zhu}, \bibfnamefont
  {Yun}}, \ and\ \bibinfo {author} {\bibfnamefont {J.~W.}\ \bibnamefont {Cai}}}
  (\bibinfo {year} {2007}),\ \bibfield  {title} {\enquote {\bibinfo {title}
  {Ultrahigh sensitivity hall effect in magnetic multilayers},}\ }\href
  {\doibase 10.1063/1.2426896} {\bibfield  {journal} {\bibinfo  {journal}
  {Applied Physics Letters}\ }\textbf {\bibinfo {volume} {90}}~(\bibinfo
  {number} {1}),\ \bibinfo {eid} {012104}}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ziegler}(1998)}]{Ziegler98}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibnamefont {Ziegler}, \bibfnamefont
  {K}}} (\bibinfo {year} {1998}),\ \bibfield  {title} {\enquote {\bibinfo
  {title} {Delocalization of 2d dirac fermions: The role of a broken
  supersymmetry},}\ }\href {\doibase 10.1103/PhysRevLett.80.3113} {\bibfield
  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo
  {volume} {80}},\ \bibinfo {pages} {3113--3116}}\BibitemShut {NoStop}%
\end{thebibliography}%
